Resilient Two-Time-Scale Local Stochastic Gradient Descent for Byzantine Federated Learning

We study local stochastic gradient descent methods for solving federated optimization over a network of agents communicating indirectly through a centralized coordinator. We are interested in the Byzantine setting where there is a subset of $f$ malicious agents that could observe the entire network and send arbitrary values to the coordinator to disrupt the performance of other non-faulty agents. The objective of the non-faulty agents is to collaboratively compute the optimizer of their respective local functions under the presence of Byzantine agents. In this setting, prior works show that the local stochastic gradient descent method can only return an approximate of the desired solutions due to the impacts of Byzantine agents. Whether this method can find an exact solution remains an open question. In this paper, we will address this open question by proposing a new variant of the local stochastic gradient descent method. Under similar conditions that are considered in the existing works, we will show that the proposed method converges exactly to the desired solutions. We will provide theoretical results to characterize the convergence properties of our method, in particular, the proposed method convergences at an optimal rate $\mathcal{O}(1/k)$ in both strongly convex and non-convex settings, where $k$ is the number of iterations. Finally, we will present a number of simulations to illustrate our theoretical results.

==> Introduction.tex <==
\section{Introduction}

The constant expansion of large networks has resulted in an exponential growth of data, creating a pressing need for higher computational power and storage requirements. To address this demand, numerous distributed algorithms have been developed, where computation and data are distributed over networks. Federated learning has emerged as a popular distributed framework that facilitates collaborative training of a shared model by multiple devices \cite{mcmahan2017communication, zhao2021fedpage, woodworth2020local,Kairouz_survery2020,Li_survery2020}. This technique is particularly relevant in the context of wireless communication networks \cite{niknam2020federated}, \cite{yang2020energy}, \cite{chen2021distributed}, \cite{khan2021federated}, where there is a growing need for efficient and scalable machine learning solutions due to the rapidly increasing number of wireless devices. In this context, a common problem often reduces to optimize an aggregate objective function that is composed of $N$  functions distributed at $N$ different  agents (e.g., mobile devices). One prominent example is the problem of federated spectrum sensing over a wireless sensor network, where the goal is to decide the availabilty of spectrum. By using federated learning framework, the updates of any optimization algorithm can be implemented locally at the agents without requiring data being transmitted to the centralized coordinator (e.g., a server/network operator). By keeping data locally, federated learning not only reduces the amount of communications between agents and the server but also provides some level of privacy. For example, in federated spectrum sensing each user learns about the availability of spectrum from their local network and sends updates to a server. Based on all the local decisions the server sends an aggregated decisions back to the users. This process continues until the network reaches an optimal solution for deciding which frequency bands are available for communication.

One of the main challenges in federated learning is the vulnerability of the system to malicious attacks where some agents in the network may fail or whose updates can be manipulated by an external entity. Such malicious agents will have detrimental impacts to the performance of other agents, and if not addressed, it can lead to catastrophic failures of entire network. Indeed, (Byzantine) malicious attacks have been identified as the most critical problem in wireless spectrum sensing \cite{shi2021challenges}.    

In this paper, we study the performance of federated learning, in particular, the celebrated distributed local stochastic gradient descent (SGD), when a (small) number of agents in the network is malicious. We will focus on Byzantine malicious attacks, where Byzantine agents can observe the entire network and send any information to the centralized coordinator. Under the presence of Byzantine agents, it is impossible for nonfaulty agents to find the optimizer of the aggregate of functions at every agent (including Byzantine agents) as Byzantine agents can send a random number irrelevant to its function. Thus, we consider another meaningful objective in this setting, where the goal is to solve the optimization problem only involving the honest agents. In particular, we consider the setting where there are up to $f$ faulty Byzantine agents with unknown identities. Our goal is address the following exact fault-tolerance problem.

\textbf{Exact fault-tolerance problem}: 
Let $\mathcal{H}$ be the set of honest agents with $|\mathcal{H}| \geq N-f$, then a distributed optimization algorithm is said to have exact fault-tolerance if it allows all the non-faulty agents to compute
\begin{align}\label{eq:exact_tolerence}
    x_{\mathcal{H}}^{*} \in \arg \min_{x\in \mathbb{R}^{d}}\sum_{i \in \mathcal{H}}q^{i}(x).
\end{align}
Note that if the number of Byzantine agent is too large, (i.e, $f\gg \mathcal{H}$, it is also impossible to solve problem \eqref{eq:exact_tolerence} by using any federated learning algorithms. We, therefore, consider the following $2f$-\textit{redundancy} condition, which is necessary and sufficient for solving problem \eqref{eq:exact_tolerence}  \cite{gupta2020fault}. 
\begin{definition}[$2f$-\textbf{redundancy}]
The set of non-faulty agents $\mathcal{H}$, with $|\mathcal{H}| \geq N-f$, is said to have $2f$-redundancy if for any subset $\mathcal{S} \subset \mathcal{H}$ with $|\mathcal{S}| \geq N -2f$,
\begin{align}
    \arg \min_{x\in \mathbb{R}^{d}}\sum_{i \in \mathcal{S}}q^{i}(x) = \arg \min_{x\in \mathbb{R}^{d}}\sum_{i \in \mathcal{H}}q^{i}(x). 
\end{align}
\end{definition}
The above definition states that solving the optimization problem defined over the honest agent is same as solving the problem defined over at least $N-2f$ honest agents. We will study the performance of distributed local SGD under the 2f-redundancy condition. Motivated by the recent work in \cite{gupta2023byzantine}, we will consider the so-called comparative elimination (CE) filter in the distributed local SGD to mitigate the detrimental impact of Byzantine agents. Our focus is to provide theoretical results to show the convergence of distributed local SGD with CE filter in a nonconvex setting. Motivated by the recent work on distributed local SGD under Byzantine attack, we will consider   with \textit{comparative elimination} byzantine filter. This filter aims to mitigate the affect of the byzantine agents. Here a strongly convex global objective is considered. However, since most of the real world applications use non-convex functions hence, investigating the impact of Byzantine agents in the presence of such objectives is crucial. This paper considers the case where the global objective function is non-convex that satisfies the popular Polyak-Łojasiewicz (PL) condition \cite{karimi2016linear}.

\noindent\textbf{The main contribution} of this paper is to study the performance of federated local SGD with \textit{comparative elimination} (CE) for solving distributed nonconvex optimization problems under Byzantine attacks and satisfying the 2f-redundancy condition.  In particular, when the objective function satisfies Polyak-\L ojasiewicz (PL) condition, we show that this method solves the exact fault-tolerance problem at a linear rate. We will study theoretical results for both deterministic and stochastic setting. Finally, we will provide a number of numerical simulations to illustrate our theoretical results.

% For the deterministic case,  Honest agents accurately compute local function gradients, achieving exact fault tolerance with exponential convergence. We require $\frac{f}{|\mathcal{H}|}\leq \frac{\mu}{3L}$ with $\frac{\mu}{L} \leq 1$ where $\mu,L$ are the properties of aggregate non-faulty agents' objective.
% \item \textbf{Stochastic case}: Here the honest users have access to a sampled version of their gradients, $\nabla Q^{i}(. , X^{i})$, achieving approximate fault tolerance with convergence to an approximate solution in the neighborhood of the optimal solution. The approximation error is proportional to the variance of the stochastic gradients and the ratio of faulty to honest agents.
% \end{itemize}
% Detailed discussion and analysis of our results can be found in Section \ref{sec:Main_results}.
\subsection{Related work}
According to existing literature, there are various Byzantine fault-tolerant aggregation schemes for distributed optimization and learning. These include \textit{multi-KRUM} \cite{blanchard2017machine}, \textit{coordinate-wise trimmed mean} (CWTM) \cite{su2019finite}, \textit{geometric median-of-means}(GMoM) \cite{chen2017distributed}, \textit{minimum-diameter averaging} (MDA) \cite{guerraoui2018hidden}, and \textit{Byzantine-robust stochastic aggregation} (RSA) \cite{li2019rsa} filters. However, it is important to note that these schemes do not guarantee \textit{exact fault-tolerance} even in a deterministic setting with $2f$-redundancy, unless additional assumptions are made regarding the objectives of the honest agents. The work by \cite{gupta2023byzantine} shows that it is possible to achieve exact fault tolerance in deterministic setting and approximate fault tolerance in stochastic setting in $2f$ redundancy scenario. Recently \cite{farhadkhani2022byzantine} proposed \textit{RESilient Averaging of Momentum} (RESAM) which presents an unified byzantine fault-tolerant framework with accelerated gradient descent based on the previously mentioned methods. They also established finite time convergence with some additional assumptions. Although their results hold for non-convex objectives, they clearly proved that such generalization and acceleration cannot be applied for the CE aggregation scheme. Our work in this paper extends the one in \cite{gupta2023byzantine} to non-convex setting, where the global objective function satisfies the PL condition, thereby expanding the analytical framework beyond the strongly convex scenario. We also want to note some relevant work in \cite{cao2019distributed, cao2020distributed}, where the authors study approximate fault tolerance problem with more relaxed conditions on the Byzantine agents. 
% with presence of arbitrary number of byzantine agents but introduced additional computation at the server end. The authors further extended their work for Newton's second order descent method in \cite{cao2020distributed}. In both the works authors established their results based on strongly convex objectives.   

% In this context, we show exact fault tolerance  that where agents have access to their true local gradients. Additionally in the case where agents merely observe an instance of their local gradients, we can only achieve approximate fault tolerance. To validate our theoretical contributions, we conduct simulations to confirm the efficacy of our proposed techniques. Furthermore, we investigate the case where the objective function is purely non-convex and may not satisfy the PL condition. Although we provide simulation results for this scenario, theoretical analysis is left for future work.
% 

% Specifically, federated learning has been applied to various wireless network scenarios, including mobile edge networks \cite{lim2020federated}, Internet of Things (IoT) \cite{khan2021federated}, 5G \cite{liu2020secure}, and 6G \cite{yang2022federated}. The motivation for our work stems from spectrum sensing tasks, including anomaly detection, authentication, and fault diagnostics, which are essential functions for the emerging NextG networks \cite{shi2022federated}, \cite{akyildiz2006next}. Typically, these scenarios employ the client-server paradigm, with single-hop wireless links being used for communication. Federated Learning is a decentralized machine learning methodology that facilitates collaborative training of a shared model by multiple devices within a wireless network, such as mobile users, UAVs, or IoT devices, without the need for raw data transfer to a central server. Here we consider a setting of $N$ agents/devices with each $i^{\text{th}}$ agent having a local function $q^{i}:\mathbb{R}^{d}\to \mathbb{R}$.In many cases, the local functions involved in Federated Learning are non-convex. For instance, in \cite{shi2022federated}, the authors employ a feed-forward neural network (FNN) to model $q^{i}$. 



% Falsified data in wireless network devices can be caused by various factors such as jamming, external interception, and eavesdropping.



==> Lemma1.tex <==
\section{Lemma \ref{lem:Lemma_V1_SC}}
Using the update equation from \eqref{eq:algo_update_Tg1} we have
\begin{align}\label{eq:x_update_error}
    x^{i}_{k,t+1} &= x^{i}_{k,t} - \beta_{k} y^{i}_{k,t} \notag\\
    & = \Bar{x}_{k} -\beta_{k}\sum_{l=0}^{t}y^{i}_{k,l}\notag\\
    & = \Bar{x}_{k} -\beta_{k}\sum_{l=0}^{t}e^{i}_{k,l} -\beta_{k}\sum_{l=0}^{t}\nabla q^{i}(\Bar{x}_{k}).
\end{align}
From which we have
\begin{align}\label{eq:x_update_T}
    x^{i}_{k,\mathcal{T}} = \Bar{x}_{k} -\beta_{k}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l} -\beta_{k}\sum_{l=0}^{\mathcal{T}-1}\nabla q^{i}(\bar{x}_{k}).
\end{align}
For our analysis, we first note that $|\mathcal{F}_{k}| = |\mathcal{H}|$ and $|\mathcal{B}_{k}| = |\mathcal{H}\backslash\mathcal{H}_{k}|$. Thus from line $15$ in Algorithm \ref{alg:cap} we have the following,
    \begin{align}
        \Bar{x}_{k+1}&=\frac{1}{|\mathcal{F}_{k}|}\sum_{i \in \mathcal{F}_{k}}x^{i}_{k,\mathcal{T}}\notag \\
        &=\frac{1}{|\mathcal{H}|}\Big[\sum_{i\in \mathcal{H}}x^{i}_{k,\mathcal{T}} + \sum_{i\in \mathcal{B}_{k}}x^{i}_{k,\mathcal{T}} - \sum_{i\in \mathcal{H} \backslash \mathcal{H}_{k}}x^{i}_{k,\mathcal{T}}\Big], \notag \\
        & = \frac{1}{|\mathcal{H}|} \sum_{i\in \mathcal{H}}x^{i}_{k,\mathcal{T}}  + V_{x}.\notag
    \end{align}
    where 
    \begin{align}\label{eq:V_x}
        V_{x} = \frac{1}{|\mathcal{H}|}\Big[\sum_{i\in \mathcal{B}_{k}}(x^{i}_{k,\mathcal{T}} -\Bar{x}_{k}) - \sum_{i\in \mathcal{H} \backslash \mathcal{H}_{k}}(x^{i}_{k,\mathcal{T}}-\Bar{x}_{k})\Big]
    \end{align}
    Next we use \eqref{eq:avg_q_h} and \eqref{eq:x_update_T} which gives us,
    \begin{align}\label{eq:x_bar_update}
        \Bar{x}_{k+1} = \Bar{x}_{k}-\mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\Bar{x}_{k})-\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}+ V_{k},
    \end{align}
    using which we have
    \begin{align}
        &\|\Bar{x}_{k+1} -x^{*}_{\mathcal{H}}\|^{2}\notag \\
        &= \|\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\|^{2} + \Big\|V_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big\|^{2} \notag\\
        &-2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\Big(V_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big)\notag
    \end{align}
    Next using the strongly convex and lipschitz continuity assumption from \eqref{eq:sc_condition},\eqref{eq:Lip_condition} respectively we have the following
    \begin{align}\label{eq:x_bar_opt}
        &\|\Bar{x}_{k+1} -x^{*}_{\mathcal{H}}\|^{2}\notag \\
        &\leq (1-2\mu\mathcal{T}\beta_{k} + \mathcal{T}^{2}L^{2}\beta_{k}^{2})\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}\notag\\
        &+ \Big\|V_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big\|^{2} \notag\\
        &-2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\Big(V_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big)\notag
    \end{align}
    Next using $\|a+b\|^{2} \leq 2\|a\|^{} + 2\|b\|^{2}$ for ant vector $a$ and $b$ we analyze the second term of the above equation as the following
    \begin{align}
        &\|\Bar{x}_{k+1} -x^{*}_{\mathcal{H}}\|^{2}\notag \\
        &\leq (1-2\mu\mathcal{T}\beta_{k} + \mathcal{T}^{2}L^{2}\beta_{k}^{2})\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + 2\|V_{x}\|^{2}\notag\\
        +& \frac{2\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2}-2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}V_{x}\notag\\
        &+2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\Big(\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big)\notag
    \end{align}
Using the inequality $2a^{T}b \leq \eta\|a\|^{2} + \frac{\|b\|^{2}}{\eta}$ for any non-zero vectors $a,b$ and for all $\eta >0$ where choose $\eta = \frac{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|}$ to analyze the second last term and $\eta = \frac{L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}$ to analyze the last term
\begin{align}\label{eq:x_bar_optimal_update}
        &\|\Bar{x}_{k+1} -x^{*}_{\mathcal{H}}\|^{2}\notag \\
        & \leq (1-2\mu\mathcal{T}\beta_{k} + \mathcal{T}^{2}L^{2}\beta_{k}^{2})\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} +2\|V_{x}\|^{2}\notag\\
        &+\frac{2\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} + \frac{|\mathcal{H}|}{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}\|V_{x}\|^{2}\notag\\
        &+\frac{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|} (\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}+L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}) \notag\\
        &+\frac{L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|} (\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}+L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2})\notag\\
        &+\frac{6\beta_{k}}{L}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}\notag\\
        & \leq (1-2\mu\mathcal{T}\beta_{k} + \mathcal{T}^{2}L^{2}\beta_{k}^{2})\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} \notag\\
        &+\frac{19L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}+ \frac{19L^{3}\mathcal{T}^{3}\beta_{k}^{3}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} \notag\\
        &+2\|V_{x}\|^{2}+ \frac{|\mathcal{H}|}{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}\|V_{x}\|^{2}\notag\\
        &+\frac{2\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} +\frac{6\beta_{k}}{L}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}.
\end{align}
Next, we analyze $\|V_{x}\|^{2}$. Using \eqref{eq:V_x} and the fact that there exists an agent $j \in \mathcal{H}$ such that $\|x^{i}_{k,t}-\Bar{x}_{k}\| \leq \|x^{j}_{k,t}-\Bar{x}_{k}\|$ for all agent $i \in \mathcal{B}_{k}$, we obtain
\begin{align}\label{eq:V_x_update}
    \|V_{x}\|^{2} &\leq \frac{2|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\|x^{j}_{k,\mathcal{T}} - \Bar{x}_{k}\|^{2} + \frac{2|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\|x^{i}_{k,\mathcal{T}} - \Bar{x}_{k}\|^{2} \notag\\
    & \leq \frac{2|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}(2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2})\notag\\
    &+ \frac{2|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}(2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2})\notag\\
    & \leq \frac{8L^{2}\mathcal{T}^{2}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + \frac{4\mathcal{T}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}\notag\\
    &+ \frac{4\mathcal{T}\beta_{k}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2},
\end{align}
% From which we have 
% \begin{align}\label{eq:Vk}
%     \mathbb{E}[\|V_{k}\|^{2}] \leq \frac{8L^{2}\mathcal{T}^{2}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] +\frac{8\mathcal{T}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\epsilon_{k},
% \end{align}
% where
% \begin{align}
%     \epsilon_{k} = \sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]
% \end{align}
Now putting back putting which back \eqref{eq:V_x_update} in \eqref{eq:x_bar_optimal_update} and taking expectation on both sides we have
\begin{align}
    &\mathbb{E}[\|\Bar{x}_{k+1}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &\leq (1-2\mu\mathcal{T}\beta_{k}+L^{2}\mathcal{T}^{2}\beta_{K}^{2})\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ \frac{35L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\frac{16L^{2}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ \frac{19L^{3}\mathcal{T}^{3}\beta^{3}_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\frac{6\beta_{k}}{L}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]+\frac{2\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+\frac{8\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]+\frac{8\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+\frac{4\beta_{k}\mathcal{T}|\mathcal{B}_{k}|}{3L|\mathcal{H}|}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]+\frac{4\beta_{k}\mathcal{T}}{3L|\mathcal{H}|}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}],\notag
\end{align}
which can be further simplified using 
\begin{align}\label{eq:e_k_t_relations}
    &\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} \leq \sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}, \notag\\
    &\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} \leq \sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2},
\end{align} thus obtaining the following,
\begin{align}\label{eq:x_bar_opt}
    &\mathbb{E}[V^{k+1}_{1}]\notag\\
    &\leq \Big(1-2\mu\mathcal{T}\beta_{k}+L^{2}\mathcal{T}^{2}\beta_{k}^{2}+\frac{35L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\Big)\mathbb{E}[V^{k}_{1}] \notag\\
    &+\Big(\frac{16L^{2}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}+ \frac{19L^{3}\mathcal{T}^{3}\beta^{3}_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\Big)\mathbb{E}[V^{k}_{1}] \notag\\
    &+\Big(2\beta^{2}_{k}\mathcal{T}\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|}+\frac{6\beta_{k}}{L} + \frac{8\beta_{k}|\mathcal{B}_{k}|}{3L|\mathcal{H}|} \Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \frac{16\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}].
\end{align}

% where 
% \begin{align}\label{eq:epsilon_k}
%     \epsilon_{k}= \sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]
% \end{align}

==> Lemma2.tex <==
\section{Lemma \ref{lem:Lemma_V2_SC}}
\begin{proof}
Using the definition of $e^{i}_{k,t}$ from \eqref{eq:e_k_t} and since $y^{i}_{k+1,0} = y^{i}_{k,\mathcal{T}}$ we have,
\begin{align}
    e^{i}_{k+1,0} &= y^{i}_{k+1,0} - \nabla q^{i}(\Bar{x}_{k+1})\notag\\
    & = y^{i}_{k,\mathcal{T}}- \nabla q^{i}(\Bar{x}_{k+1})\notag\\
    & = e^{i}_{k,\mathcal{T}} + \nabla q^{i}(\Bar{x}_{k})-\nabla q^{i}(\Bar{x}_{k+1})
\end{align}
Next, applying the inequality $\|a + b\|^2 \leq (1+\eta)\|a\|^{2} + (1+\frac{1}{\eta})\|b\|^{2}$, with the choice of $\eta = \frac{\alpha_{k}}{2}$ we obtain,
\begin{align}
    &\|e^{i}_{k+1,0}\|^{2} \notag\\
    & \leq \Big(1+\frac{\alpha_{k}}{2}\Big)\|e^{i}_{k,\mathcal{T}}\|^{2} + \Big(1+\frac{2}{\alpha_{k}}\Big)\|\nabla q^{i}(\Bar{x}_{k}) - \nabla q^{i}(\Bar{x}_{k+1})\|^{2}\notag\\
    &\leq \Big(1+\frac{\alpha_{2}}{2}\Big)\|e^{i}_{k,\mathcal{T}}\|^{2} + \Big(1+\frac{2}{\alpha_{k}}\Big)L^{2}\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}\notag\\
    &\leq \Big(1+\frac{\alpha_{2}}{2}\Big)\|e^{i}_{k,\mathcal{T}}\|^{2} + \frac{3L^{2}}{\alpha_{k}}\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2},
\end{align}
% where the last inequality is obtained due to $\alpha_{k} \leq 1$ which leads to $\Big(1+\frac{2}{\alpha_{k}}\Big)L^{2} \leq \frac{3L^{2}}{\alpha_{k}}$. 
Thus we have
\begin{align}\label{eq:V_2_r0}
    &\mathbb{E}[V^{k+1}_{2}] = \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|e^{i}_{k+1,0}\|^{2}]\notag\\
    &\leq \Big(1+\frac{\alpha_{k}}{2}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|e^{i}_{k,\mathcal{T}}\|^{2}] + \frac{3L^{2}}{\alpha_{k}|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|\Bar{x}_{k+1} - \Bar{x}_{k}\|^{2}]
\end{align}
Next we analyze the first term in the right hand side of the above inequality. Using \eqref{eq:e_k_t} we have 
\begin{align}
    &e^{i}_{k,t+1}\notag\\
    &= y^{i}_{k,t+1} - \nabla q^{i}(\Bar{x}_{k})\notag\\
    & = (1-\alpha_{k})y^{i}_{k,t} + \alpha_{k}\nabla Q^{i}(x^{i}_{k,t};\Delta^{i}_{k,t}) - \nabla q^{i}(\Bar{x}_{k})\notag\\
    & = (1-\alpha_{k})e^{i}_{k,t}  + \alpha_{k}\nabla Q^{i}(x^{i}_{k,t};\Delta^{i}_{k,t}) - \nabla q^{i}(\Bar{x}_{k})\notag\\
    &+ (1-\alpha_{k})\nabla q^{i}(\Bar{x}_{k})\notag\\
    & = (1-\alpha_{k})e^{i}_{k,t} + \alpha_{k}(\nabla Q^{i}(x^{i}_{k,t},\Delta^{i}_{k,t}) - \nabla q^{i}(x^{i}_{k,t}))\notag\\
    &+\alpha_{k}(\nabla q^{i}(x^{i}_{k,t})-\nabla q^{i}(\Bar{x}_{k}))
\end{align}
Next squaring both sides of the above equation and taking conditional expectation with respect to the filtration $\mathcal{P}_{k,t}$ we have
\begin{align}
    &\mathbb{E}[\|e^{i}_{k,t+1}\|^{2}|\mathcal{P}_{k,t}]\notag\\
    &= (1-\alpha_{k})^{2}\|e^{i}_{k,t}\|^{2} + \alpha^{2}_{k}\|\nabla q^{i}(x^{i}_{k,t})-\nabla q^{i}(\Bar{x}_{k})\|^{2}\notag\\
    &+ \alpha^{2}_{k}\mathbb{E}[\|\nabla Q^{i}(x^{i}_{k,t},\Delta^{i}_{k,t}) - \nabla q^{i}(x^{i}_{k,t})\|^{2}]\notag\\
    &+ 2\alpha_{k}(1-\alpha_{k})(\nabla q^{i}(x^{i}_{k,t})-\nabla q^{i}(\Bar{x}_{k}))^{T}e^{i}_{k,t}\notag\\
    & + 2\alpha_{k}(1-\alpha_{k})\mathbb{E}[(\nabla Q^{i}(x^{i}_{k,t},\Delta^{i}_{k,t}) - \nabla q^{i}(x^{i}_{k,t}))^{T}e^{i}_{k,t}|\mathcal{P}_{k,t}]\notag\\
    &+2\alpha^{2}_{k}\mathbb{E}[(\nabla Q^{i}(x^{i}_{k,t},\Delta^{i}_{k,t}) - \nabla q^{i}(x^{i}_{k,t}))^{T}(\nabla q^{i}(x^{i}_{k,t})-\nabla q^{i}(\Bar{x}_{k})|\mathcal{P}_{k,t}]\notag
\end{align}
Due to the unbiased estimates of the gradients as indicated by \eqref{eq:sigma}, the second last term and the last term of the above equation is zero. Further due to the bounded variance of the stochastic gradients and Lipschitz continuity of $\nabla q^{\mathcal{H}}$ we have
\begin{align}
    &\mathbb{E}[\|e^{i}_{k,t+1}\|^{2}] \leq (1-\alpha_{k})^{2}\mathbb{E}[\|e^{i}_{k,t}\|^{2}] + \alpha^{2}_{k}L^{2}\mathbb{E}[\|x^{i}_{k,t} - \Bar{x}_{k}\|^{2}] \notag\\
    & + \alpha^{2}_{k}\sigma^{2}+ 2\alpha_{k}(1-\alpha_{k})\mathbb{E}[(\nabla q^{i}(x^{i}_{k,t}) - \nabla q^{i}(\Bar{x}_{k}))^{T}e^{i}_{k,t}]\notag
\end{align}
Next using the inequality $2a^{T}b \leq \|a\|^{2} + \|b\|^{2}$ for vectors $a$ and $b$ along with the Lipschiz continuity of $\nabla q^{i}$ we analyze the last term of the above equation as the following
\begin{align}\label{eq:e_k_t_iteration}
    &\mathbb{E}[\|e^{i}_{k,t+1}\|^{2}] \notag\\
    &\leq (1-\alpha_{k})^{2}\mathbb{E}[\|e^{i}_{k,t}\|^{2}] + \alpha^{2}_{k}L^{2}\mathbb{E}[\|x^{i}_{k,t} - \Bar{x}_{k}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\notag\\
    & + \alpha_{k}(1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,t}\|^{2}]+ \alpha_{k}(1-\alpha_{k})L^{2}\mathbb{E}[\|x^{i}_{k,t}-\Bar{x}_{k}\|^{2}]\notag\\
    & = (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,t}\|^{2}] + \alpha_{k}L^{2}\mathbb{E}[\|x^{i}_{k,t} - \Bar{x}_{k`}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\notag\\
    & \leq (1-\alpha_{k})^{t+1}\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\sum_{l=0}^{t}(1-\alpha_{k})^{l} \notag\\
    & + \alpha_{k}L^{2}\sum_{l=0}^{t}(1-\alpha_{k})^{t-l}\mathbb{E}[\|x^{i}_{k,l} - \Bar{x}_{k}\|^{2}],
\end{align}
which gives us 
\begin{align}
    &\mathbb{E}[\|e^{i}_{k,\mathcal{T}}\|^{2}]\notag\\
    &\leq (1-\alpha_{k})^{\mathcal{T}}\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + + \alpha^{2}_{k}\sigma^{2}\sum_{l=0}^{\mathcal{T}-1}(1-\alpha_{k})^{l} \notag\\
    &+ \alpha_{k}L^{2}\sum_{l=0}^{\mathcal{T}-1}(1-\alpha_{k})^{\mathcal{T}-l-1}\mathbb{E}[\|x^{i}_{k,l} - \Bar{x}_{k}\|^{2}]\notag
\end{align}
Next, since $\alpha_{k} \leq 1$, it implies that $(1-\alpha_{k}) \leq 1$ and $(1-\alpha_{k})^{\mathcal{T}} \leq (1-\alpha_{k})$. Therefore we have the following
\begin{align}
    &\mathbb{E}[\|e^{i}_{k,\mathcal{T}}\|^{2}]\notag\\
    &\leq (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + \alpha_{k}L^{2}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|x^{i}_{k,l} - \Bar{x}_{k}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\mathcal{T}\notag
\end{align}
Further using the result from \eqref{eq:x_k_T_minus_bar_x_squared} we obtain the following
\begin{align}
    &\mathbb{E}[\|e^{i}_{k,\mathcal{T}}\|^{2}]\notag\\
    &\leq (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\mathcal{T}\notag\\
    &+ \alpha_{k}L^{2}\sum_{l=0}^{\mathcal{T}-1}\Big(2\beta^{2}_{k}L^{2}\mathcal{T}^{2}\mathbb{E}[\|\Bar{x}_{k} - x^{*}_{\mathcal{H}}\|^{2}] + 2\beta^{2}_{k}\mathcal{T}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\Big) \notag\\
    &= (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + 2\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{3}\mathbb{E}[V^{k}_{1}]+\alpha^{2}_{k}\sigma^{2}\mathcal{T}\notag\\
    &+2\alpha_{k}\beta_{k}^{2}L^{2}\mathcal{T}^{2}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag.
    \end{align}
Putting the above relation back in Eq. \eqref{eq:V_2_r0} and using the definition of the Lyapunov function for the average gradient error from Eq. \eqref{eq:V_2_def}, we have,
\begin{align}\label{eq:V_2_r1}
    &\mathbb{E}[V^{k+1}_{2}] \notag\\
    &\leq (1-\alpha_{k})\Big(1+\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}] + \frac{3L^{2}}{\alpha_{k}|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|\Bar{x}_{k+1} - \Bar{x}_{k}\|^{2}]\notag\\
    &+ 2\alpha_{k}\Big(1+\frac{\alpha_{k}}{2}\Big)\beta^{2}_{k}L^{4}\mathcal{T}^{3}\mathbb{E}[V^{k}_{1}] + \alpha_{k}^{2}\Big(1+\frac{\alpha_{k}}{2}\Big)\sigma^{2}\mathcal{T}\notag\\
    &+\frac{2\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}}{|\mathcal{H}|}\Big(1+\frac{\alpha_{k}}{2}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}] 
\end{align}
Here since $\alpha_{k} \leq 1$, we have the following relations
\begin{align*}
    &\Big(1+\frac{\alpha_{k}}{2}\Big) \leq \frac{3}{2} \ \text{and} \ (1-\alpha_{k})\Big(1+\frac{\alpha_{k}}{2}\Big) \leq 1-\frac{\alpha_{k}}{2}
\end{align*}
using which we get
\begin{align}\label{eq:V_k_2}
     &\mathbb{E}[V^{k+1}_{2}] \leq \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}] + 3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{3}\mathbb{E}[V^{k}_{1}]\notag\\
    & +\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]+ \frac{3\alpha_{k}^{2}\sigma^{2}\mathcal{T}}{2}\notag\\
    & + \frac{3L^{2}}{\alpha_{k}|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|\Bar{x}_{k+1} - \Bar{x}_{k}\|^{2}]
\end{align}
Finally we analyze the last term in the right hand side of the above inequality. For this we observe that from Eq. \eqref{eq:x_bar_update} using the inequality $\|a+b\|^{2} \leq 2\|a\|^{2}+\|b\|^{2}$ for any two vectors $a,b$, we have
\begin{align}
    &\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}\notag\\
    &= \Big\|\mathcal{E}_{k}-\mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\Bar{x}_{k})-\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big\|^{2}\notag\\
    & \leq 2\|\mathcal{E}_{x}\|^{2} + 2\Big\|\mathcal{T}\beta_{k}(\nabla q^{\mathcal{H}}(\Bar{x}_{k})-\nabla q^{\mathcal{H}}(x^{*}_{\mathcal{H}}))+\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big\|^{2}\notag.
\end{align}
Using the Lipschitz continuity of \( \nabla q^{\mathcal{H}} \) and noting that \( x^{*}_{\mathcal{H}} \) is the minimizer of \( q^{\mathcal{H}}(\bar{x}_{k}) \), implying \( \nabla q^{\mathcal{H}}(x^{*}_{\mathcal{H}}) = 0 \), we have
\begin{align}\label{eq:diff_x_k}
     &\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}\notag\\
    &\leq 2\|\mathcal{E}_{x}\|^{2} + 4\beta^{2}_{k}\mathcal{T}^{2}L^{2}\|\Bar{x}_{k} - x^{*}_{\mathcal{H}}\|^{2} + \frac{4\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}
\end{align}
Next, we further analyze the term $\|\mathcal{E }_{x}\|^{2}$ from \eqref{eq:V_x_update_0}. For this for some agent $j \in \mathcal{H}$ using \eqref{eq:e_k_t_iteration} we get
\begin{align}
    &\mathbb{E}[\|\mathcal{E}_{x}\|^{2}] \notag\\
    &\leq \frac{8\beta^{2}_{k}\mathcal{T}^{2}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\frac{4\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{l=0}^{\mathcal{T}-1}\Big[(1-\alpha_{k})^{l}\mathbb{E}[\|e^{j}_{k,0}\|^{2}] \notag\\
    &\hspace{2cm}+ \alpha_{k}L^{2}\sum_{l'=0}^{l-1}\mathbb{E}[\|x^{j}_{k,l'} - \Bar{x}_{k}\|^{2}] + \alpha^{2}_{k}\sigma^{2}l\Big] \notag\\
    &+ \frac{4\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i\in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\Big[(1-\alpha_{k})^{t}\mathbb{E}[\|e^{i}_{k,0}\|^{2}]\notag\\
    &\hspace{2cm}+ \alpha_{k}L^{2}\sum_{l'=0}^{l-1}\mathbb{E}[\|x^{i}_{k,l'} - \Bar{x}_{k}\|^{2}]+ \alpha^{2}_{k}\sigma^{2}l\Big] \notag\\
\end{align}
Since \( \alpha_{k} \leq 1 \), it follows that \( (1-\alpha_{k})^{t} \leq 1 \). Additionally, for any agent $j \in \mathcal{H}$ we use the following 
\begin{align*}
    &\sum_{l=0}^{\mathcal{T}-1}\|e^{j}_{k,0}\|^{2} \leq \sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2},\notag\\
    &\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,0}\|^{2} \leq \sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2},\notag
\end{align*} using which we have
\begin{align}\label{eq:V_x_update_2}
    &\mathbb{E}[\|\mathcal{E}_x\|^{2}]\notag\\
    &\leq \frac{8\beta^{2}_{k}\mathcal{T}^{2}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+\frac{8\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
    &+\frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\mathbb{E}[\|x^{j}_{k,l'} - \Bar{x}_{k}\|^{2}]\notag\\
    &+\frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i\in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\mathbb{E}[\|x^{i}_{k,l'} - \Bar{x}_{k}\|^{2}]\notag\\
    &+\frac{8\alpha^{2}_{k}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
\end{align}
Next using \eqref{eq:x_k_T_minus_bar_x_squared} we analyze the third last term in the right hand side of the above inequality as
\begin{align}\label{eq:V_x_term_3}
    &\frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\mathbb{E}[\|x^{j}_{k,l'} - \Bar{x}_{k}\|^{2}]\notag\\
    &\leq \frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\Big( 2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\Big)\notag\\
    & \leq \frac{8\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[V^{k}_{1}] \notag\\
    &\hspace{2cm}+ \frac{8\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{l= 0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
\end{align}
Similarly, using \eqref{eq:x_k_T_minus_bar_x_squared} the third last term in the right-hand side of \eqref{eq:V_x_update_2} can expressed as
\begin{align}\label{eq:V_x_term_2}
    &\frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\mathbb{E}[\|x^{j}_{k,l'} - \Bar{x}_{k}\|^{2}]\notag\\
    &\leq \frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\Big( 2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\Big)\notag\\
    & \leq\frac{8\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[V^{k}_{1}] \notag\\
    &\hspace{2cm}+ \frac{8\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{l= 0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
\end{align}
Thus, using the results of \eqref{eq:V_x_term_3} and \eqref{eq:V_x_term_2}, then \eqref{eq:V_x_update_2} can be expressed as
\begin{align}\label{eq:V_x_update_latest}
    &\mathbb{E}[\|\mathcal{E}_x\|^{2}] \leq \Big(\frac{8\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} + \frac{16\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+ \Big(\frac{8\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} + \frac{16\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+\frac{8\alpha^{2}_{k}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
\end{align}
Putting back the above result in \eqref{eq:diff_x_k} we have 
\begin{align}\label{eq:diff_x_k_update}
    &\mathbb{E}[\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}] \notag\\
    &\leq \Big(4\beta^{2}_{k}L^{2}\mathcal{T}^{2} + \frac{16\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} + \frac{32\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+ \Big(\frac{4\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}+\frac{16\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} \Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \frac{32\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]+\frac{16\alpha^{2}_{k}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}
\end{align}
Further putting the above result back in \eqref{eq:V_k_2} we get
\begin{align}
     &\mathbb{E}[V^{k+1}_{2}] \notag\\
     &\leq \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}] + 3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{4}\mathbb{E}[V^{k}_{1}]\notag\\
    & +\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]+ \frac{3\alpha_{k}^{2}\sigma^{2}\mathcal{T}^{2}}{2}\notag\\
    & + \frac{3L^{2}}{\alpha_{k}|\mathcal{H}|}\sum_{i \in \mathcal{H}}\Big[\Big(4\beta^{2}_{k}L^{2}\mathcal{T}^{2} + \frac{16\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+ \frac{32\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{4\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}+\frac{16\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} \Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \frac{32\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\Big]\notag\\
    & +\frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}, \notag
\end{align}
which upon simplification gives us the following
\begin{align}
    &\mathbb{E}[V^{k+1}_{2}]\notag\\
    &\leq \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}] + \Big(3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}+\frac{12\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\alpha_{k}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{48\beta^{2}_{k}L^{4}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}}+\frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{6}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+ \Big(\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{12\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{\alpha_{k}|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \Big(\frac{48\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}} + \frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.\notag
\end{align}
Hence proved.
\end{proof}


==> Lemma3.tex <==
\section{Lemma \ref{lem:Lemma_V1_PL}}`
Using Assumption \eqref{eq:Assump_1} we have
\begin{align}\label{eq:diff_q_h_0}
    &\nabla q^{\mathcal{H}}(\Bar{x}_{k+1})- \nabla q^{\mathcal{H}}(\Bar{x}_{k})\notag\\
    &\leq \underbrace{\nabla q^{\mathcal{H}}(\Bar{x}_{k})^{T}(\Bar{x}_{k+1}-\Bar{x}_{k})}_{A} + \underbrace{\frac{L}{2}\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}}_{B}.
\end{align}
Using \eqref{eq:x_bar_update}, we analyze term A in the above equation as the following
\begin{align}\label{eq:diff_q_h_0_termA}
    &\nabla q^{\mathcal{H}}(\Bar{x}_{k})^{T}(\Bar{x}_{k+1}-\Bar{x}_{k})\notag\\
    &= -\mathcal{T}\beta_{k}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} -\frac{\beta_{k}}{|\mathcal{H}|}\nabla q^{\mathcal{H}}(\Bar{x}_{k})^{T}\Big(\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}e^{i}_{k,t}\Big) \notag\\
    &\hspace{5cm}+ V_{x}^{T}\nabla q^{\mathcal{H}}(\Bar{x}_{k})
\end{align}
Analyzing the second term in the right-hand side of the above equation we have
\begin{align}\label{eq:TermA_subterm2}
    &-\frac{\beta_{k}}{|\mathcal{H}|}\nabla q^{\mathcal{H}}(\Bar{x}_{k})^{T}\Big(\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}e^{i}_{k,t}\Big) \notag\\
    & \leq \frac{\beta_{k}}{|\mathcal{H}|}\Bigg[\frac{L\mathcal{T}|\mathcal{B}_{k}|}{2\mu}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} + \frac{\mu}{2L|\mathcal{B}_{k}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2}\Bigg]\notag\\
    & =\frac{\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{2\mu|\mathcal{H}|}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} + \frac{\mu\beta_{k}}{2L}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2}
\end{align}
Next for our analysis using \eqref{eq:V_x} we notice the following
\begin{align}\label{eq:V_x_update_order_one}
  \|V_x\| \leq \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{B}_{k}}\|x^{i}_{k,\mathcal{T}}-\Bar{x}_{k}\| + \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H} \backslash  \mathcal{H}_{k}}\|x^{i}_{k,\mathcal{T}}-\Bar{x}_{k}\|,  \notag
\end{align}
using which, and noting that an agent $j \in \mathcal{H}$ such that $\|x^{i}_{k,\mathcal{T}}-\Bar{x}_{k}\| \leq \|x^{j}_{k,\mathcal{T}}-\Bar{x}_{k}\|$ for all $i \in \mathcal{B}_{k}$ we have 
\begin{align}
    &\|V_{x}\| \leq \frac{|\mathcal{B}_{k}|}{|\mathcal{H}|}\|x^{j}_{k,\mathcal{T}}-\Bar{x}_{k}\| + \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H} \backslash \mathcal{H}_{k}}\|x^{i}_{k,\mathcal{T}}-\Bar{x}_{k}\| \notag\\
    & \overset{\eqref{eq:x_update_T}}{\leq} \frac{\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|}\sum_{t=0}^{\mathcal{T}-1}\|e^{j}_{k,t}\| + \frac{\beta_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}\|\nabla q^{j}(\Bar{x}_{k})-\nabla q^{j}(x^{*}_{\mathcal{H}})\|\notag\\
    &+\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}\backslash \mathcal{H}_{k}}\Big(\beta_{k}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\| + \beta_{k}\mathcal{T}\|\nabla q^{i}(\Bar{x}_{k})-\nabla q^{i}(x^{*}_{\mathcal{H}})\|\Big)\notag\\
    & \overset{\eqref{eq:Assump_3}}{\leq} \frac{2\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{\mu|\mathcal{H}|}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\| + \frac{\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|}\sum_{t=0}^{\mathcal{T}-1}\|e^{j}_{k,t}\|\notag\\
    &+ \frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|
\end{align}
Using the above relation we analyze the last term in the right-hand side of the Eq. \ref{eq:diff_q_h_0}
\begin{align}\label{eq:TermA_subterm3}
    &V_{x}^{T}\nabla q^{\mathcal{H}}(\Bar{x}_{k})\notag\\
    & \leq \|V_{x}\|\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|\notag\\
    & \leq \frac{2\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{\mu|\mathcal{H}|}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} + \frac{\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|}\sum_{t=0}^{\mathcal{T}-1}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|\|e^{j}_{k,t}\|\notag\\
    &+ \frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{t=0}^{\mathcal{T}-1}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|\|e^{i}_{k,t}\|\notag\\
    & \leq \frac{2\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{\mu|\mathcal{H}|}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}\notag\\
    &+ \frac{\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|}\sum_{t=0}^{\mathcal{T}-1}\Big(\frac{L}{8\mu}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} + \frac{2\mu}{L}\|e^{j}_{k,t}\|^{2}\Big)\notag\\
    &+ \frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{t=0}^{\mathcal{T}-1}\Big(\frac{L}{8\mu}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} + \frac{2\mu}{L}\|e^{i}_{k,t}\|^{2}\Big)\notag\\
    &=\frac{9\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{4\mu|\mathcal{H}|}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} + \frac{2\mu\beta_{k}|\mathcal{B}_{k}|}{L|\mathcal{H}|}\sum_{t=0}^{\mathcal{T}-1}\|e^{j}_{k,t}\|^{2}\notag\\
    &+ \frac{2\beta_{k}\mu}{L|\mathcal{H}|}\sum_{i \in \mathcal{H}\backslash \mathcal{H}_{k}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2}\notag\\
    & \overset{\eqref{eq:e_k_t_relations}}{\leq} \frac{9\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{4\mu|\mathcal{H}|}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} + \frac{4\mu\beta_{k}|\mathcal{B}_{k}|}{L|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|e^{j}_{k,t}\|^{2}
\end{align}
Putting back results from \eqref{eq:TermA_subterm2} and \eqref{eq:TermA_subterm3} back into Eq. \eqref{eq:diff_q_h_0_term1} we have
\begin{align}\label{eq:V_1_TermA}
    &\nabla q^{\mathcal{H}}(\Bar{x}_{k})^{T}(\Bar{x}_{k+1}-\Bar{x}_{k})\notag\\
    & \leq \Big(-\mathcal{T}\beta_{k}+\frac{11\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{4\mu|\mathcal{H}|}\Big)\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}\notag\\
    &\hspace{2cm}+ \Big(\frac{\mu\beta_{k}}{2L} + \frac{4\mu\beta_{k}|\mathcal{B}_{k}|}{L|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2}.
\end{align}
Next, by analyzing the term B from Eq. \eqref{eq:diff_q_h_0} using \eqref{eq:x_update_T}, we note the following
\begin{align}\label{eq:diff_q_h_0_termB}
    &\frac{L}{2}\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2} \leq \frac{\beta^{2}_{k}L\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|y^{i}_{k,t}\|^{2} + L\|V_{x}\|^{2}\notag\\
    &\leq \frac{\beta^{2}_{k}L\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\Big( 2L^{2}\|\Bar{x}_{k}-x^{*}\|^{2}+2\|e^{i}_{k,t}\|^{2}\Big) + L\|V_{x}\|^{2}\notag\\
    &\leq \frac{2L^{3}\beta^{2}_{k}\mathcal{T}^{2}}{\mu^{2}}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} + \frac{2\beta^{2}_{k}L\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2} + L\|V_{x}\|^{2}\notag\\
    &\overset{\eqref{eq:V_x_update},\eqref{eq:Assump_3}}{\leq}\frac{2L^{3}\mathcal{T}^{2}\beta^{2}_{k}}{\mu^{2}}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} + \frac{2\beta^{2}_{k}L\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2} \notag\\
    &+ \frac{8L^{3}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{\mu^{2}|\mathcal{H}|^{2}}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} + \frac{4\beta^{2}_{k}\mathcal{T}L|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{t=0}^{\mathcal{T}-1}\|e^{j}_{k,t}\|^{2}\notag\\
    &+\frac{4\beta^{2}_{k}L\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2}\notag\\
    &\overset{\eqref{eq:e_k_t_relations}}{\leq} \Big(\frac{2L^{3}\mathcal{T}^{2}\beta^{2}_{k}}{\mu^{2}}+\frac{8L^{3}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{\mu^{2}|\mathcal{H}|^{2}}\Big)\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}\notag\\
    &+\Big(\frac{2\beta^{2}_{k}L\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{8\beta^{2}_{k}L\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2}.
\end{align}
Finally, putting back the results from \eqref{eq:diff_q_h_0_termA} and \eqref{eq:diff_q_h_0_termB} back into Eq. \eqref{eq:diff_q_h_0} we have the following
\begin{align}\label{eq:diff_q_h_0_final}
    &\mathbb{E}[\nabla q^{\mathcal{H}}(\Bar{x}_{k+1})-\nabla q^{\mathcal{H}}(\Bar{x}_{k})]\notag\\
    &\leq \Big(\frac{11\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{4\mu|\mathcal{H}|} + \frac{2L^{3}\mathcal{T}^{2}\beta^{2}_{k}}{\mu^{2}} + \frac{8L^{3}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{\mu^{2}|\mathcal{H}|^{2}}\Big)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
    &+\Big(\frac{\mu\beta_{k}}{2L} + \frac{4\mu\beta_{k}|\mathcal{B}_{k}|}{L|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2}\notag\\
    &+\Big(\frac{2\beta^{2}_{k}L\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{8\beta^{2}_{k}L\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2}
\end{align}

==> Lemma4.tex <==
\section{Lemma \ref{lem:Lemma_V2_SC}}

==> LemmaTheorems.tex <==
\section{Main Results}

\input{main files/main-lemmas}

\subsection{Strongly convex condition}
In this section we will present our result in the scenario where we assume the average
non-faulty cost function, denoted by $q^{\mathcal{H}}(x)$, to be strongly convex satisfying the following assumption.
\begin{assumption}\label{eq:Assumption_strong_convexity}
The objective function $q^{\mathcal{H}}(.)$ is strongly convex.
\begin{align}\label{eq:sc_condition}
    (y-x)^{T}(\nabla q^{\mathcal{H}}(y) - \nabla q^{\mathcal{H}}(x)) \geq \mu \|y-x\|^{2}, \ \forall x,y \in \mathbb{R}^{d}.
\end{align}
\end{assumption}
\begin{remark}
This assumption does not imply that each local functions necessarily are strongly convex satisfy PL condition in the above cases. However, under $2-f$ redundancy condition one can show that 
\begin{align}
    x^{*}_{\mathcal{H}} \in \bigcap \limits_{i\in \mathcal{H}} \arg \min_{x\in \mathbb{R}^{d}} q^{i}(x)
\end{align}
For detailed proof see Lemma $1$ in \cite{gupta2020fault}. Thus, Algorithm \ref{alg:cap} aims to find a point in the intersection of the minimizer sets of the local functions $q^{i}$.
\end{remark}
Here we define the lypunov function for the optimality gap be given by
\begin{align}
    V^{1}_{k} = \|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}
\end{align}
where $\Bar{x}_{k}$ be defined as in line $15$ in Algorithm \ref{alg:cap}. Further we define the lyapunov function for the cumulative gradient error given by
\begin{align}
    V^{k}_{2} = \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}
\end{align}
where $e^{i}_{k,t}$ be the gradient error as defined in \eqref{eq:e_k_t}.
\begin{lemma}
    Let $e^{i}_{k,t}$ be defied as in \eqref{eq:e_k_t} and let the step size $\alpha_{k}$ satisfy
    \begin{align}
        \alpha_{k} \leq \frac{1}{2L\mathcal{T}}
    \end{align}
    then the following holds
    \begin{align}
        &\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] \notag\\
        &\leq 2\mathcal{T}\mathbb{E}[V^{k}_{2}] + 4\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{3}\mathbb{E}[V^{k}_{1}] + 2\alpha^{2}_{k}\sigma^{2}\mathcal{T}.
    \end{align}
\end{lemma}
\begin{proof}
    From Lemma \ref{lem:e_k_t} we have
    \begin{align}
        &\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
        &\leq (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,l-1}\|^{2}] + \alpha_{k}L^{2}\mathbb{E}[\|x^{i}_{k,l-1}-\bar{x}_{k}\|^{2}] + \alpha^{2}\sigma^{2}\notag\\
        &\leq (1-\alpha)^{l}\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + \alpha_{k}L^{2}\sum_{l'=0}^{l-1}(1-\alpha_{k})^{l-l'-1}\mathbb{E}[\|x^{i}_{k,l'}-\bar{x}_{k}\|^{2}] \notag\\
        &\hspace{2cm}+ \alpha_{k}\sigma^{2}\sum_{l'=0}^{l-1}(1-\alpha_{k})^{l'}.
    \end{align}
    Here, note that since \(\alpha_k \leq 1\), it follows that \((1 - \alpha_k) \leq 1\), which further implies \((1 - \alpha_k)^l \leq (1 - \alpha_k)\). Utilizing this and result from Lemma \ref{lem:x_k_t_minus_x_bar_squared}, we have
    \begin{align}
        &\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
        &\leq (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + \alpha_{k}L^{2}\sum_{l'=0}^{l-1}\mathbb{E}[\|x^{i}_{k,l'}-\bar{x}_{k}\|^{2}] + \alpha^{2}_{k}\sigma^{2}l\notag\\
        &\leq (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + \alpha^{2}_{k}\sigma^{2}l\notag\\
        &+\alpha_{k}L^{2}\sum_{l'=0}^{l-1}\Big(2L^{2}\mathcal{T}^{2}\beta^{2}_{k}\mathbb{E}[\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + 2\mathcal{T}\beta^{2}_{k}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\Big)\notag\\
        & = (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + 2\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}l\mathbb{E}[\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
        &\hspace{2cm}+ 2\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}l\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] + \alpha^{2}_{k}\sigma^{2}l,\notag
    \end{align}
    using which we have 
    \begin{align}
        &\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] \notag\\
        &\leq \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}(1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}l\notag\\
        &\hspace{2cm}+ 2\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
        &\hspace{2cm}+ 2\alpha^{2}_{k}\beta^{2}_{k}L^{2}\mathcal{T}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}l\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
        &=\mathcal{T}\mathbb{E}[V^{k}_{2}] + 2\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{3}\mathbb{E}[V^{k}_{1}]\notag\\
        & \hspace{1cm}+ 2\alpha^{2}_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}\frac{1}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\mathcal{T}.
    \end{align}
    Next, since \(\beta_k \leq \alpha_k \leq 1\), which implies \(\alpha_k^2 \beta_k^2 \leq \alpha_k^2\), we have
    \begin{align}
        &(1-2\alpha^{2}_{k}L^{2}\mathcal{T}^{2})\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] \notag\\
        &\leq \mathcal{T}\mathbb{E}[V^{k}_{2}] + 2\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{3}\mathbb{E}[V^{k}_{1}] + \alpha^{2}\sigma^{2}\mathcal{T}.\notag
    \end{align}
    Here we note tahr since $\alpha_{k} \leq \frac{1}{L\mathcal{T}}$ we have $1-2\alpha^{2}_{k}L^{2}\mathcal{T}^{2} \geq 0$. Thus dividing both sides of the above inequality by $1-2\alpha^{2}_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}$ we have
    \begin{align*}
         &\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] \notag\\
        &\leq \frac{\mathcal{T}\mathbb{E}[V^{k}_{2}]}{1-2\alpha^{2}_{k}L^{2}\mathcal{T}^{2}} + \frac{2\alpha_{k}\beta^{2}_{k}L^{4}}{1-2\alpha^{2}_{k}L^{2}\mathcal{T}^{2}}\mathbb{E}[V^{k}_{2}]\mathcal{T}^{3}\mathbb{E}[V^{k}_{1}] \notag\\
        & \hspace{2cm}+\frac{\alpha^{2}\sigma^{2}\mathcal{T}}{1-2\alpha_{k}\beta^{2}_{k}L^{2}}.
    \end{align*}
    Further note  that \(\alpha_k \leq \frac{1}{2L\mathcal{T}}\) implies \(\frac{1}{1 - 2\alpha_k^2 L^2 \mathcal{T}^2} \leq 2\), using which we have
    \begin{align}
        &\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
        & \leq 2\mathcal{T}\mathbb{E}[V^{k}_{2}] + 4\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{3}\mathbb{E}[V^{k}_{1}] + 2\alpha^{2}\sigma^{2}\mathcal{T}.
    \end{align}
\end{proof}
\begin{lemma}\label{lem:Lemma_V1_SC}
Let the lypunov function for the optimality gap be given by
\begin{align}
    V^{1}_{k} = \|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}
\end{align}
where $\Bar{x}_{k}$ be defined as in line $15$ in Algorithm \ref{alg:cap} then 
    \begin{align}
    &\mathbb{E}[V^{k+1}_{1}]\notag\\
    &\leq \Big(1-2\mu\beta_{k}\mathcal{T} + \frac{35L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}+L^{2}\mathcal{T}^{2}\beta^{2}_{k} \Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{16L^{2}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} + \frac{19L^{3}\mathcal{T}^{3}\beta^{3}_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{6\beta_{k}}{L} + \frac{8\beta_{k}|\mathcal{B}_{k}|}{3L|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+\Big(\frac{2\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{16\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}].
\end{align}
\end{lemma}
\tdoan{Present proof of this lemma here with \textbf{specific detail of every single step} in your analysis, i.e., deriving the bound of each term separately. The current version in the appendix is not good enough. Same for Lemma 7.}

\begin{proof}
Using the update equation from \eqref{eq:algo_update_Tg1} and the definition of $e^{i}_{k,t}$ from \eqref{eq:e_k_t} we have
\begin{align}\label{eq:x_update_error}
    x^{i}_{k,t+1} &= x^{i}_{k,t} - \beta_{k} y^{i}_{k,t} \notag\\
    & = \Bar{x}_{k} -\beta_{k}\sum_{l=0}^{t}y^{i}_{k,l}\notag\\
    & = \Bar{x}_{k} -\beta_{k}\sum_{l=0}^{t}e^{i}_{k,l} -\beta_{k}\sum_{l=0}^{t}\nabla q^{i}(\Bar{x}_{k}).
\end{align}
From which we have
\begin{align}\label{eq:x_update_T}
    x^{i}_{k,\mathcal{T}} = \Bar{x}_{k} -\beta_{k}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l} -\beta_{k}\sum_{l=0}^{\mathcal{T}-1}\nabla q^{i}(\bar{x}_{k}).
\end{align}
For our analysis, we first note that $|\mathcal{F}_{k}| = |\mathcal{H}|$ and $|\mathcal{B}_{k}| = |\mathcal{H}\backslash\mathcal{H}_{k}|$. Thus from line $15$ in Algorithm \ref{alg:cap} we have the following,
    \begin{align}
        \Bar{x}_{k+1}&=\frac{1}{|\mathcal{F}_{k}|}\sum_{i \in \mathcal{F}_{k}}x^{i}_{k,\mathcal{T}}\notag \\
        &=\frac{1}{|\mathcal{H}|}\Big[\sum_{i\in \mathcal{H}}x^{i}_{k,\mathcal{T}} + \sum_{i\in \mathcal{B}_{k}}x^{i}_{k,\mathcal{T}} - \sum_{i\in \mathcal{H} \backslash \mathcal{H}_{k}}x^{i}_{k,\mathcal{T}}\Big], \notag \\
        & = \frac{1}{|\mathcal{H}|} \sum_{i\in \mathcal{H}}x^{i}_{k,\mathcal{T}}  + \mathcal{E}_{x}.\notag
    \end{align}
    where 
    \begin{align}\label{eq:V_x}
        \mathcal{E}_{x} = \frac{1}{|\mathcal{H}|}\Big[\sum_{i\in \mathcal{B}_{k}}(x^{i}_{k,\mathcal{T}} -\Bar{x}_{k}) - \sum_{i\in \mathcal{H} \backslash \mathcal{H}_{k}}(x^{i}_{k,\mathcal{T}}-\Bar{x}_{k})\Big]
    \end{align}
    Here we note that the term $\mathcal{E}_{x}$ represents an error term that arises due to the presence of Byzantine agents. Next we use \eqref{eq:x_update_T} which gives us,
    \begin{align}
        \bar{x}_{k+1} &= \bar{x}_{k} - \frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}}\nabla q^{i}(\bar{x}_{k}) - \beta_{k}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l} + \mathcal{E}_{x}\notag.
    \end{align}
    Next using the definition of $q^{\mathcal{H}}(x)$ from \eqref{eq:avg_q_h} we obtain $\nabla q^{\mathcal{H}}(\bar{x}_{k}) = \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\nabla q^{i}(\bar{x}_{k})$, which leads to 
    \begin{align}\label{eq:x_bar_update}
        \Bar{x}_{k+1} = \Bar{x}_{k}-\mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\Bar{x}_{k})-\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}+ \mathcal{E}_{k},
    \end{align}
    using which we have
    \begin{align}\label{eq:x_bar_squared_update}
        &\|\Bar{x}_{k+1} -x^{*}_{\mathcal{H}}\|^{2}\notag \\
        &= \underbrace{\|\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\|^{2}}_{\text{Term 1}} + \underbrace{\Big\|\mathcal{E}_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big\|^{2}}_{\text{Term 2}} \notag\\
        &\underbrace{-2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\Big(\mathcal{E}_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big)}_{\text{Term 3}}.
    \end{align}
    First, we analyze Term 1 on the right-hand side of the equation above. Note that $x^{*}_{\mathcal{H}}$ is the minimizer of $q^{\mathcal{H}}(x)$ i.e $\nabla q^{\mathcal{H}}(x^{*}_{\mathcal{H}}) = 0$, using which we have
    \begin{align}
        &\|\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\|^{2}\notag\\
        &= \|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}-2\mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})^{T}(\bar{x}_{k}-x^{*}_{\mathcal{H}}) \notag\\
        &\hspace{2cm}+ \mathcal{T}^{2}\beta^{2}_{K}\|\nabla q^{\mathcal{H}}(\bar{x}_{k})\|^{2}\notag\\
         &= \|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}-2\mathcal{T}\beta_{k}(\nabla q^{\mathcal{H}}(\bar{x}_{k})-\nabla q^{\mathcal{H}}(x^{*}_{\mathcal{H}}))^{T}(\bar{x}_{k}-x^{*}_{\mathcal{H}}) \notag\\
        &\hspace{2cm}+ \mathcal{T}^{2}\beta^{2}_{K}\|\nabla q^{\mathcal{H}}(\bar{x}_{k})-\nabla q^{\mathcal{H}}(x^{*}_{\mathcal{H}})\|^{2}\notag.
    \end{align}
    Next using Lipschitz continuity of $\nabla q^{\mathcal{H}}$ from Assumption \ref{eq:Assumption_Lipschitz} and strong convexity of $q^{\mathcal{H}}$ from Assumption \ref{eq:Assumption_strong_convexity} we have 
    \begin{align*}
        &-(\nabla q^{\mathcal{H}}(\bar{x}_{k})-\nabla q^{\mathcal{H}}(x^{*}_{\mathcal{H}}))^{T}(\bar{x}_{k}-x^{*}_{\mathcal{H}}) \leq -\mu\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2},\notag\\
        &\|\nabla q^{\mathcal{H}}(\bar{x}_{k})-\nabla q^{\mathcal{H}}(x^{*}_{\mathcal{H}})\|^{2} \leq L^{2}\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2},
    \end{align*}
    using which we have
    \begin{align}\label{eq:x_bar_squared_update_Term_1}
         &\|\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\|^{2}\notag\\
         &\leq (1-2\mu\mathcal{T}\beta_{k} + L^{2}\mathcal{T}^{2}\beta^{2}_{k})\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}
    \end{align}
    Next we will analyze Term 2 in the right hand side of \eqref{eq:x_bar_squared_update}. Thus we have
    \begin{align}\label{eq:x_bar_squared_update_Term_2_v0}
        &\Big\|\mathcal{E}_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big\|^{2}\notag\\
        &\leq 2\|\mathcal{E}_{x}\|^{2}+ \frac{2\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}\notag\\
        &\leq 2\|\mathcal{E}_{x}\|^{2}+ \frac{2\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{K}|}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}.
    \end{align}
    Next we note that to analyze $\|\mathcal{E}_{x}\|^{2}$ we require to analyze $\|x^{i}_{k,\mathcal{T}}-\bar{x}_{k}\|^{2}$ term. For this, using the update for any honest agent $i \in \mathcal{H}$
\begin{align}
    x^{i}_{k,t+1} = x^{i}_{k,t}-\beta_{k}y^{i}_{k,t},\notag
\end{align}
we have 
\begin{align}
    \|x^{i}_{k,t+1}-\Bar{x}_{k}\|^{2} &= \Big\|\sum_{l=0}^{t}(x^{i}_{k,l+1}-x^{i}_{k,l})\Big\|^{2}\notag\\
    & \leq (t+1)\sum_{l=0}^{t}\|x^{i}_{k,l+1}-x^{i}_{k,l}\|^{2}\notag\\
    &= \beta_{k}^{2}(t+1)\sum_{l=0}^{t}\|y^{i}_{k,l}\|^{2}\notag.
\end{align}
Next using $y^{i}_{k,t} = e^{i}_{k,t} + \nabla q^{i}(\bar{x}_{k})$ which implies
\begin{align*}
    \|y^{i}_{k,t}\|^{2} \leq 2\|e^{i}_{k,t}\|^{2} + 2L^{2}\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2},
\end{align*}
we have 
\begin{align*}
    &\|x^{i}_{k,t+1}-\Bar{x}_{k}\|^{2}\notag\\
    &\leq 2L^{2}(t+1)^{2}\beta_{k}^{2}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + 2(t+1)\beta_{k}^{2}\sum_{l=0}^{t}\|e^{i}_{k,l}\|^{2},\notag
\end{align*}
which further gives us
\begin{align}\label{eq:x_k_T_minus_bar_x_squared}
    \|x^{i}_{k,\mathcal{T}}-\Bar{x}_{k}\|^{2}\leq 2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}.
\end{align}
Next, we analyze $\|\mathcal{E}_{x}\|^{2}$. Utilizing \eqref{eq:V_x} and the noting that there exists an agent $j \in \mathcal{H}$ such that $\|x^{i}_{k,t}-\Bar{x}_{k}\| \leq \|x^{j}_{k,t}-\Bar{x}_{k}\|$ for all agent $i \in \mathcal{B}_{k}$, we obtain 
\begin{align}\label{eq:V_x_update_0}
    \|\mathcal{E}_{x}\|^{2} &\leq \frac{2|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\|x^{j}_{k,\mathcal{T}} - \Bar{x}_{k}\|^{2} + \frac{2|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\|x^{i}_{k,\mathcal{T}} - \Bar{x}_{k}\|^{2} \notag\\
    & \leq \frac{2|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}(2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2})\notag\\
    &+ \frac{2|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}(2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2})\notag\\
    & \leq \frac{8L^{2}\mathcal{T}^{2}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + \frac{4\mathcal{T}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}\notag\\
    &+ \frac{4\mathcal{T}\beta_{k}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2},
\end{align}
which can be further simplified using 
\begin{align}\label{eq:e_k_t_relations}
    &\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} \leq \sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}, \notag\\
    &\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} \leq \sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2},
\end{align} thus obtaining the following,
\begin{align}\label{eq:V_x_update}
     &\|\mathcal{E}_{x}\|^{2}\notag\\
     &\leq \frac{8L^{2}\mathcal{T}^{2}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + \frac{8\mathcal{T}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}.
\end{align}
Putting this back in \eqref{eq:x_bar_squared_update_Term_2_v0}, term 2 on the right-hand side \eqref{eq:x_bar_squared_update} can be expressed as 
\begin{align}\label{eq:x_bar_squared_update_Term_2_final}
    &\Big\|\mathcal{E}_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big\|^{2}\notag\\
    &\leq \frac{16L^{2}\mathcal{T}^{2}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}\notag\\
    &\hspace{2cm}+ \Big(\frac{16\beta_{k}^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} + \frac{2\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}.
\end{align}
Next, from Term 3 in the right hand side of \eqref{eq:x_bar_update} we have 
\begin{align}\label{eq:x_bar_squared_update_Term_3_v0}
    &-2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\Big(\mathcal{E}_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big)\notag\\
    &= \underbrace{-2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\mathcal{E}_{x}}_{\text{Term 3a}}\notag\\
    &+\underbrace{2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\Big(\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big)}_{\text{Term 3b}}
\end{align}
To analyze Term 3a in the equation above, we apply the inequality \( 2a^{T}b \leq \eta\|a\|^{2} + \frac{\|b\|^{2}}{\eta} \) for any non-zero vectors \( a \) and \( b \), choosing \( \eta = \frac{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|} \). This gives us the following
\begin{align}
    &-2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\mathcal{E}_{x}\notag\\
    & \leq \frac{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|} \|\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\|^{2} + \frac{|\mathcal{H}|}{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}\|\mathcal{E}_{x}\|^{2}\notag\\
    \notag\\
    & \leq \frac{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|} (\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}+L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}) \notag\\
    &\hspace{6cm}+ \frac{|\mathcal{H}|}{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}\|\mathcal{E}_{x}\|^{2}\notag.
\end{align}
The last inequality is obtained using the strong convexity of $q^{\mathcal{H}}$ and Lipschitz continuity of $\nabla q^{\mathcal{H}}$. Next using \eqref{eq:V_x_update} Term 3a from \eqref{eq:x_bar_squared_update_Term_3_v0} becomes
\begin{align}\label{eq:x_bar_squared_update_Term_3a}
     &-2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\mathcal{E}_{x}\notag\\
     &\leq\frac{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|} (\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}+L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2})\notag\\
    &+\frac{8L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{3|\mathcal{H}|}\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}+\frac{8\beta_{k}|\mathcal{B}_{k}|}{3L|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}\notag\\
    &= \Big(\frac{17L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{3|\mathcal{H}|} + \frac{3L^{3}\mathcal{T}^{3}\beta^{3}_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|}\Big)\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}\notag\\
    &+ \frac{8\beta_{k}|\mathcal{B}_{k}|}{3L|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}
\end{align}
To analyze Term 3b in \eqref{eq:x_bar_squared_update_Term_3_v0}, we use the inequality \( 2a^{T}b \leq \eta\|a\|^{2} + \frac{\|b\|^{2}}{\eta} \) for any non-zero vectors \( a \) and \( b \), choosing \( \eta = \frac{L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|} \), which gives us
\begin{align}\label{eq:x_bar_squared_update_Term_3b}
    &2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\Big(\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big)\notag\\
    &\leq \frac{L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\|\bar{x}_{k}-x^{*}_{\mathcal{H}}-\mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\|^{2} + \frac{6\beta_{k}}{L}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}\notag\\
    &\leq \frac{L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}(\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + L^{2}\mathcal{T}^{2}\beta^{2}_{k}\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2})\notag\\
    &+ \frac{6\beta_{k}}{L}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}.
\end{align}
Putting back the results from \eqref{eq:x_bar_squared_update_Term_3a} and \eqref{eq:x_bar_squared_update_Term_3b} back into \eqref{eq:x_bar_squared_update_Term_3_v0}, Term 3 becomes
\begin{align}\label{eq:x_bar_squared_update_Term_3_final}
     &-2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\Big(\mathcal{E}_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big)\notag\\
     &\leq \Big(\frac{35L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|} + \frac{19L^{3}\mathcal{T}^{3}\beta^{3}_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\Big)\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}\notag\\
     &+\Big(\frac{6\beta_{k}}{L} + \frac{8\beta_{k}|\mathcal{B}_{k}|}{3|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}
\end{align}
Finally, substituting the results of Term 1, Term 2, and Term 3 from \eqref{eq:x_bar_squared_update_Term_1}, \eqref{eq:x_bar_squared_update_Term_2_final}, and \eqref{eq:x_bar_squared_update_Term_3_final}, respectively, into \eqref{eq:x_bar_squared_update}, we obtain
\begin{align}
    &\|\bar{x}_{k+1}-x^{*}_{\mathcal{H}}\|^{2}\notag\\
    &\leq \Big(1-2\mu\beta_{k}\mathcal{T} + \frac{35L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}+L^{2}\mathcal{T}^{2}\beta^{2}_{k} \Big)\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}\notag\\
    &+\Big(\frac{16L^{2}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} + \frac{19L^{3}\mathcal{T}^{3}\beta^{3}_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\Big)\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}\notag\\
    &+\Big(\frac{6\beta_{k}}{L} + \frac{8\beta_{k}|\mathcal{B}_{k}|}{3L|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}\notag\\
    &+\Big(\frac{2\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{16\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}\notag,
\end{align}
from which upon taking expectation on both the sides and using the definition $V^{k}_{1} = \|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}$ we obtain
\begin{align}
    &\mathbb{E}[V^{k+1}_{1}]\notag\\
    &\leq \Big(1-2\mu\beta_{k}\mathcal{T} + \frac{35L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}+L^{2}\mathcal{T}^{2}\beta^{2}_{k} \Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{16L^{2}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} + \frac{19L^{3}\mathcal{T}^{3}\beta^{3}_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{6\beta_{k}}{L} + \frac{8\beta_{k}|\mathcal{B}_{k}|}{3L|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+\Big(\frac{2\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{16\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag.
\end{align}
Hence proved.
\end{proof}



\begin{lemma}\label{lem:Lemma_V2_SC}
Let the lyapunov function for the cumulative gradient error be given by
\begin{align}\label{eq:V_2_def}
    V^{k}_{2} = \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}
\end{align}
where $e^{i}_{k,t}$ be the gradient error as defined in \eqref{eq:e_k_t}, then
    \begin{align}
          &\mathbb{E}[V^{k+1}_{2}]\notag\\
    &\leq \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}] + \Big(3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}+\frac{12\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\alpha_{k}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{48\beta^{2}_{k}L^{4}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}}+\frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{6}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+ \Big(\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{12\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{\alpha_{k}|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \Big(\frac{48\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}} + \frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
    \end{align}
\end{lemma}

\begin{proof}
Using the definition of $e^{i}_{k,t}$ from \eqref{eq:e_k_t} and since $y^{i}_{k+1,0} = y^{i}_{k,\mathcal{T}}$ we have,
\begin{align}
    e^{i}_{k+1,0} &= y^{i}_{k+1,0} - \nabla q^{i}(\Bar{x}_{k+1})\notag\\
    & = y^{i}_{k,\mathcal{T}}- \nabla q^{i}(\Bar{x}_{k+1})\notag\\
    & = e^{i}_{k,\mathcal{T}} + \nabla q^{i}(\Bar{x}_{k})-\nabla q^{i}(\Bar{x}_{k+1})
\end{align}
Next, applying the inequality $\|a + b\|^2 \leq (1+\eta)\|a\|^{2} + (1+\frac{1}{\eta})\|b\|^{2}$, with the choice of $\eta = \frac{\alpha_{k}}{2}$ we obtain,
\begin{align}
    &\|e^{i}_{k+1,0}\|^{2} \notag\\
    & \leq \Big(1+\frac{\alpha_{k}}{2}\Big)\|e^{i}_{k,\mathcal{T}}\|^{2} + \Big(1+\frac{2}{\alpha_{k}}\Big)\|\nabla q^{i}(\Bar{x}_{k}) - \nabla q^{i}(\Bar{x}_{k+1})\|^{2}\notag\\
    &\leq \Big(1+\frac{\alpha_{2}}{2}\Big)\|e^{i}_{k,\mathcal{T}}\|^{2} + \Big(1+\frac{2}{\alpha_{k}}\Big)L^{2}\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}\notag\\
    &\leq \Big(1+\frac{\alpha_{2}}{2}\Big)\|e^{i}_{k,\mathcal{T}}\|^{2} + \frac{3L^{2}}{\alpha_{k}}\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2},
\end{align}
% where the last inequality is obtained due to $\alpha_{k} \leq 1$ which leads to $\Big(1+\frac{2}{\alpha_{k}}\Big)L^{2} \leq \frac{3L^{2}}{\alpha_{k}}$. 
Thus we have
\begin{align}\label{eq:V_2_r0}
    &\mathbb{E}[V^{k+1}_{2}] = \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|e^{i}_{k+1,0}\|^{2}]\notag\\
    &\leq \Big(1+\frac{\alpha_{k}}{2}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|e^{i}_{k,\mathcal{T}}\|^{2}] + \frac{3L^{2}}{\alpha_{k}|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|\Bar{x}_{k+1} - \Bar{x}_{k}\|^{2}]
\end{align}
Next we analyze the first term in the right hand side of the above inequality. Using \eqref{eq:e_k_t} we have 
\begin{align}
    &e^{i}_{k,t+1}\notag\\
    &= y^{i}_{k,t+1} - \nabla q^{i}(\Bar{x}_{k})\notag\\
    & = (1-\alpha_{k})y^{i}_{k,t} + \alpha_{k}\nabla Q^{i}(x^{i}_{k,t};\Delta^{i}_{k,t}) - \nabla q^{i}(\Bar{x}_{k})\notag\\
    & = (1-\alpha_{k})e^{i}_{k,t}  + \alpha_{k}\nabla Q^{i}(x^{i}_{k,t};\Delta^{i}_{k,t}) - \nabla q^{i}(\Bar{x}_{k})\notag\\
    &+ (1-\alpha_{k})\nabla q^{i}(\Bar{x}_{k})\notag\\
    & = (1-\alpha_{k})e^{i}_{k,t} + \alpha_{k}(\nabla Q^{i}(x^{i}_{k,t},\Delta^{i}_{k,t}) - \nabla q^{i}(x^{i}_{k,t}))\notag\\
    &+\alpha_{k}(\nabla q^{i}(x^{i}_{k,t})-\nabla q^{i}(\Bar{x}_{k}))
\end{align}
Next squaring both sides of the above equation and taking conditional expectation with respect to the filtration $\mathcal{P}_{k,t}$ we have
\begin{align}
    &\mathbb{E}[\|e^{i}_{k,t+1}\|^{2}|\mathcal{P}_{k,t}]\notag\\
    &= (1-\alpha_{k})^{2}\|e^{i}_{k,t}\|^{2} + \alpha^{2}_{k}\|\nabla q^{i}(x^{i}_{k,t})-\nabla q^{i}(\Bar{x}_{k})\|^{2}\notag\\
    &+ \alpha^{2}_{k}\mathbb{E}[\|\nabla Q^{i}(x^{i}_{k,t},\Delta^{i}_{k,t}) - \nabla q^{i}(x^{i}_{k,t})\|^{2}]\notag\\
    &+ 2\alpha_{k}(1-\alpha_{k})(\nabla q^{i}(x^{i}_{k,t})-\nabla q^{i}(\Bar{x}_{k}))^{T}e^{i}_{k,t}\notag\\
    & + 2\alpha_{k}(1-\alpha_{k})\mathbb{E}[(\nabla Q^{i}(x^{i}_{k,t},\Delta^{i}_{k,t}) - \nabla q^{i}(x^{i}_{k,t}))^{T}e^{i}_{k,t}|\mathcal{P}_{k,t}]\notag\\
    &+2\alpha^{2}_{k}\mathbb{E}[(\nabla Q^{i}(x^{i}_{k,t},\Delta^{i}_{k,t}) - \nabla q^{i}(x^{i}_{k,t}))^{T}(\nabla q^{i}(x^{i}_{k,t})-\nabla q^{i}(\Bar{x}_{k})|\mathcal{P}_{k,t}]\notag
\end{align}
Due to the unbiased estimates of the gradients as indicated by \eqref{eq:sigma}, the second last term and the last term of the above equation is zero. Further due to the bounded variance of the stochastic gradients and Lipschitz continuity of $\nabla q^{\mathcal{H}}$ we have
\begin{align}
    &\mathbb{E}[\|e^{i}_{k,t+1}\|^{2}] \leq (1-\alpha_{k})^{2}\mathbb{E}[\|e^{i}_{k,t}\|^{2}] + \alpha^{2}_{k}L^{2}\mathbb{E}[\|x^{i}_{k,t} - \Bar{x}_{k}\|^{2}] \notag\\
    & + \alpha^{2}_{k}\sigma^{2}+ 2\alpha_{k}(1-\alpha_{k})\mathbb{E}[(\nabla q^{i}(x^{i}_{k,t}) - \nabla q^{i}(\Bar{x}_{k}))^{T}e^{i}_{k,t}]\notag
\end{align}
Next using the inequality $2a^{T}b \leq \|a\|^{2} + \|b\|^{2}$ for vectors $a$ and $b$ along with the Lipschiz continuity of $\nabla q^{i}$ we analyze the last term of the above equation as the following
\begin{align}\label{eq:e_k_t_iteration}
    &\mathbb{E}[\|e^{i}_{k,t+1}\|^{2}] \notag\\
    &\leq (1-\alpha_{k})^{2}\mathbb{E}[\|e^{i}_{k,t}\|^{2}] + \alpha^{2}_{k}L^{2}\mathbb{E}[\|x^{i}_{k,t} - \Bar{x}_{k}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\notag\\
    & + \alpha_{k}(1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,t}\|^{2}]+ \alpha_{k}(1-\alpha_{k})L^{2}\mathbb{E}[\|x^{i}_{k,t}-\Bar{x}_{k}\|^{2}]\notag\\
    & = (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,t}\|^{2}] + \alpha_{k}L^{2}\mathbb{E}[\|x^{i}_{k,t} - \Bar{x}_{k`}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\notag\\
    & \leq (1-\alpha_{k})^{t+1}\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\sum_{l=0}^{t}(1-\alpha_{k})^{l} \notag\\
    & + \alpha_{k}L^{2}\sum_{l=0}^{t}(1-\alpha_{k})^{t-l}\mathbb{E}[\|x^{i}_{k,l} - \Bar{x}_{k}\|^{2}],
\end{align}
which gives us 
\begin{align}
    &\mathbb{E}[\|e^{i}_{k,\mathcal{T}}\|^{2}]\notag\\
    &\leq (1-\alpha_{k})^{\mathcal{T}}\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + + \alpha^{2}_{k}\sigma^{2}\sum_{l=0}^{\mathcal{T}-1}(1-\alpha_{k})^{l} \notag\\
    &+ \alpha_{k}L^{2}\sum_{l=0}^{\mathcal{T}-1}(1-\alpha_{k})^{\mathcal{T}-l-1}\mathbb{E}[\|x^{i}_{k,l} - \Bar{x}_{k}\|^{2}]\notag
\end{align}
Next, since $\alpha_{k} \leq 1$, it implies that $(1-\alpha_{k}) \leq 1$ and $(1-\alpha_{k})^{\mathcal{T}} \leq (1-\alpha_{k})$. Therefore we have the following
\begin{align}
    &\mathbb{E}[\|e^{i}_{k,\mathcal{T}}\|^{2}]\notag\\
    &\leq (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + \alpha_{k}L^{2}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|x^{i}_{k,l} - \Bar{x}_{k}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\mathcal{T}\notag
\end{align}
Further using the result from \eqref{eq:x_k_T_minus_bar_x_squared} we obtain the following
\begin{align}
    &\mathbb{E}[\|e^{i}_{k,\mathcal{T}}\|^{2}]\notag\\
    &\leq (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + \alpha^{2}_{k}\sigma^{2}\mathcal{T}\notag\\
    &+ \alpha_{k}L^{2}\sum_{l=0}^{\mathcal{T}-1}\Big(2\beta^{2}_{k}L^{2}\mathcal{T}^{2}\mathbb{E}[\|\Bar{x}_{k} - x^{*}_{\mathcal{H}}\|^{2}] + 2\beta^{2}_{k}\mathcal{T}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\Big) \notag\\
    &= (1-\alpha_{k})\mathbb{E}[\|e^{i}_{k,0}\|^{2}] + 2\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{3}\mathbb{E}[V^{k}_{1}]+\alpha^{2}_{k}\sigma^{2}\mathcal{T}\notag\\
    &+2\alpha_{k}\beta_{k}^{2}L^{2}\mathcal{T}^{2}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag.
    \end{align}
Putting the above relation back in Eq. \eqref{eq:V_2_r0} and using the definition of the Lyapunov function for the average gradient error from Eq. \eqref{eq:V_2_def}, we have,
\begin{align}\label{eq:V_2_r1}
    &\mathbb{E}[V^{k+1}_{2}] \notag\\
    &\leq (1-\alpha_{k})\Big(1+\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}] + \frac{3L^{2}}{\alpha_{k}|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|\Bar{x}_{k+1} - \Bar{x}_{k}\|^{2}]\notag\\
    &+ 2\alpha_{k}\Big(1+\frac{\alpha_{k}}{2}\Big)\beta^{2}_{k}L^{4}\mathcal{T}^{3}\mathbb{E}[V^{k}_{1}] + \alpha_{k}^{2}\Big(1+\frac{\alpha_{k}}{2}\Big)\sigma^{2}\mathcal{T}\notag\\
    &+\frac{2\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}}{|\mathcal{H}|}\Big(1+\frac{\alpha_{k}}{2}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}] 
\end{align}
Here since $\alpha_{k} \leq 1$, we have the following relations
\begin{align*}
    &\Big(1+\frac{\alpha_{k}}{2}\Big) \leq \frac{3}{2} \ \text{and} \ (1-\alpha_{k})\Big(1+\frac{\alpha_{k}}{2}\Big) \leq 1-\frac{\alpha_{k}}{2}
\end{align*}
using which we get
\begin{align}\label{eq:V_k_2}
     &\mathbb{E}[V^{k+1}_{2}] \leq \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}] + 3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{3}\mathbb{E}[V^{k}_{1}]\notag\\
    & +\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]+ \frac{3\alpha_{k}^{2}\sigma^{2}\mathcal{T}}{2}\notag\\
    & + \frac{3L^{2}}{\alpha_{k}|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|\Bar{x}_{k+1} - \Bar{x}_{k}\|^{2}]
\end{align}
Finally we analyze the last term in the right hand side of the above inequality. For this we observe that from Eq. \eqref{eq:x_bar_update} using the inequality $\|a+b\|^{2} \leq 2\|a\|^{2}+\|b\|^{2}$ for any two vectors $a,b$, we have
\begin{align}
    &\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}\notag\\
    &= \Big\|\mathcal{E}_{k}-\mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\Bar{x}_{k})-\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big\|^{2}\notag\\
    & \leq 2\|\mathcal{E}_{x}\|^{2} + 2\Big\|\mathcal{T}\beta_{k}(\nabla q^{\mathcal{H}}(\Bar{x}_{k})-\nabla q^{\mathcal{H}}(x^{*}_{\mathcal{H}}))+\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big\|^{2}\notag.
\end{align}
Using the Lipschitz continuity of \( \nabla q^{\mathcal{H}} \) and noting that \( x^{*}_{\mathcal{H}} \) is the minimizer of \( q^{\mathcal{H}}(\bar{x}_{k}) \), implying \( \nabla q^{\mathcal{H}}(x^{*}_{\mathcal{H}}) = 0 \), we have
\begin{align}\label{eq:diff_x_k}
     &\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}\notag\\
    &\leq 2\|\mathcal{E}_{x}\|^{2} + 4\beta^{2}_{k}\mathcal{T}^{2}L^{2}\|\Bar{x}_{k} - x^{*}_{\mathcal{H}}\|^{2} + \frac{4\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}
\end{align}
Next, we further analyze the term $\|\mathcal{E }_{x}\|^{2}$ from \eqref{eq:V_x_update_0}. For this for some agent $j \in \mathcal{H}$ using \eqref{eq:e_k_t_iteration} we get
\begin{align}
    &\mathbb{E}[\|\mathcal{E}_{x}\|^{2}] \notag\\
    &\leq \frac{8\beta^{2}_{k}\mathcal{T}^{2}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\frac{4\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{l=0}^{\mathcal{T}-1}\Big[(1-\alpha_{k})^{l}\mathbb{E}[\|e^{j}_{k,0}\|^{2}] \notag\\
    &\hspace{1cm}+ \alpha_{k}L^{2}\sum_{l'=0}^{l-1}(1-\alpha_{k})^{l-l'-1}\mathbb{E}[\|x^{j}_{k,l'} - \Bar{x}_{k}\|^{2}] + \alpha^{2}_{k}\sigma^{2}l'\Big] \notag\\
    &+ \frac{4\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i\in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\Big[(1-\alpha_{k})^{t}\mathbb{E}[\|e^{i}_{k,0}\|^{2}]\notag\\
    &\hspace{1cm}+ \alpha_{k}L^{2}\sum_{l'=0}^{l-1}(1-\alpha_{k})^{l-l'-1}\mathbb{E}[\|x^{i}_{k,l'} - \Bar{x}_{k}\|^{2}]+ \alpha^{2}_{k}\sigma^{2}l'\Big] \notag\\
\end{align}
Since \( \alpha_{k} \leq 1 \), it follows that \( (1-\alpha_{k})^{t} \leq 1 \) for any $t \in [0,\mathcal{T}-1]$. Additionally, for any agent $j \in \mathcal{H}$ we use the following 
\begin{align*}
    &\sum_{l=0}^{\mathcal{T}-1}\|e^{j}_{k,0}\|^{2} \leq \sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2},\notag\\
    &\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,0}\|^{2} \leq \sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2},\notag
\end{align*} using which we have
\begin{align}\label{eq:V_x_update_2}
    &\mathbb{E}[\|\mathcal{E}_x\|^{2}]\notag\\
    &\leq \frac{8\beta^{2}_{k}\mathcal{T}^{2}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+\frac{8\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
    &+\frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\mathbb{E}[\|x^{j}_{k,l'} - \Bar{x}_{k}\|^{2}]\notag\\
    &+\frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i\in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\mathbb{E}[\|x^{i}_{k,l'} - \Bar{x}_{k}\|^{2}]\notag\\
    &+\frac{8\alpha^{2}_{k}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
\end{align}
Next using \eqref{eq:x_k_T_minus_bar_x_squared} we analyze the third last term in the right hand side of the above inequality as
\begin{align}\label{eq:V_x_term_3}
    &\frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\mathbb{E}[\|x^{j}_{k,l'} - \Bar{x}_{k}\|^{2}]\notag\\
    &\leq \frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\Big( 2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\Big)\notag\\
    & \leq \frac{8\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[V^{k}_{1}] \notag\\
    &\hspace{2cm}+ \frac{8\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{l= 0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
\end{align}
Similarly, using \eqref{eq:x_k_T_minus_bar_x_squared} the third last term in the right-hand side of \eqref{eq:V_x_update_2} can expressed as
\begin{align}\label{eq:V_x_term_2}
    &\frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\mathbb{E}[\|x^{j}_{k,l'} - \Bar{x}_{k}\|^{2}]\notag\\
    &\leq \frac{4\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{t=0}^{\mathcal{T}-1}\sum_{l'=0}^{t-1}\Big( 2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\Big)\notag\\
    & \leq\frac{8\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[V^{k}_{1}] \notag\\
    &\hspace{2cm}+ \frac{8\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{l= 0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
\end{align}
Thus, using the results of \eqref{eq:V_x_term_3} and \eqref{eq:V_x_term_2}, then \eqref{eq:V_x_update_2} can be expressed as
\begin{align}\label{eq:V_x_update_latest}
    &\mathbb{E}[\|\mathcal{E}_x\|^{2}] \leq \Big(\frac{8\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} + \frac{16\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+ \Big(\frac{8\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} + \frac{16\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+\frac{8\alpha^{2}_{k}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
\end{align}
Putting back the above result in \eqref{eq:diff_x_k} we have 
\begin{align}\label{eq:diff_x_k_update}
    &\mathbb{E}[\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}] \notag\\
    &\leq \Big(4\beta^{2}_{k}L^{2}\mathcal{T}^{2} + \frac{16\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} + \frac{32\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+ \Big(\frac{4\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}+\frac{16\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} \Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \frac{32\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]+\frac{16\alpha^{2}_{k}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}
\end{align}
Further putting the above result back in \eqref{eq:V_k_2} we get
\begin{align}
     &\mathbb{E}[V^{k+1}_{2}] \notag\\
     &\leq \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}] + 3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{4}\mathbb{E}[V^{k}_{1}]\notag\\
    & +\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]+ \frac{3\alpha_{k}^{2}\sigma^{2}\mathcal{T}^{2}}{2}\notag\\
    & + \frac{3L^{2}}{\alpha_{k}|\mathcal{H}|}\sum_{i \in \mathcal{H}}\Big[\Big(4\beta^{2}_{k}L^{2}\mathcal{T}^{2} + \frac{16\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+ \frac{32\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{4\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}+\frac{16\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} \Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \frac{32\alpha_{k}\beta^{4}_{k}\mathcal{T}^{4}L^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\Big]\notag\\
    & +\frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}, \notag
\end{align}
which upon simplification gives us the following
\begin{align}
    &\mathbb{E}[V^{k+1}_{2}]\notag\\
    &\leq \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}] + \Big(3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}+\frac{12\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\alpha_{k}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{48\beta^{2}_{k}L^{4}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}}+\frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{6}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+ \Big(\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{12\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{\alpha_{k}|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \Big(\frac{48\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}} + \frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.\notag
\end{align}
Hence proved.
\end{proof}
\tdoan{Could you ask one more lemma to  show how you handle the term $\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]$? Should you relate it to $V_{1}^{k}$ and $V_{2}^{k}$?}

\textcolor{blue}{Amit: I do not express \( \sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] \) in terms of \( V_{1}^{k} \) and \( V_{2}^{k} \) separately. Instead, I used the fact that \( V^{k}_{2} = \frac{1}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\|e^{i}_{k,0}\|^{2} \leq \frac{1}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} \). This leads to a term with \( -\frac{\alpha_{k}}{2} \) in the coefficients, which I then used to cancel out other terms related to \( \frac{1}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} \).
}
\tdoan{Don't see how you can eliminate $\frac{1}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}$.}\\
\begin{thm}\label{Theorem:SC_Tg1}
    Let $\{x^{i}_{k}\}$ and $\{y^{i}_{k}\}$ be generated by Algorithm \ref{alg:cap} for $\mathcal{T}>1$. We assume that the CE filter in Algorithm \eqref{alg:cap} satisfies the following condition
    \begin{align}\label{eq:filter_condition}
        \frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} = \frac{f}{N-f} \leq \frac{\mu}{3L}
    \end{align}
    Then choosing the step sizes $\alpha_{k}$ and $\beta_{k}$ as $\alpha_{k} = \frac{C_\alpha}{1+h+k}$ and $\beta_{k} = \frac{C_\beta}{1+h+k}$ with $C_{\alpha} < C_{\beta}$ satisfying 
    \begin{align}
        C_{\beta} = \frac{72}{\mu\mathcal{T}},\ C_{\alpha} \geq \frac{C_{\beta}}{C}
    \end{align} where,
    \begin{align}
        &C = \min \Big\{1, \frac{L}{80}, \frac{\mu}{(48)^{2}L^{4}\mathcal{T}} ,\frac{1}{170(L+1)^{2}\mathcal{T}}\Big\}\notag\\
        &h \geq \max\Big\{C_{\alpha},\frac{(42)^{2}L^{4}\mathcal{T}C_{\alpha}}{\mu}, \frac{(21)^{2}L^{2}\mathcal{T}C_{\beta}}{\mu}\Big\}
    \end{align}
    then we have 
\begin{align}\label{eq:convergence_2}
    &\mathbb{E}[V_{k+1}] \leq\frac{h^{2}\mathbb{E}[V^{0}]}{(1+h+k)^{2}} + \frac{3C_{\alpha}\sigma^{2}\mathcal{T}}{2(1+h+k)} + \frac{16C^{2}_{\alpha}L^{2}\mathcal{T}^{2}\sigma^{2}f}{(1+k+k)|\mathcal{H}|}.
\end{align}
\end{thm}

\begin{proof}
From the definition of the coupled Lyapunov function from \eqref{eq:lypunov_sc} we have
\begin{align*}
    \mathbb{E}[V^{k+1}] = &\mathbb{E}[\|\bar{x}_{k+1}-x^{*}_{\mathcal{H}}\|^{2}] + \mathbb{E}[e_{k+1}]\notag\\
    & = \mathbb{E}[V^{k+1}_{1}] + \mathbb{E}[V^{k+1}_{2}].\notag
\end{align*}
    Using results from Lemma 1 and Lemma 2, we have
    \begin{align}\label{eq:Lyapunov_V_k_update_v0}
        &\mathbb{E}[V^{k+1}] = \mathbb{E}[V^{k+1}_{1}]+\mathbb{E}[V^{k+1}_{2}]\notag\\
        &\leq\Big(1-2\mu\beta_{k}\mathcal{T} + \frac{35L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}+L^{2}\mathcal{T}^{2}\beta^{2}_{k} \Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{16L^{2}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} + \frac{19L^{3}\mathcal{T}^{3}\beta^{3}_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{6\beta_{k}}{L} + \frac{8\beta_{k}|\mathcal{B}_{k}|}{3L|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+\Big(\frac{2\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{16\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\ 
        &+\Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}] + \Big(3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}+\frac{12\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\alpha_{k}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+\Big(\frac{48\beta^{2}_{k}L^{4}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}}+\frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{6}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+ \Big(\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{12\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{\alpha_{k}|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \Big(\frac{48\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}} + \frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
    \end{align}
    Using the relation $\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{\mu}{3L}$ from \eqref{eq:filter_condition} we have
    \begin{align}
        -2\mu\beta_{k}\mathcal{T} + \frac{35L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}&\leq -2\mu\beta_{k}\mathcal{T} + \frac{35L\mathcal{T}\beta_{k}}{6}\Big(\frac{\mu}{3L}\Big)\notag\\
        & = -2\mu\beta_{k}\mathcal{T} + \frac{35\mu\beta_{k}\mathcal{T}}{18}\notag\\
        & = -\frac{\mu\beta_{k}\mathcal{T}}{18},\notag
    \end{align}
    using which \eqref{eq:Lyapunov_V_k_update_v0} becomes
    \begin{align}\label{eq:Lyapunov_V_k_update}
        &\mathbb{E}[V^{k+1}] \notag\\
        &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\mathbb{E}[V^{k}_{1}] + \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
        & + \Big(\underbrace{L^{2}\beta^{2}_{k}\mathcal{T}^{2} + \frac{16L^{2}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} +\frac{19L^{3}\beta^{3}_{k}\mathcal{T}^{3}|\mathcal{B}_{k}|}{6|\mathcal{H}|}}_{1}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
        &+\Big(\underbrace{\frac{48\beta^{2}_{k}L^{4}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}}+\frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{6}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}}_{2}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
        &+\Big(\underbrace{3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2} + \frac{12\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\alpha_{k}} }_{3}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
        &+\Big(\underbrace{\frac{6\beta_{k}}{L} + \frac{8\beta_{k}|\mathcal{B}_{k}|}{3L|\mathcal{H}|} + \frac{2\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}+\frac{16\beta^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} }_{4}\Big)\sum_{i\in\mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+\Big(\underbrace{\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{12\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{\alpha_{k}|\mathcal{H}|}}_{5}\Big)\sum_{i\in\mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+\Big(\underbrace{\frac{48\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}} + \frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}}_{6}\Big)\sum_{i\in\mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}
    \end{align}
    Next simplify each of the terms $1,2,3,4,5$ and $6$ as shown in the above equation. Using $\beta_{k}L\mathcal{T} \leq 1$ and $\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{\mu}{3L}\leq \frac{1}{3}$, we simplify term $1$ as 
    \begin{align}\label{eq:Simplify_Term1}
        &L^{2}\beta^{2}_{k}\mathcal{T}^{2} + \frac{16L^{2}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} +\frac{19L^{2}\beta^{2}_{k}\mathcal{T}^{2}(\beta_{k}L\mathcal{T})|\mathcal{B}_{k}|}{6|\mathcal{H}|}\notag\\
        &\leq \Big(1+\frac{16}{9}+\frac{19}{18}\Big)L^{2}\beta^{2}_{k}\mathcal{T}^{2}\leq \frac{69L^{2}\mathcal{T}^{2}\beta^{2}}{18}
    \end{align}
    Additionally using $\beta_{k} \leq \alpha_{k}$ along with $\beta_{k}L\mathcal{T}\leq 1$ and $\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{1}{3}$, term $2$ can be simplified as
    \begin{align}\label{eq:Simplify_Term2}
        &\frac{48\beta^{2}_{k}L^{4}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}} + \frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{6}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\notag\\
        &= \frac{48\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{9\alpha_{k}} + \frac{96(\beta_{k}L\mathcal{T})^{2}\beta^{2}_{k}\mathcal{T}^{2}L^{4}}{9}\notag\\
        &=\frac{16\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\alpha_{k}} + \frac{32\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3}\notag\\
        &\leq \frac{16\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\alpha_{k}} + \frac{32\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2}}{3}.
    \end{align}
Using $\beta_{k} \leq 1$ we have $\alpha_{k}\beta^{2}_{k} \leq \alpha_{k}\beta_{k}$ using which term $3$ can be  expressed as
\begin{align}\label{eq:Simplify_Term3}
     &3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2} + \frac{12\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\alpha_{k}}\notag\\
     &\leq 3\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2} + \frac{12\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\alpha_{k}}.
\end{align}
    Note that $\beta_{k}L\mathcal{T} \leq 1$ implies $\beta_{k} \leq \frac{1}{L\mathcal{T}}$ using which along with $\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{1}{3}$, we simplify term $4$ as the following
    \begin{align}\label{eq:Simplify_Term4}
        &\frac{6\beta_{k}}{L} + \frac{8\beta_{k}|\mathcal{B}_{k}|}{3L|\mathcal{H}|} + \frac{2\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{16\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\notag\\
        & \leq \Big(6+\frac{2}{3}+\frac{16}{9}+\frac{8}{9}\Big)\frac{\beta_{k}}{L} \leq \frac{28\beta_{k}}{3L}
    \end{align}
    Next, by noting that \( L \leq L+1 \leq (L+1)^{2} \) and \( L^{2} \leq (L+1)^{2} \), along with the facts that \( \beta_{k} \leq \alpha_{k} \) (implying \( \frac{\beta^{2}_{k}}{\alpha_{k}} \leq \beta_{k} \)), \( \alpha_{k} \leq 1 \), and \( \beta_{k}L\mathcal{T} \leq 1 \), Term 5 can be simplified as follows
    \begin{align}\label{eq:Simplify_Term5}
        &\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{12\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{\alpha_{k}|\mathcal{H}|}\notag\\
        &\leq \beta_{k}L\mathcal{T} + \frac{4\beta^{2}_{k}L^{2}\mathcal{T}}{\alpha_{k}}\notag\\
        &\leq \beta_{k}(L+1)^{2}\mathcal{T} + 4\beta_{k}(L+1)^{2}\mathcal{T} = 5\beta_{k}(L+1)^{2}\mathcal{T.}
    \end{align}
    Similarly, term $6$ can be expressed as \begin{align}\label{eq:Simplify_Term6}
        &\frac{48\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}} + \frac{96\beta^{4}_{k}\mathcal{T}^{4}L^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\notag\\
        &\leq \frac{16\beta^{2}_{k}L^{2}\mathcal{T}}{3\alpha_{k}} + \frac{32\beta_{k}L\mathcal{T}}{3} = 16\beta_{k}(L+1)^{2}\mathcal{T}.
    \end{align}
Thus putting back the results from \eqref{eq:Simplify_Term1}, \eqref{eq:Simplify_Term2}, \eqref{eq:Simplify_Term3}, \eqref{eq:Simplify_Term4}, \eqref{eq:Simplify_Term5} and \eqref{eq:Simplify_Term6} in the inequality \eqref{eq:Lyapunov_V_k_update} we get 
\begin{align}\label{eq:Lyapunov_V_k_update_1}
        &\mathbb{E}[V^{k+1}] \notag\\
        &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\mathbb{E}[V^{k}_{1}] + \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
        &+\Big(\frac{69L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18} + \frac{16\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\alpha_{k}} + \frac{32\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2}}{3}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
        &+\Big(3\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2} + \frac{12\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\alpha_{k}}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
        &+\Big(\frac{28\beta_{k}}{L}  + 21\beta_{k}(L+1)^{2}\mathcal{T}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.\notag\\
        &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\mathbb{E}[V^{k}_{1}] + \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
        &+\Big(\frac{69L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18} + \frac{52\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\alpha_{k}} + \frac{41\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2}}{3}\Big)\mathbb{E}[V^{k}_{1}] \notag\\
        &+\Big(\frac{28\beta_{k}}{3L} + 21\beta_{k}(L+1)^{2}\mathcal{T}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}\notag\\
        &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{36}\Big)\mathbb{E}[V^{k}_{1}] + \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
        &+\Big(-\frac{\mu\mathcal{T}\beta_{k}}{36} + \frac{69L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18} + \frac{52\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\alpha_{k}} \Big)\mathbb{E}[V^{k}_{1}] \notag\\
        &+ \frac{41\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2}}{3}\mathbb{E}[V^{k}_{1}] \notag\\
        &+\Big(\frac{28\beta_{k}}{3L} + 21\beta_{k}(L+1)^{2}\mathcal{T}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
\end{align}
Next using the definition of the Lyapunov function $V^{k}$, the above the inequality can be expressed as the following
\begin{align}\label{eq:Lyapunov_V_k_update_2}
    &\mathbb{E}[V^{k+1}]\notag\\
    &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{36}\Big)\mathbb{E}[V^{k}]\notag\\
    &-\Big(1-\frac{\mu\mathcal{T}\beta_{k}}{36}\Big)\mathbb{E}[V^{k}_{2}]+ \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
        &+\Big(-\frac{\mu\mathcal{T}\beta_{k}}{36} + \frac{69L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18} + \frac{52\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\alpha_{k}} \Big)\mathbb{E}[V^{k}_{1}] \notag\\
        &+ \frac{41\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2}}{3}\mathbb{E}[V^{k}_{1}] \notag\\
        &+\Big(\frac{28\beta_{k}}{3L} + 21\beta_{k}(L+1)^{2}\mathcal{T}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
\end{align}
Here we note that $$V^{k}_{2} = \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2} \leq \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}, $$ using which the third term in the right hand side of \eqref{eq:Lyapunov_V_k_update_2} becomes
\begin{align*}
    &\Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
    &\leq \Big(1-\frac{\alpha_{k}}{2}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &\leq \Big(1-\frac{\alpha_{k}}{4}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] -\frac{\alpha_{k}}{4|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}].
\end{align*}
Here we note that since $-\frac{\alpha_{k}}{4} \leq -\frac{\alpha_{k}}{4|\mathcal{H}|}$, the above inequality is also satisfied by
\begin{align*}
     &\Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
     &\leq \Big(1-\frac{\alpha_{k}}{4}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] -\frac{\alpha_{k}}{4}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}],
\end{align*}
using which \eqref{eq:Lyapunov_V_k_update_2} becomes
\begin{align}\label{eq:V_k_update_last_but_1}
    &\mathbb{E}[V^{k+1}]\notag\\
    &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{36}\Big)\mathbb{E}[V^{k}]\notag\\
    &-\Big(1-\frac{\mu\mathcal{T}\beta_{k}}{36}\Big)\mathbb{E}[V^{k}_{2}]+ \Big(1-\frac{\alpha_{k}}{4}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
        &+\Big(-\frac{\mu\mathcal{T}\beta_{k}}{36} + \frac{69L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18} + \frac{52\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\alpha_{k}} \Big)\mathbb{E}[V^{k}_{1}] \notag\\
        &+ \frac{41\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2}}{3}\mathbb{E}[V^{k}_{1}] \notag\\
        &+\Big(-\frac{\alpha_{k}}{4}+\frac{28\beta_{k}}{3L} + 21\beta_{k}(L+1)^{2}\mathcal{T}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}} \notag\\
    &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{36}\Big)V^{k}\notag\\
    & \underbrace{ - \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{36}\Big)V^{k}_{2} +\Big(1-\frac{\alpha_{k}}{4}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]}_{6}\notag\\
    &+\Big(\underbrace{\frac{-\mu\mathcal{T}\beta_{k}}{108} + \frac{69L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18}}_{7}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    &+ \Big(\underbrace{\frac{-\mu\mathcal{T}\beta_{k}}{54}+\frac{41\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2}}{3} + \frac{52\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\alpha_{k}}}_{8}\Big)\mathbb{E}[V^{k}_{1}]\notag\\
    & + \Big(\underbrace{\frac{-\alpha_{k}}{4} + \frac{28\beta_{k}}{3L} + 21\beta_{k}(L+1)^{2}\mathcal{T}}_{9}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
\end{align}
Next we analyze the terms $6,7,8$ and $9$. Using the result $\frac{\beta_{k}}{\alpha_{k}} \leq \frac{9}{\mu\mathcal{T}}$ we have
\begin{align*}
    \frac{\mu\mathcal{T}\beta_{k}}{36} \leq \frac{\alpha_{k}}{4},
\end{align*} 
which implies
\begin{align*}
     \frac{1-\frac{\mu\mathcal{T}\beta_{k}}{36}}{1-\frac{\alpha_{k}}{4}} \geq 1.
\end{align*}
Further, using the definition of $V^{k}_{2}$ and the above result, we have 
\begin{align}\label{eq:Term6_0}
\frac{1-\frac{\mu\mathcal{T}\beta_{k}}{36}}{1-\frac{\alpha_{k}}{4}} \geq 1\geq 
    \frac{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}} {\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}}.
\end{align}
Using the fact that $$\Bigg(\frac{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}} {\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}}\Bigg)^{2} \leq 1$$ which implies $$\frac{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}} {\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}} \leq \frac{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}}{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}}$$ we observe that \tdoan{Why we have this?}\\
\textcolor{blue}{Amit: I want to show Term $6 \leq 0$ i.e I want
\begin{align}
    &-\Big(1-\frac{\mu \mathcal{T}\beta_{k}}{36}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2} \notag\\
    &\hspace{2cm}+\Big(1-\frac{\alpha_{k}}{4}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} \leq 0 \notag
\end{align}
Rearranging we have
\begin{align*}
    \Big(1-\frac{\alpha_{k}}{4}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} \leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{36}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}
\end{align*}
Here note since $\beta_{k}L\mathcal{T} \leq 1, \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{36}\Big) \leq 1$ i.e positive. Hence 
\begin{align*}
    \frac{1-\frac{\alpha_{k}}{4}}{1-\frac{\mu\mathcal{T}\beta_{k}}{36}} \leq \frac{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}}{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}} \leq 1.
\end{align*}
This gives
\begin{align*}
     \frac{1-\frac{\alpha_{k}}{4}}{1-\frac{\mu\mathcal{T}\beta_{k}}{36}} \leq 1,
\end{align*}
implying $\frac{\beta_{k}}{\alpha_{k}} \leq \frac{9}{\mu \mathcal{T}}$. Thus staring from this condition we will have 
\begin{align*}
    \frac{1-\frac{\alpha_{k}}{4}}{1-\frac{\mu\mathcal{T}\beta_{k}}{36}} \leq 1 \leq \frac{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}}{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}}
\end{align*}
However this doesn't necessarily mean
\begin{align*}
    \frac{1-\frac{\alpha_{k}}{4}}{1-\frac{\mu\mathcal{T}\beta_{k}}{36}}  \leq \frac{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}}{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}}
\end{align*}
}
\begin{align*}
    \frac{1-\frac{\mu\mathcal{T}\beta_{k}}{36}}{1-\frac{\alpha_{k}}{4}}\geq \frac{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}}{\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}}
\end{align*}
implies \eqref{eq:Term6_0}. Thus \tdoan{How?} 
\begin{align*}
     &-\Big(1-\frac{\mu\mathcal{T}\beta_{k}}{36}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}\notag\\
     &\hspace{2cm}+\Big(1-\frac{\alpha_{k}}{4}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}] \leq 0
\end{align*}
Thus, term $6$ is non-positive and consequently be ignored in the analysis.
Note with the choice of step size $\beta_{k}  = \frac{C_{\beta}}{1+h+k}$ where $h \geq \frac{(21)^{2}L^{2}\mathcal{T}C_{\beta}}{\mu}$ we have
\begin{align}
    \frac{C_{\beta}}{h} \leq \frac{\mu}{(21)^{2}L^{2}\mathcal{T}},\notag
\end{align}
which implies 
\begin{align*}
    \beta_{k} = \frac{C_{\beta}}{1+h+k} \leq \frac{\mu}{(21)^{2}L^{2}\mathcal{T}},
\end{align*}
using which term $7$ becomes
\begin{align*}
    &\frac{-\mu\mathcal{T}\beta_{k}}{108} + \frac{69L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18}\notag\\
& \leq \frac{-\mu\mathcal{T}\beta_{k}}{108} + \frac{69L^{2}\mathcal{T}^{2}\beta_{k}}{18}\Big(\frac{\mu}{(21)^{2}L^{2}\mathcal{T}}\Big) = -\frac{\mu\mathcal{T}\beta_{k}}{4(21)^{2}} \leq 0
\end{align*}
Next choosing the step-size $\alpha_{k} = \frac{C_{\alpha}}{1+h+k}$ where $h \geq \frac{(42)^{2}L^{4}\mathcal{T}C_{\alpha}}{\mu}$ we have
\begin{align*}
    \frac{C_{\alpha}}{h} \leq \frac{\mu}{(42)^{2}(1+L)^{4}\mathcal{T}},
\end{align*}
using which we get 
\begin{align*}
    \alpha_{k} = \frac{C_{\alpha}}{1+h+k} \leq \frac{\mu}{(42)^{2}L^{4}\mathcal{T}}.
\end{align*}
Thus we have
\begin{align}\label{eq:Term8_1}
    &-\frac{\mu\mathcal{T}\beta_{k}}{108}+\frac{41\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2}}{3}\notag\\
    &\leq -\frac{\mu\mathcal{T}\beta_{k}}{108}+\frac{41\beta_{k}L^{4}\mathcal{T}^{2}}{3}\Big(\frac{\mu}{(42)^{2}L^{4}\mathcal{T}}\Big)\notag\\
    &=-\frac{\mu\mathcal{T}\beta_{k}}{108}+\frac{41\mu\mathcal{T}\beta_{k}}{3(42)^{2}} = -\frac{96\mu\mathcal{T}\beta_{k}}{(42)^{2}}\leq 0.
\end{align}
Further using $\frac{\beta_{k}}{\alpha_{k}} = \frac{C_{\beta}}{C_{\alpha}} \leq \frac{\mu}{(48)^{2}L^{4}\mathcal{T}}$, we have
\begin{align}\label{eq:Term8_2}
    &-\frac{\mu\mathcal{T}\beta_{k}}{108} + \frac{52\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\alpha_{k}}\notag\\
    &\leq-\frac{\mu\mathcal{T}\beta_{k}}{108} + \frac{52\beta_{k}L^{4}\mathcal{T}^{2}}{3}\Big(\frac{\mu}{(48)^{2}L^{4}\mathcal{T}}\Big) = -\frac{4\mu\mathcal{T}\beta_{k}}{(48)^{2}} \leq 0
\end{align}
Thus using the results from \eqref{eq:Term8_1} and \eqref{eq:Term8_2}, Term $8$ becomes
\begin{align*}
    &\frac{-\mu\mathcal{T}\beta_{k}}{54}+\frac{41\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2}}{3} + \frac{52\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\alpha_{k}}\notag\\
    & = \Big(\frac{-\mu\mathcal{T}\beta_{k}}{108}+\frac{41\alpha_{k}\beta_{k}L^{4}\mathcal{T}^{2}}{3} \Big) + \Big(\frac{-\mu\mathcal{T}\beta_{k}}{108}+\frac{52\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\alpha_{k}}\Big)\leq 0.
\end{align*}
Next we note that Term $9$ which can be expressed as 
\begin{align}
    &-\frac{\alpha_{k}}{4} + \frac{28\beta_{k}}{3L} + 21\beta_{k}(L+1)^{2}\mathcal{T}\notag\\
    &= -\frac{\alpha_{k}}{8}\Big(1-\frac{224\beta_{k}}{3L\alpha_{k}}\Big)-\frac{\alpha_{k}}{8}\Big(1-\frac{168\beta_{k}(L+1)^{2}\mathcal{T}}{\alpha_{k}}\Big),\notag
\end{align}
Upon using $\frac{\beta_{k}}{\alpha_{k}} \leq \frac{L}{80}$ and $\frac{\beta_{k}}{\alpha_{k}} \leq \frac{1}{170(1+L)^{2}\mathcal{T}}$ we have
\begin{align}
    &1-\frac{224\beta_{k}}{3L\alpha_{k}} \geq 1-\frac{224}{3L}\Big(\frac{L}{80}\Big) = \frac{1}{15} \geq 0,\notag\\
    &1-\frac{168(L+1)^{2}\mathcal{T}}{\alpha_{k}} \geq 1-168(L+1)^{2}\mathcal{T}\Big(\frac{1}{170(L+1)^{2}\mathcal{T}}\Big)\notag\\
    &\hspace{5cm}=\frac{1}{85} \geq 0,\notag
\end{align}
using which Term $9$ becomes
\begin{align*}
     &-\frac{\alpha_{k}}{4} + \frac{28\beta_{k}}{3L} + 21\beta_{k}(L+1)^{2}\mathcal{T}\notag\\
    &= -\frac{\alpha_{k}}{8}\Big(1-\frac{224\beta_{k}}{3L\alpha_{k}}\Big)-\frac{\alpha_{k}}{8}\Big(1-\frac{168\beta_{k}(L+1)^{2}\mathcal{T}}{\alpha_{k}}\Big)\notag\\
    &\leq -\frac{\alpha_{k}}{8}\Big(\frac{1}{15} + \frac{1}{85}\Big) = -\frac{\alpha_{k}}{102}\leq 0
\end{align*}
Thus we notice that each of the terms $6,7,8$ and $9$ are non-positive hence we can ignore them in the analysis. Thus the inequality \eqref{eq:V_k_update_last_but_1} can be expressed as the following
\begin{align*}
    &\mathbb{E}[V^{k+1}] \notag\\
    &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{36}\Big)V^{k}+ \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
\end{align*}
Here we note that with $C_{\beta}\leq C_{\alpha}$ and $h \geq C_{\alpha}$ we ensure that $\beta_{k}\leq\alpha_{k}\leq 1$ which implies $\alpha_{k}\beta^{2}_{k} \leq \alpha^{3}_{k}\leq \alpha^{2}_{k}$. Further since $\beta_{k} = \frac{C_{\beta}}{1+h+}$ with $C_{\beta} = \frac{72}{\mu\mathcal{T}}$ and $\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{f}{|\mathcal{H}|} \leq \frac{1}{3}$ we have 
\begin{align*}
    &\mathbb{E}[V^{k+1}]\notag\\
    &\leq \Big(1-\frac{2}{1+h+k}\Big)\mathbb{E}[V^{k}] + \frac{3C_{\alpha}^{2}\sigma^{2}\mathcal{T}}{2(1+h+k)^{2}} + \frac{16C_{\alpha}^{2}L^{2}\mathcal{T}^{2}f\sigma^{2}}{(1+h+k)^{2}|\mathcal{H}|}\notag\\
    & = \Big(\frac{h+k-1}{h+k+1}\Big)\mathbb{E}[V^{k}] + \frac{3C_{\alpha}^{2}\sigma^{2}\mathcal{T}}{2(1+h+k)^{2}} + \frac{16C_{\alpha}^{2}L^{2}\mathcal{T}^{2}f\sigma^{2}}{(1+h+k)^{2}|\mathcal{H}|}.
\end{align*}
Multiplying both sides of the above inequality by $(1+h+k)^2$ we have the following
\begin{align*}
    &(1+h+k)^{2}\mathbb{E}[V^{k+1}]\notag\\
    &\leq (h+k)^{2}\mathbb{E}[V^{k}] + \frac{3C_{\alpha}^{2}\sigma^{2}\mathcal{T}}{2} + \frac{16C_{\alpha}^{2}L^{2}\mathcal{T}^{2}f\sigma^{2}}{|\mathcal{H}|}\notag\\
    &\leq h^{2}\mathbb{E}[V^{0}] + \frac{3C_{\alpha}^{2}\sigma^{2}\mathcal{T}(1+k)}{2} + \frac{16C_{\alpha}^{2}L^{2}\mathcal{T}^{2}f\sigma^{2}(1+k)}{|\mathcal{H}|},\notag
\end{align*}
which gives us the following
\begin{align*}
    &\mathbb{E}[V^{k+1}] \notag\\
    &\leq \frac{h^{2}\mathbb{E}[V^{0}]}{(1+h+k)^{2}} + \frac{3C_{\alpha}\sigma^{2}\mathcal{T}(1+k)}{2(1+h+k)^{2}} + \frac{16C^{2}_{\alpha}L^{2}\mathcal{T}^{2}\sigma^{2}f(1+k)}{(1+h+k)^{2}|\mathcal{H}|}\notag\\
    &\leq \frac{h^{2}\mathbb{E}[V^{0}]}{(1+h+k)^{2}} + \frac{3C_{\alpha}\sigma^{2}\mathcal{T}}{2(1+h+k)} + \frac{16C^{2}_{\alpha}L^{2}\mathcal{T}^{2}\sigma^{2}f}{(1+h+k)|\mathcal{H}|}
\end{align*}

\subsection{Non-convex satisfying PL condition}\label{sec:PL}
 Here we assume that the average non-faulty cost function with the honest agents, $q^{\mathcal{H}}(x)$ to be non-convex satisfying PL condition satisfying the following assumption
 \begin{assumption}\label{eq:Assump_3}
(PL condition and quadratic growth). The function $q^{\mathcal{H}}$ satisfies PL condition and quadratic growth
\begin{align}\label{eq:PL condition}
    \frac{1}{2}\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} \geq \mu (q^{\mathcal{H}}(\Bar{x}_{k}) - q^{\mathcal{H}}(x^{*}_{\mathcal{H}})) \geq \frac{\mu^{2}}{2}\|\Bar{x}_{k} - x^{*}_{\mathcal{H}}\|^{2}.
\end{align}
\end{assumption}
\begin{lemma}\label{lem:Lemma_V1_PL}
The difference between $\nabla q^{\mathcal{H}}(\Bar{x}_{k+1})$ and $\nabla q^{\mathcal{H}}(\Bar{x}_{k})$ where $\Bar{x}_{k}$ be defined as in line $15$ in Algorithm \ref{alg:cap} satisfy the following 
    \begin{align}
        &\mathbb{E}[\nabla q^{\mathcal{H}}(\Bar{x}_{k+1}) -\nabla q^{\mathcal{H}}(\Bar{x}_{k})]\notag\\
        &\leq \Big(-\mathcal{T}\beta_{k} + \frac{11\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{4\mu|\mathcal{H}|}\Big)\|\mathbb{E}[\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
        &+\Big(\frac{2L^{3}\beta^{2}_{k}\mathcal{T}^{2}}{\mu^{2}} + \frac{4L^{3}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\|\mathbb{E}[\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
        &+\Big(\frac{\mu\beta_{k}}{L}+\frac{ 16\mu\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|} \Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+\Big(\frac{2\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{L|\mathcal{H}|} +\frac{8\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{L|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}].
    \end{align}
\end{lemma}
Next using Lemma \ref{lem:Lemma_V2_SC} for non-convex satisfying PL condition we have the following lemma.
\begin{lemma}\label{lem:Lemma_V2_PL}
Let the lyapunov function for the cumulative gradient error be given by
\begin{align}\label{eq:V_2_def_PL}
    V^{k}_{2} = \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}
\end{align}
where $e^{i}_{k,t}$ be the gradient error as defined in \eqref{eq:e_k_t}, then
    \begin{align}
        &\mathbb{E}[V^{k+1}_{2}] \leq \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}] \notag\\
        &+\Big(3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}+\frac{60\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\alpha_{k}} \Big)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
        &+\frac{96\beta^{4}\mathcal{T}^{4}L^{6}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}} \mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
        &+ \Big(\frac{3\alpha_{k}\beta^{2}_{k}L^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{12\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{\alpha_{k}|\mathcal{H}|}\Big)\sum_{i\in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
    &+ \Big(\frac{48\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}} + \frac{96\alpha_{k}\beta^{4}_{k}L^{4}\mathcal{T}^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i\in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
    & + \frac{3\alpha_{k}^{2}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
    \end{align}
\end{lemma}
\end{proof}
\begin{thm}\label{Theorem:SC_Tg1}
    Let $\{x^{i}_{k}\}$ and $\{y^{i}_{k}\}$ be generated by Algorithm \ref{alg:cap} for $\mathcal{T}>1$. We assume that the CE filter in Algorithm \eqref{alg:cap} satisfies the condition in \eqref{eq:filter_condition}. Further let the average of the cost functions of the honest agents satift non-convexity with PL condition in \eqref{eq:Assump_3}. Then choosing the step sizes $\alpha_{k}$ and $\beta_{k}$ as $\alpha_{k} = \frac{C_\alpha}{1+h+k}$ and $\beta_{k} = \frac{C_\beta}{1+h+k}$ with $C_{\alpha} < C_{\beta}$ satisfying 
    \begin{align}
        C_{\beta} = \frac{48}{\mu\mathcal{T}},\ C_{\alpha} \geq \frac{C_{\beta}}{C}
    \end{align} where,
    \begin{align}
        &C = \min \Big\{1, \frac{1}{448(L+1)^{2}\mathcal{T}}, \frac{\mu^{2}}{2280L^{4}\mathcal{T}}, \frac{3L}{88\mu`}\Big\}
    \end{align}
    then we have 
\begin{align}\label{eq:convergence_2}
    &\mathbb{E}[V_{k+1}] \leq\frac{h^{2}\mathbb{E}[V^{0}]}{(1+h+k)^{2}} + \frac{3C_{\alpha}\sigma^{2}\mathcal{T}}{2(1+h+k)} + \frac{16C^{2}_{\alpha}L^{2}\mathcal{T}^{2}\sigma^{2}f}{(1+k+k)|\mathcal{H}|}.
\end{align}
\end{thm}
\begin{proof}
    Using the realtion from Lemma \ref{lem:Lemma_V2_SC} and Assumption \ref{eq:Assump_3} we get the following
    \begin{align}
        &\mathbb{E}[\nabla q^{\mathcal{H}}(\Bar{x}_{k+1})-\nabla q^{\mathcal{H}}(\Bar{x}_{k})] + \mathbb{E}[V^{k+1}_{2}]\notag\\
        &\leq \Big(-\mathcal{T}\beta_{k} + \frac{11\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{4\mu|\mathcal{H}|} + \frac{2\beta^{2}_{k}L^{3}\mathcal{T}^{2}}{\mu^{2}}\Big)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
        &+ \frac{8\beta^{2}_{k}L^{3}\mathcal{T}^{2}|\mathcal{B}|^{2}}{\mu^{2}|\mathcal{H}|^{2}}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
        &+\Big(\frac{3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}} + \frac{60\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}\alpha_{k}}\Big)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
        &+ \frac{96\beta^{4}_{k}L^{6}\mathcal{T}^{4}|\mathcal{B}_{k}|^{2}}{\mu^{2}|\mathcal{H}|^{2}}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
        &+\Big(\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{12\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{\alpha_{k}|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+\Big(\frac{48\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}} + \frac{96\alpha_{k}\beta^{4}_{k}L^{4}\mathcal{T}^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        & + \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.\notag
    \end{align}
    Using the filter condition from \eqref{eq:filter_condition} we have the following
    \begin{align}
       & -\mathcal{T}\beta_{k} + \frac{11\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{4\mu|\mathcal{H}|}\notag\\
       & \leq -\mathcal{T}\beta_{k} + \frac{11\mathcal{T}\beta_{k}}{12} = -\frac{\mathcal{T}\beta_{k}}{12},\notag
    \end{align}
    using which we have
    \begin{align}\label{eq:diff_h_V2}
        &\mathbb{E}[\nabla q^{\mathcal{H}}(\Bar{x}_{k+1})-\nabla q^{\mathcal{H}}(\Bar{x}_{k})] + \mathbb{E}[V^{k+1}_{2}]\notag\\
        &\leq \Big(-\frac{\mathcal{T}\beta_{k}}{12} + \frac{2\beta^{2}_{k}L^{3}\mathcal{T}^{2}}{\mu^{2}}+ \frac{8\beta^{2}_{k}L^{3}\mathcal{T}^{2}|\mathcal{B}_{k }|^{2}}{\mu^{2}|\mathcal{H}|^{2}}\Big)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
        & + \frac{96\beta^{4}_{k}L^{6}\mathcal{T}^{4}|\mathcal{B}_{k}|^{2}}{\mu^{2}|\mathcal{H}|^{2}}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]+ \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
        &+\Big(\frac{3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}} + \frac{60\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}\alpha_{k}}\Big)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
        &+\Big(\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{12\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{\alpha_{k}|\mathcal{H}|}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        &+\Big(\frac{48\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}} + \frac{96\alpha_{k}\beta^{4}_{k}L^{4}\mathcal{T}^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        & + \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
    \end{align}
    Next using $h \geq \frac{(36.17)(L+1)^{4}\mathcal{T}C_{\beta}}{\mu^{2}}$, which satisfies $\beta_{k} = \frac{C_{\beta_{k}}}{1+h+k}\leq \frac{\mu^{2}}{(36.17)L^{3}\mathcal{T}}$, it implies $\beta_{k} \leq \frac{\mu^{2}}{(36.17)L^{3}\mathcal{T}} \leq \frac{1}{(36.17)L\mathcal{T}}$. This in-turn imples $\beta_{k}L\mathcal{T} \leq 1$. Furthermore, along with the condition $\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{\mu}{3L} \leq \frac{1}{3}$ we have
    \begin{align}
        &\frac{2\beta^{2}_{k}L^{3}\mathcal{T}^{2}}{\mu^{2}}+ \frac{8\beta^{2}_{k}L^{3}\mathcal{T}^{2}|\mathcal{B}_{k }|^{2}}{\mu^{2}|\mathcal{H}|^{2}}+\frac{96\beta^{4}_{k}L^{6}\mathcal{T}^{4}|\mathcal{B}_{k}|^{2}}{\mu^{2}|\mathcal{H}|^{2}} \notag\\
        &+ \frac{3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}} + \frac{60\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}\alpha_{k}}\notag\\
        &\leq \frac{2\beta^{2}_{k}L^{3}\mathcal{T}^{2}}{\mu^{2}}+ \frac{8\beta^{2}_{k}L^{3}\mathcal{T}^{2}}{9\mu^{2}} + \frac{32(\beta_{k}L\mathcal{T})^{2}\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{3\mu^{2}}\notag\\
        &+ \frac{3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}} + \frac{60\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}\alpha_{k}}.\notag
    \end{align}
    Here note that since $L>0$ we have $L^{3}\leq (L+1)^{3} \leq (L+1)^{4}$. Further using $\alpha_{k} \leq 1$ which implies $\alpha_{k}\beta^{2}_{k} \leq \beta^{2}_{k}$ using which we have
     \begin{align}\label{eq:co_eff_q_h}
         &\frac{2\beta^{2}_{k}L^{3}\mathcal{T}^{2}}{\mu^{2}}+ \frac{8\beta^{2}_{k}L^{3}\mathcal{T}^{2}|\mathcal{B}_{k }|^{2}}{\mu^{2}|\mathcal{H}|^{2}}+\frac{96\beta^{4}_{k}L^{6}\mathcal{T}^{4}|\mathcal{B}_{k}|^{2}}{\mu^{2}|\mathcal{H}|^{2}} \notag\\
        &+ \frac{3\alpha_{k}\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}} + \frac{60\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}\alpha_{k}}\notag\\
        &\leq \frac{149\beta^{2}_{k}(L+1)^{4}\mathcal{T}^{2}}{9\mu^{2}} + \frac{60\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}\alpha_{k}}.
     \end{align}
    Similarly, using $\beta_{k}L\mathcal{T} \leq 1 $, $\beta_{k} \leq \alpha_{k} \leq 1$ and $\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{\mu}{3L} \leq \frac{1}{3}$ we have 
    \begin{align}\label{eq:co_eff_epsilion}
    &\frac{3\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|} + \frac{12\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|}{\alpha_{k}|\mathcal{H}|}\notag\\
    &+ \frac{48\beta^{2}_{k}L^{2}\mathcal{T}|\mathcal{B}_{k}|^{2}}{\alpha_{k}|\mathcal{H}|^{2}} + \frac{96\alpha_{k}\beta^{4}_{k}L^{4}\mathcal{T}^{4}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\notag\\
    &\leq \alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2} + \frac{4\beta^{2}_{k}L^{2}\mathcal{T}}{\alpha_{k}} + \frac{48\beta^{2}_{k}L^{2}\mathcal{T}}{\alpha_{k}} + \frac{28\alpha_{k}(\beta_{k}L\mathcal{T})^{3}\beta_{k}L\mathcal{T}}{3}\notag\\
    &\leq \frac{35\beta_{k}L\mathcal{T}}{3} + \frac{28\beta_{k}L^{2}\mathcal{T}}{3} \leq 21\beta_{k}(L+1)^{2}\mathcal{T}
    \end{align}
    Putting back the relations from \eqref{eq:co_eff_q_h} and \eqref{eq:co_eff_epsilion} into \eqref{eq:diff_h_V2} we have
    \begin{align}
        &\mathbb{E}[\nabla q^{\mathcal{H}}(\Bar{x}_{k+1})-\nabla q^{\mathcal{H}}(\Bar{x}_{k})] + \mathbb{E}[V^{k+1}_{2}]\notag\\
        & \leq \Big(-\frac{\mathcal{T}\beta_{k}}{12} + \frac{149\beta^{2}_{k}(L+1)^{4}\mathcal{T}^{2}}{9\mu^{2}} + \frac{60\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}\alpha_{k}}\Big)\mathbb{E}[\nabla q^{\mathcal{H}}(\Bar{x}_{k})]\notag\\
        & + 21\beta_{k}(L+1)^{2}\mathcal{T}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}] + \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
         & + \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.
    \end{align}
    Next using $\beta_{k} \leq \frac{\mu^{2}}{(48.17)L^{3}\mathcal{T}}$ and $\frac{C_{\beta}}{C_{\alpha}} = \frac{\beta_{k}}{\alpha_{k}} \leq \frac{\mu^{2}}{2160L^{4}\mathcal{T}}$ we have the following results
    \begin{align}
        &-\frac{\mathcal{T}\beta_{k}}{36} + \frac{149(L+1)^{4}\mathcal{T}^{2}}{9\mu^{2}} \leq -\frac{\mathcal{T}\beta_{k}}{36} + \frac{149\mathcal{T}\beta_{k}}{9.17.48} \leq 0,\notag\\
        &-\frac{\mathcal{T}\beta_{k}}{36} + \frac{60\beta^{2}_{k}L^{4}\mathcal{T}^{2}}{\mu^{2}\alpha_{k}} \leq 0,\notag
    \end{align}
    using which we have 
    \begin{align}
        &\mathbb{E}[\nabla q^{\mathcal{H}}(\Bar{x}_{k+1})-\nabla q^{\mathcal{H}}(\Bar{x}_{k})] + \mathbb{E}[V^{k+1}_{2}]\notag\\
        &\leq -\frac{\mathcal{T}\beta_{k}}{36}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]+ \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
        & + 21\beta_{k}(L+1)^{2}\mathcal{T}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}] \notag\\
         & + \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.\notag
    \end{align}
    Next, since $q^{\mathcal{H}}(\Bar{x}_{k})$ is non-convex satisfying PL condition hence $-\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} \leq -2\mu(q^{\mathcal{H}}(\Bar{x}_{k}) - q^{\mathcal{H}}(x^{*}))$, which gives us 
    \begin{align}
        &\mathbb{E}[\nabla q^{\mathcal{H}}(\Bar{x}_{k+1}) - \nabla q^{\mathcal{H}}(x^{*}_{\mathcal{H}})] + \mathbb{E}[V^{k+1}_{2}]\notag\\
        &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\mathbb{E}[\nabla q^{\mathcal{H}}(\Bar{x}_{k}) - \nabla q^{\mathcal{H}}(x^{*}_{\mathcal{H}})]+ \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]\notag\\
        & + 21\beta_{k}(L+1)^{2}\mathcal{T}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}] \notag\\
         & + \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.\notag
    \end{align}
    Using the definition of the aggregate lyapunov function and $V^{k}_{1}$ we have the following
    \begin{align}\label{eq:V_k_PL_update_0}
        &\mathbb{E}[V^{k+1}]\notag\\
        &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\mathbb{E}[V^{k}]+ \Big(1-\frac{\alpha_{k}}{2}\Big)\mathbb{E}[V^{k}_{2}]-\Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\mathbb{E}[V_{2}^{k}]\notag\\
        & + 21\beta_{k}(L+1)^{2}\mathcal{T}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}] \notag\\
         & + \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}\notag\\
         &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\mathbb{E}[V^{k}]+ \Big(1-\frac{\alpha_{k}}{4}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
         &-\Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|e^{i}_{k,0}\|^{2}]\notag\\
         &+\Big(-\frac{\alpha_{k}}{4|\mathcal{H}|} + 21\beta_{k}(L+1)^{2}\mathcal{T}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
         & + \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.\notag
    \end{align}
    Next let $\epsilon_{k,t} = \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\|e^{i}_{k,t}\|^{2}$ and $\epsilon_{k,0} = \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}$, using which we have $\frac{\epsilon_{0}}{\epsilon_{t}} \leq 1$. This also implies $\Big(\frac{\epsilon_{0}}{\epsilon_{t}}\Big) \leq 1$ further implying $\frac{\epsilon_{0}}{\epsilon_{t}} \leq \frac{\epsilon_{t}}{\epsilon_{0}}$. Now using $\frac{C_{\beta}}{C_{\alpha}} = \frac{\beta_{k}}{\alpha_{k}} \leq \frac{9}{2\mu\mathcal{T}}$ we have
    \begin{align}
        \frac{1-\frac{\alpha_{k}}{4}}{1-\frac{\mu\mathcal{T}\beta_{k}}{18}} \leq 1 \leq \frac{\epsilon_{t}}{\epsilon_{0}}. \notag
    \end{align}
    Note that the above inequality is satisfied by
    \begin{align}
         \frac{1-\frac{\alpha_{k}}{4}}{1-\frac{\mu\mathcal{T}\beta_{k}}{18}} \leq \frac{\epsilon_{0}}{\epsilon_{t}},\notag
    \end{align}
    which implies
    \begin{align}
        &\Big(1-\frac{\alpha_{k}}{4}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
        & \hspace{2cm}-\Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\mathbb{E}[\|e^{i}_{k,0}\|^{2}] \leq 0.\notag
    \end{align}
    Using the above the above result we further simplify \eqref{eq:V_k_PL_update_0} as 
    \begin{align}
        &\mathbb{E}[V^{k+1}]\notag\\
        &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\mathbb{E}[V^{k}]\notag\\
         &+\Big(-\frac{\alpha_{k}}{4|\mathcal{H}|} + 21\beta_{k}(L+1)^{2}\mathcal{T}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
         & + \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.\notag
    \end{align}
    Note that the above inequality is further satisfied by the following
    \begin{align}
        &\mathbb{E}[V^{k+1}]\notag\\
        &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\mathbb{E}[V^{k}]\notag\\
         &+\Big(-\frac{\alpha_{k}}{4} + 21\beta_{k}(L+1)^{2}\mathcal{T}\Big)\sum_{i \in \mathcal{H}}\sum_{t=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\notag\\
         & + \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.\notag
    \end{align}
    Next $\frac{\beta_{k}}{\alpha_{k}} \leq \frac{1}{84(L+1)^{2}\mathcal{T}}$ implies
    \begin{align}
        -\frac{\alpha_{k}}{4} + 21\beta_{k}(L+1)^{2}\mathcal{T} \leq 0,\notag
    \end{align}
    using which we have
    \begin{align}
        &\mathbb{E}[V^{k+1}]\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\mathbb{E}[V^{k}]\notag\\
         & + \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{48\alpha_{k}\beta^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}.\notag
    \end{align}
    Next using $\beta_{k} \leq \alpha_{k} \leq 1$ we $\alpha_{k}\beta^{2}_{k} \leq \alpha^{2}_{k}$. Further using $\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{f}{|\mathcal{H}|} \leq \frac{\mu}{3L} \leq \frac{1}{3}$ we have
    \begin{align}
         &\mathbb{E}[V^{k+1}]\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}\Big)\mathbb{E}[V^{k}]\notag\\
         & + \frac{3\alpha^{2}_{k}\sigma^{2}\mathcal{T}}{2} + \frac{16\alpha^{2}_{k}L^{2}\mathcal{T}^{2}f^{2}\sigma^{2}}{|\mathcal{H}|^{2}}
    \end{align}
     Further since $\beta_{k} = \frac{C_{\beta}}{1+h+k}$ with $C_{\beta} = \frac{36}{\mu\mathcal{T}}$ we have 
\begin{align*}
    &\mathbb{E}[V^{k+1}]\notag\\
    &\leq \Big(1-\frac{2}{1+h+k}\Big)\mathbb{E}[V^{k}] + \frac{3C_{\alpha}^{2}\sigma^{2}\mathcal{T}}{2(1+h+k)^{2}} + \frac{16C_{\alpha}^{2}L^{2}\mathcal{T}^{2}f\sigma^{2}}{(1+h+k)^{2}|\mathcal{H}|}\notag\\
    & = \Big(\frac{h+k-1}{h+k+1}\Big)\mathbb{E}[V^{k}] + \frac{3C_{\alpha}^{2}\sigma^{2}\mathcal{T}}{2(1+h+k)^{2}} + \frac{16C_{\alpha}^{2}L^{2}\mathcal{T}^{2}f\sigma^{2}}{(1+h+k)^{2}|\mathcal{H}|}.
\end{align*}
Multiplying both sides of the above inequality by $(1+h+k)^2$ we have the following
\begin{align*}
    &(1+h+k)^{2}\mathbb{E}[V^{k+1}]\notag\\
    &\leq (h+k)^{2}\mathbb{E}[V^{k}] + \frac{3C_{\alpha}^{2}\sigma^{2}\mathcal{T}}{2} + \frac{16C_{\alpha}^{2}L^{2}\mathcal{T}^{2}f\sigma^{2}}{|\mathcal{H}|}\notag\\
    &\leq h^{2}\mathbb{E}[V^{0}] + \frac{3C_{\alpha}^{2}\sigma^{2}\mathcal{T}(1+k)}{2} + \frac{16C_{\alpha}^{2}L^{2}\mathcal{T}^{2}f\sigma^{2}(1+k)}{|\mathcal{H}|},\notag
\end{align*}
which gives us the following
\begin{align*}
    &\mathbb{E}[V^{k+1}] \notag\\
    &\leq \frac{h^{2}\mathbb{E}[V^{0}]}{(1+h+k)^{2}} + \frac{3C_{\alpha}\sigma^{2}\mathcal{T}(1+k)}{2(1+h+k)^{2}} + \frac{16C^{q}_{\alpha}L^{2}\mathcal{T}^{2}\sigma^{2}f(1+k)}{(1+h+k)^{2}|\mathcal{H}|}\notag\\
    &\leq \frac{h^{2}\mathbb{E}[V^{0}]}{(1+h+k)^{2}} + \frac{3C_{\alpha}\sigma^{2}\mathcal{T}}{2(1+h+k)} + \frac{16C^{q}_{\alpha}L^{2}\mathcal{T}^{2}\sigma^{2}f}{(1+h+k)|\mathcal{H}|}
\end{align*}
\end{proof}

==> MainReults_new.tex <==
\section{Main Results}
In this section, we present the main results of this paper, where we provide convergence rates of Algorithm \ref{alg:cap}
\subsection{Strongly convex condition}
\begin{thm}\label{Theorem:SC_Tg1}
    Let $\{\Bar{x}_{k}\}$ be generated by Algorithm \ref{alg:cap} for $\mathcal{T}>1$ and assume that the following condition hold.
    \begin{align}\label{eq:filter_condition}
        \frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{\mu}{3L}
    \end{align}
Let the step sizes $\alpha_{k}$ and $\beta_{k}$ satisfy
\begin{align}\label{eq:step_size_a_b_g}
    &\beta_{k} \leq \frac{\mu}{(18)^{2}L^{2}\mathcal{T}}, \quad \leq \alpha_{k} \leq \frac{\mu}{(42)^{3}L\mathcal{T}},\notag \\
    &\frac{\beta_{k}}{\alpha_{k}} \leq \min\Big\{\frac{18}{\mu\mathcal{T}},\frac{1}{(16)^{2}L\mathcal{T}^{3}}, \frac{\sqrt{\mu}}{L\mathcal{T}}\Big\}
\end{align}

Further let $\gamma$ satisfy
\begin{align}\label{eq:sc_gamma}
    \frac{180\mathcal{T}}{L}\leq \gamma \leq \frac{\mu}{(46)^{3}L^{2}\mathcal{T}^{3}}
\end{align}
then
\begin{align}\label{eq:convergence_1}
    &V_{k+1} \leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{90}\Big)V_{k} +\Gamma \alpha_{k}\beta_{k}\sigma^{2}
\end{align}
where
% \begin{align*}
%     \Gamma = \frac{(12)^{2}\mathcal{T}^{3}|\mathcal{H}|}{L} + \frac{(12)^{3}\gamma\mathcal{T}|\mathcal{H}|}{\mu L} + (15)^{2}\gamma \mathcal{T}|\mathcal{H}|
% \end{align*}
% \begin{align*}
%     \Gamma = \frac{212\mathcal{T}^{3}{L} + 292\gamma\alpha_{k}\beta_{k}\mathcal{T}^{3}
% \end{align*}
\begin{equation*}
    \Gamma = 292\gamma\mathcal{T}^{3}|\mathcal{H}| + \frac{12\mathcal{T}^{3}|\mathcal{H}|}{L}
\end{equation*}
Further let $\alpha_{k}, \beta_{k}$ be chosen as
\begin{align}\label{eq:sc_step}
    \beta_{k} = \frac{\beta_{0}}{k+1} ,\ \alpha_{k} = \frac{\alpha_{0}}{(k+1)^{2/3}}
\end{align} with $$\beta_{0} = \frac{90}{\mu\mathcal{T}}.$$Then we have
\begin{align}\label{eq:convergence_2}
    &V_{k+1} \leq \Big(\frac{1}{1+k}\Big)V_{1} + \frac{3\Gamma\alpha_{0}\beta_{0}\sigma^{2}}{(1+k)^{2/3}}.
\end{align}
\end{thm}
\subsection{PL condition}
\begin{thm}\label{Theorem:PL_Tg1}
    Let $\{\Bar{x}_{k}\}$ be generated by Algorithm \ref{alg:cap} for $\mathcal{T}>1$ and assume that the following condition hold.
    \begin{align}\label{eq:filter_condition}
        \frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{\mu}{3L}
    \end{align}
Let the step sizes $\alpha_{k}$ and $\beta_{k}$ satisfy
\begin{align}\label{eq:step_size_a_b_g}
    &\beta_{k} \leq \frac{3\mu^{2}}{208L^{2}\mathcal{T}}, \quad \frac{1}{1+\eta} \leq \alpha_{k} \leq \frac{\mu}{(27)^{2}L\mathcal{T}},\notag \\
    &\frac{\beta_{k}}{\alpha_{k}} \leq \min\Big\{\frac{(1+\eta)|\mathcal{H}|}{3(1+2\eta)\mu L}, \frac{1}{360(1+\eta)L\mathcal{T}|\mathcal{H}|}, \frac{L}{73\mu}, \frac{1}{120L}, \frac{3}{5\mu\mathcal{T}}\Big\}
\end{align}
Further let $\gamma$ satisfy
\begin{align}\label{eq:sc_gamma}
     \gamma \leq \min\Big\{\frac{\mu^{2}}{(19)^{3}(1+\eta)L^{2}\mathcal{T}|\mathcal{H}|},\frac{\mu^{2}}{(39)^{2}(1+2\eta)L^{2}\mathcal{T}^{2}|\mathcal{H}|}\Big\}
\end{align}
where 
\begin{align}\label{eq:eta}
    \eta \leq \zeta - \frac{1}{2};\ \zeta = \frac{1}{320 L^{2}\mathcal{T}|\mathcal{H}|}
\end{align}
then
\begin{align}\label{eq:convergence_1}
    &V_{k+1} \leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{6}\Big)V_{k} +\Gamma \alpha_{k}\beta_{k}\sigma^{2}
\end{align}
where
\begin{align*}
    \Gamma = \frac{8\mu\mathcal{T}^{3}|\mathcal{H}|}{L} + 18L\mathcal{T}^{3}|\mathcal{H}| + 56\gamma\mathcal{T}^{2}|\mathcal{H}|  + \frac{370\gamma\mathcal{T}}{\mu L}
\end{align*}
Further let $\alpha_{k}, \beta_{k}$ be chosen as
\begin{align}\label{eq:sc_step}
    \beta_{k} = \frac{\beta_{0}}{k+1} ,\ \alpha_{k} = \frac{\alpha_{0}}{(k+1)^{2/3}}
\end{align} with $$\beta_{0} = \frac{6}{\mu\mathcal{T}}.$$Then we have
\begin{align}\label{eq:convergence_2}
    &V_{k+1} \leq \Big(\frac{1}{1+k}\Big)V_{1} + \frac{3\Gamma\alpha_{0}\beta_{0}\sigma^{2}}{(1+k)^{2/3}}.
\end{align}
\end{thm}



==> Main_Idea.tex <==
\section{Technical Assumptions and Preliminaries}
We present in this section the main technical assumptions and some preliminaries, which will help to facilitate the development of our main results later. In particular, we will consider the following two main assumptions, which are now considered to be standard in the literature of stochastic optimization. 

\begin{assumption}\label{eq:Assumption_noise}
    The The random variables $\Delta^{i}_{k}$, for all i and k, are i.i.d., and there exists a positive constant $\sigma$ such that
    \begin{align}
        &\mathbb{E}[\nabla Q^{i}(x,\Delta^{i}_{k,t})|\mathcal{P}_{k,t}] = \nabla q^{i}(x), \quad \forall x \in \mathbb{R}^{d},\notag\\
        &\mathbb{E}[\|\nabla Q^{i}(x,\Delta^{i}_{k,t})-\nabla q^{i}(x)\|^{2}|\mathcal{P}_{k,t}] \leq \sigma^{2}, \quad \forall x \in \mathbb{R}^{d}. \label{eq:sigma}
    \end{align}
\end{assumption}

\begin{assumption}\label{eq:Assumption_Lipschitz}
(Lipschitz smoothness): The non-faulty agents’
functions have Lispchitz continuous gradients, i.e. there exists a positive constant $L < \infty$ such that
\begin{align}\label{eq:Lip_condition}
    \|\nabla q^{i}(y) - \nabla q^{i}(x)\| \leq L \|y-x\|, \ \forall x,y \in \mathbb{R}^{d}.
\end{align}
\end{assumption}
\textcolor{blue}{This section added}\\In this work $x^{*}_{\mathcal{H}}$ is the set of minimizers for sum of all honest agents' cost function as indicated by the problem in \eqref{eq:exact_tolerence}. This implies that $x^{*}_{\mathcal{H}}$ is the set of minimizers for $q^{\mathcal{H}}$. Under $2f$ redundancy one can show that the following 
\begin{align}\label{eq:redundancy_condition}
    x^{*}_{\mathcal{H}} \in \bigcap \limits_{i\in \mathcal{H}} \arg \min_{x\in \mathbb{R}^{d}} q^{i}(x) = \arg \min_{x\in \mathbb{R}^{d}}\sum_{i \in \mathcal{H}}q^{i}(x) 
\end{align}
We observe that the above result does not rely on the convexity or differentiability of $q^{i}$ and holds as long as the set $\bigcap \limits_{i\in \mathcal{H}} \arg \min_{x\in \mathbb{R}^{d}} q^{i}(x)$ is non-empty. Consequently, this result is applicable to cases where $q^{\mathcal{H}}$ is strongly convex as well as the case where it is non-convex satisfying PL condition. The proof can be found in Lemma 1 of Appendix A in \cite{gupta2020resilience}.


% For the ease of understanding the proposed algorithm we consider the inner loop in algorithm $1$ in lines $6$ and $7$. Through out the paper we consider i.i.d sampling of gradients by each agents hence we consider $g^{i}(x^{i}_{k,t}) = \nabla Q^{i}(x^{i}_{k,t};\Delta ^{i}_{k,t})$, thus we have
% \begin{align}\label{eq:algo_update_Tg1}
%     &x^{i}_{k,t+1} = x^{i}_{k,t} - \beta_{k} y^{i}_{k,t},\\
%     &y^{i}_{k,t+1} = (1-\alpha_{k})y^{i}_{k,t} + \alpha_{k}\nabla Q^{i}(x^{i}_{k,t};\Delta ^{i}_{k,t}),
% \end{align}
% where $\beta_{k} << \alpha_{k}$. Note that after the agents perform local SGD in the inner loop every $\mathcal{T}$ steps the global variable $\Bar{x}_{k}$ is updated by the server after passing through the CE filter and after performing aggregation as show in lines $11-15$. The main idea for each agent is to come to consensus among themselves at $x^{*}_{\mathcal{H}}$, the optimal solution to the problem \eqref{eq:exact_tolerence}. Thus the algorithm asymptotically pushes the local estimates of the agent, $x^{i}_{k,t}$ towards the global variable $\Bar{x}_{k}$ which finally converges to $x^{*}_{\mathcal{H}}$ as the global clock approaches infinity. This motivates us to analyze the term $\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}$ which is a standard optimally gap term in optimization theory where the objectives are strongly convex. Note that since $\Bar{x}_{k}$ is the global estimate of $x^{*}_{\mathcal{H}}$ maintained by the server, we refer $\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}$ as the \textit{global optimality gap}. Next, we define the average cost of the non-faulty agents defined as 

% \begin{align}\label{eq:avg_q_h}
%     q^{\mathcal{H}}(x) = \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}q^{i}(x),
% \end{align}
% For objectives satisfying PL condition we resort to the gap between the functional value of the estimate and the optimal functional value given by $q^{\mathcal{H}}(\Bar{x}_{k}) - q^{\mathcal{H}}(x^{*}_{\mathcal{H}})$. We refer this quantity as the \textit{global functional optimality gap}. However the main idea here is to reduce the impact of variance which is a consequence of i.i.d sampling of the stochastic gradients. Thus as global clock $k$ approaches infinity, the variable $y^{i}_{k,t}$ is pushed towards the exact gradient $\nabla q^{i}(\Bar{x}_{k})$. This motivates us to introduce the \textit{gradient error} term given by
% \begin{align}\label{eq:e_k_t}
%     e^{i}_{k,t} = y^{i}_{k,t} - \nabla q^{i}(\Bar{x}_{k})
% \end{align}
% which maintains the error between the gradient estimate $y^{i}_{k,t}$ and the true gradient $q^{i}(\Bar{x}_{k})$ at every local SGD steps. We further define a variable that maintains \textit{average squared gradient error} for each global iteration given by
% \begin{align}\label{eq:e_k}
%     e_{k} = \frac{1}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\|e^{i}_{k}\|^{2}
% \end{align}
% Note that the \textit{global optimality gap} or the \textit{global functional optimality gap} solely does not guarantee that $e_{k}=0$ hence we adopt a coupled lyapunov function from the two-time scale literature given by
% \begin{align}\label{eq:lypunov_sc}
%     V_{k} = \|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} +e_{k}
% \end{align}
% for strongly convex objectives.  For objectives satisfying PL condition we consider the following lyapunov function
% \begin{align}\label{eq:lypunov_pl}
%     V_{k} = q^{\mathcal{H}}(\Bar{x}_{k}) - q^{\mathcal{H}}(x^{*}_{\mathcal{H}}) + e_{k}
% \end{align}
% Thus our goal is to study the evolution of $V_{k}$ from which we can establish the convergence rate of the algorithm $1$ for both the cases when the global objective satisfy strong convexity and non-convex with PL condition respectively. In the next section we will mention all the assumptions used throughout the rest of the paper.

% Under each assumptions of global objective we will study the one-shot gradient case when $\mathcal{T}=1$ along with the case with $\mathcal{T}>1$. For $\mathcal{T}=1$ case the agents locally perform a single update step before sending their local models to the server.Thus, the inner loop updates in this case reduces to the following
% \begin{align}\label{eq:update_Teq1}
%     &x^{i}_{k,1} = x^{i}_{k,0} - \beta_{k} y^{i}_{k,0} = \Bar{x}_{k} - \beta_{k} y^{i}_{k,0},\\
%     &y^{i}_{k,1} = (1-\alpha_{k})y^{i}_{k,0} + \alpha_{k}\nabla Q^{i}(x^{i}_{k,0};\Delta ^{i}_{k,0}).
% \end{align}
% in which case the gradient error and the cumulative gradient terms are the following
% \begin{align}\label{eq:grad_error_Teq1}
%     e^{i}_{k,0} = y^{i}_{k,0} - \nabla q^{i}(x^{i}_{k,0}), \quad e_{k} = \sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}.
% \end{align}

==> Main_results.tex <==
% \section{Preliminary Results}
% The main findings of our study are based on set of preliminary results. In this  section, we expound upon these preliminary findings, recognizing their role in establishing the main results. Our results for this section are presented in the following sections.
% \subsubsection{$\mathcal{T}=1$ case}
% \begin{lemma}
%     The gradient error, $e^{i}_{k,t}$ corresponding to an agent $i \in \mathcal{H}$ satisfy the following
% \begin{align}
%     &e^{i}_{k+1,t} = (1-\alpha_{k})e^{i}_{k,t} + (\nabla q^{i}(\Bar{x}_{k})-\nabla q^{i}(\Bar{x}_{k+1})) \notag\\
%     &+ \alpha_{k}(\nabla Q^{i}(x^{i}_{k,0};\Delta^{i}_{k,t})-\nabla q^{i}(x^{i}_{k,0})).
% \end{align}
% \end{lemma}
% \subsubsection{$\mathcal{T}>1$ case} 
% % \begin{align}
% %     &e^{i}_{k+1,t}\notag\\
% %     &= (1-\alpha_{k+1})^{t}(1-\alpha_{k})^{\mathcal{T}-t}e^{i}_{k,t} + (1-\alpha_{k+1})^{t}(1-\alpha_{k})^{\mathcal{T}-t}\nabla q^{i}(x^{i}_{k,t})\notag\\
% %     &+ \nabla q^{i}(x^{i}_{k+1,t}) + \alpha_{k}(1-\alpha_{k+1})^{t}\sum_{l=t}^{\mathcal{T}-1}(1-\alpha_{k})^{\mathcal{T}-t}\nabla Q^{i}(x^{i}_{k,i};\Delta^{i}_{k,l})\notag\\
% %     &\alpha_{k+1}\sum_{l=0}^{t-1}\sum_{l=0}^{t-1}\nabla Q^{i}(x^{i}_{k+1,l};\Delta^{i}_{k+1,l})
% % \end{align}
% \begin{lemma}
% For simplicity we consider $\alpha_{k}=\alpha$. The gradient error in this case for an honest agent $i \in \mathcal{H}$ can be expressed as
%     \begin{align}
%     e^{i}_{k+1,t} &= (1-\alpha)^{\mathcal{T}}e^{i}_{k,t} + (1-\alpha)^{\mathcal{T}}\nabla q^{i}(x^{i}_{k,t}) - \nabla q^{i}(x^{i}_{k+1,t})\notag\\
%     &+\alpha(1-\alpha)^{t}\sum_{l=t}^{\mathcal{T}-1}(1-\alpha)^{\mathcal{T}-l-1}\nabla Q^{i}(x^{i}_{k,l};\Delta^{i}_{k,l})\notag\\
%     &+\alpha\sum_{l=0}^{t-1}(1-\alpha)^{t-l-1}\nabla Q^{i}(x^{i}_{k+1,l};\Delta^{i}_{k+1,l}).
% \end{align}
% % Based on the above relation the cumulative gradient error satisfy the following
% % \begin{align}
    
% % \end{align}
% \end{lemma}
\section{Main results}
In this section we will provide our theoretical findings on the convergence properties of the two-time scale local SGD with CE filter. Here we present both the results for strongly convex and non convex with PL condition case where we investigate how Algorithm \ref{alg:cap} is affected in presence of gradient noise, local function properties and by the byzantine agents.
\subsection{Strongly convex case}
% \subsubsection{$\mathcal{T}=1$ case}
% This is a one shot gradient case where each honest agent $i$ performs a single local gradient step and sends its estimate of the local optimizer to the server. For this case the agent follow the update rule in \eqref{eq:update_Teq1}. Additionally for global iteration $k-1$ to $k$, the honest agents updates their gradient estimate as $y^{i}_{k,0} = y^{i}_{k-1,1}$. The gradient and the cumulative gradient term follows from \eqref{eq:grad_error_Teq1}. We next present the main result for this section in the following Theorem.

% \begin{thm}\label{Thm:sc_Teq1}
%     Let $\Bar{x}_{k}$ be generated by Algorithm \ref{alg:cap} for $\mathcal{T}=1$ following the updates given by \eqref{eq:update_Teq1} and assume that the following condition hold.
%     \begin{align}\label{eq:filter_condition_sc_Teq1}
%         \frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{\mu}{3L}
%     \end{align}
% Let 
% \begin{align}
%     \frac{1}{\alpha_{0}} \leq \frac{\mu}{24L},\quad \beta_{0} \leq  \frac{\mu}{48L^{2}}
% \end{align}
% Further let $\gamma$ satisfy
% \begin{align}\label{eq:sc_gamma_Teq_1}
%     \gamma_{0} \leq \gamma \leq \frac{\mu}{4L^{2}}
% \end{align}
% where 
% \begin{align*}
%     \gamma_{0} = \max \Big\{\frac{5\mu}{48L^{4}}, \frac{35}{L}\Big\}
% \end{align*}
% then
% \begin{align*}
%     V_{k+1} \leq \Big(1-\frac{\mu\beta_{k}}{4}\Big)V_{k} +\gamma\beta_{k}\alpha_{k}|\mathcal{H}|\sigma^{2}.
% \end{align*}
% Further let $\alpha_{k}, \beta_{k}$ be chosen as
% \begin{align}\label{eq:sc_step}
%     \beta_{k} = \frac{\beta_{0}}{k+1} ,\ \alpha_{k} = \frac{\alpha_{0}}{(k+1)^{2/3}},
% \end{align}
% then for time $k^{'} >0$, we have
% \begin{align}
%     V_{k+1}\leq  \frac{k^{'}}{k+1}V_{k^{'}} + \frac{3\alpha_{0}\beta_{0}\gamma_{0}|\mathcal{H}|\mathcal{T}\sigma^{2}}{(k+1)^{2/3}}
% \end{align}
% \end{thm}

\subsubsection{$\mathcal{T}>1$ case}
For $i \in \mathcal{H}$, step $6$ in Algorithm \ref{alg:cap} is equivalent to
\begin{align}\label{eq:Algo_T1}
    &x^{i}_{k,t+1} = x^{i}_{k,t} - \beta_{k}y^{i}_{k,t},\\
    & y^{i}_{k,t+1} = (1-\alpha_{k})y^{i}_{k,t} + \alpha_{k}\nabla Q^{i}(x^{i}_{k,t},\Delta^{i}_{k,t}).
\end{align}
Additionally for global iteration $k-1$ to $k$, the honest agents updates their gradient estimate as the following
\begin{align}
    y^{i}_{k,0} = y^{i}_{k-1,\mathcal{T}}
\end{align}
Further, we define the error in the gradient estimate as the following
\begin{align}\label{eq:grad_error}
    e^{i}_{k,t} = y^{i}_{k,t} - \nabla q^{i}_{k,t} 
\end{align}

From the updates we observe that as $k \to \infty$, for $i \in \mathcal{H}$, the variables in the algorithm converges as following
\begin{align}
    x^{i}_{k,t} \to \Bar{x}_{k} \to x^{*}_{\mathcal{H}}
\end{align}
Also we have as $k \to \infty$
\begin{align}
    y^{i}_{k,t} \to \nabla q^{i}(\Bar{x}_{k}),\ \implies \ y^{i}_{k,t}-\nabla q^{i}(\Bar{x}_{k}) \to 0
\end{align}
which implies
\begin{align}
    e^{i}_{k,t} \to 0
\end{align}
We also define a term that accumulates all the gradient error terms over all honest agent over a period of local SGD. We define it as
\begin{align}
    e_{k,t} = \sum_{i\in \mathcal{H}}\sum_{l=0}^{t}\|e^{i}_{k,l}\|^{2} \leq \sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}.
\end{align}
Following this definition we have
\begin{align}
   & e_{k,t+1} = \sum_{i\in \mathcal{H}}\sum_{l=0}^{t+1}\|e^{i}_{k,l}\|^{2}= \sum_{i\in \mathcal{H}}\sum_{l=0}^{t}\|e^{i}_{k,l+1}\|^{2} \notag\\
   &\leq \sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l+1}\|^{2}.
\end{align}
From the above algorithm updates we have the following relations
\begin{align}\label{eq:x_update}
     x^{i}_{k,t+1} &= x^{i}_{k,t} - \beta_{k}e^{i}_{k,t} - \beta_{k}(\nabla q^{i}(x_{k,t})-\nabla q^{i}(x^{*}_{\mathcal{H}})), \notag\\
   & = \Bar{x}_{k} - \sum_{l=0}^{t}\beta_{k}e^{i}_{k,l} - \sum_{l=0}^{t}\beta_{k}(\nabla q^{i}(x_{k,l})-\nabla q^{i}(x^{*}_{\mathcal{H}})). 
\end{align}
which also implies
\begin{align}\label{eq:x_update_capT}
    x^{i}_{k,\mathcal{T}} &= \Bar{x}_{k} - \sum_{l=0}^{\mathcal{T}-1}\beta_{k}e^{i}_{k,l}-\sum_{l=0}^{\mathcal{T}-1}\beta_{k}(\nabla q^{i}(x_{k,l})-\nabla q^{i}(x^{*}_{\mathcal{H}})).
\end{align}
The progression of the gradient error term for any $t \in [0,\mathcal{T}-1]$ is given by
\begin{align}\label{eq:e_kt}
    &e^{i}_{k,t+1} = (1-\alpha)e^{i}_{k,t} + (\nabla q^{i}(x^{i}_{k,t})-\nabla q^{i}(x^{i}_{k,t+1})) \notag\\
    &+ \alpha (\nabla Q^{i}(x^{i}_{k,t};\Delta^{i}_{k,t})-\nabla q^{i}(x^{i}_{k,t})).
\end{align}
To study the convergence rate of the algorithm we will consider the evolution of the following quantities:
\begin{itemize}
    \item Optimality gap between local variable and optima given by $\|x^{i}_{k,l} - x^{*}\|^{2}$ with any local SGD step for any $l \in [0,\mathcal{T}-1]$.
    \item Optimality gap between global variable and optima given by $\|\Bar{x}_{k} - x^{*}\|^{2}$ for any global iteration $k$.
    \item The gradient error accumulation term, $e_{k}$.
\end{itemize}
For convergence rate analysis let us consider the following coupled Lyapunov function
\begin{align}\label{eqLtwo_time_scale_lyapunov_Tgq1}
    V_{k} = \|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + \frac{\gamma \beta_{k}}{\alpha_{k}}e_{k}.
\end{align}
Our result for the stochastic setting is presented below.

%  \subsection{Non-convex satisfying PL condition}
% \subsubsection{$T=1$ case}
% The updates for honest agents $i \in \mathcal{H}$, the updates in Algorithm 1 is given by
% \begin{align}\label{eq:PL_updates_Teq1}
%     &x^{i}_{k,1} = x^{i}_{k,0} -\beta_{k}y^{i}_{k,0}, \notag\\
%     &y^{i}_{k,1} = (1-\alpha_{k})y^{i}_{k,0} + \alpha_{k}\nabla Q^{i}(x^{i}_{k,0};\Delta^{i}_{k,0})
% \end{align}
% The gradient estimation error is given by
% \begin{align}
%     e^{i}_{k,0} = y^{i}_{k,0}-\nabla q^{i}(x^{i}_{k,0})
% \end{align}
% Based on this we define a cumulative squared gradient estimation error term  given by
% \begin{align}
%     e_{k}= \sum_{i \in \mathcal{H}}\|e^{i}_{k,0}\|^{2}
% \end{align}
% % Similarly we have
% % \begin{align}
% %     e_{k,1}= \sum_{i \in \mathcal{H}}\|e^{i}_{k,1}\|^{2}
% % \end{align}
% \begin{thm}\label{theorem:PL_teq1}
%         Let $\{\Bar{x}_{k}\}$ be generated by Algorithm \ref{alg:cap} for $\mathcal{T}>1$ and assume that the following condition hold.
%     \begin{align}\label{eq:PL_filter_condition}
%         \frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{\mu}{3L}
%     \end{align}
% For the step sizes $\alpha_{k}$ and $\beta_{k}$ let the following hold 
% \begin{align}
%     \frac{1}{\alpha_{0}} \leq  \min \Big\{56,\frac{34}{L}\Big\}, \quad \beta_{0} \leq \frac{3\mu^{2}}{68L^{3}\mathcal{T}}
% \end{align}
% . Further let $\gamma$ satisfy
% \begin{align}\label{eq:PL_gamma}
%     \gamma_{0}\leq \gamma \leq \frac{17\alpha^{2}_{0}}{18L}
% \end{align}
% where 
% \begin{align*}
%     \gamma_{0} = \max\Big \{ \frac{56\mu}{L}, \frac{10L}{3}, \frac{20}{51}\Big\}
% \end{align*}
% \begin{align*}
%     V_{k} \leq \Big(1-\frac{\mu\beta_{k}}{12}\Big)V_{k} +\gamma\beta_{k}\alpha_{k}|\mathcal{H}|\sigma^{2}.
% \end{align*}
% Further let $\alpha_{k}, \beta_{k}$ be chosen as
% \begin{align}\label{eq:PL_step}
%     \beta_{k} = \frac{\beta_{0}}{k+1} ,\ \alpha_{k} = \frac{\alpha_{0}}{(k+1)^{2/3}}
% \end{align}
% then for time $k^{'} >0$, we have
% \begin{align}
%     V_{k+1} \leq  \frac{k^{'}}{k+1}V_{k^{'}} + \frac{3\alpha_{0}\beta_{0}\gamma_{0}|\mathcal{H}|\mathcal{T}\sigma^{2}}{(k+1)^{2/3}}
% \end{align}
% \end{thm}

% \subsubsection{$T>1$ case}
%  \begin{thm}\label{theorem:PL}
%     Let $\{\Bar{x}_{k}\}$ be generated by Algorithm \ref{alg:cap} for $\mathcal{T}>1$ and assume that the following condition hold.
%     \begin{align}\label{eq:PL_filter_condition}
%         \frac{|\mathcal{B}_{k}|}{|\mathcal{H}|} \leq \frac{\mu}{3L}
%     \end{align}
% Let the step sizes $\alpha_{k}$ and $\beta_{k}$ satisfy the following
% \begin{align}
%     \frac{1}{\alpha_{0}} \leq \frac{1}{4\mathcal{T}}, \quad \beta_{0} \leq \frac{\mu^{2}}{112L^{3}\mathcal{T}}
% \end{align}. Further let $\gamma$ satisfy
% \begin{align}\label{eq:PL_gamma}
%     \gamma_{0}\leq \gamma \leq \frac{\mu^{2}\mathcal{T}}{38L^{2}}
% \end{align}
% where 
% \begin{align*}
%     \gamma_{0} = \max\Big \{ \frac{3\mu\mathcal{T}}{53}, \mathcal{T}, \frac{51L^{2}\mathcal{T}^{2}}{83\mu^{2}}\Big\}
% \end{align*}
% then
% \begin{align}
%     V_{k+1,t+1}\leq \Big(1-\frac{\mu\beta_{k}L\mathcal{T}}{18}\Big)V_{k,t} + \gamma\alpha_{k}\beta_{k}\mathcal{T}|\mathcal{H}|\sigma^{2}.
% \end{align}
% Further let $\alpha_{k}, \beta_{k}$ be chosen as
% \begin{align}\label{eq:PL_step}
%     \beta_{k} = \frac{\beta_{0}}{k+1} ,\ \alpha_{k} = \frac{\alpha_{0}}{(k+1)^{2/3}}
% \end{align}
% then for time $k^{'} >0$, we have
% \begin{align}
%     V_{k+1} \leq  \frac{k^{'}}{k+1}V_{k^{'}} + \frac{3\alpha_{0}\beta_{0}\gamma_{0}|\mathcal{H}|\mathcal{T}\sigma^{2}}{(k+1)^{2/3}}
% \end{align}
% \end{thm}





==> Theorem_1.tex <==
\subsection{Theorem \ref{Theorem:SC_Tg1} proof}\label{Appendix:Theorem_sc_Tg1}
\begin{proof}
Using the update from \eqref{eq:algo_update_Tg1} and \eqref{eq:grad_error} we have
\begin{align}
    &\|x^{i}_{k,t+1} - x^{*}_{\mathcal{H}}\|\notag\\
    &\leq \|x^{i}_{k,t+!} - x^{i}_{k,t}\| + \|x^{i}_{k,t}-x^{*}_{\mathcal{H}}\|\notag\\
    & = \|x^{i}_{k,t}-x^{*}_{\mathcal{H}}\| + \beta_{k}\|y^{i}_{k,t}\|\notag\\
    &\leq \|x^{i}_{k,t}-x^{*}_{\mathcal{H}}\| + \beta_{k}L\|\Bar{x}_{k} - x^{*}_{\mathcal{H}}\| + \beta_{k}\|e^{i}_{k,t}\|\notag\\
    & \leq \|x^{i}_{k,0}-x^{*}_{\mathcal{H}}\| + (t+1)\beta_{k}L\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\| + \beta_{k}\sum_{l=0}^{t}\|e^{i}_{k,l}\|.\notag
\end{align}
Next using the fact that $x^{i}_{k,0}=\Bar{x}_{k}$ and $1+x \leq \exp{x}$ for any $x \in \mathbb{R}^{+}$ we have the following
\begin{align}
    \|x^{i}_{k,t+1} -x^{*}_{\mathcal{H}}\|&\leq (1+\beta_{k}L\mathcal{T})\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\| + \beta_{k}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|\notag\\
    & \leq\exp{(\beta_{k}L\mathcal{T})}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\| + \beta_{k}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|.\notag
\end{align}
Following from the assumption in \eqref{eq:step_size_a_b_g} we have 
\begin{align*}
    \beta_{k}L\mathcal{T} \leq \frac{\mu}{540L} \leq \frac{1}{540} \leq \ln{2}
\end{align*}
using which we have
\begin{align}
    \|x^{i}_{k,t+1}-x^{*}_{\mathcal{H}}\|\leq 2\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\| + \beta_{k}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|
\end{align}
From \eqref{eq:algo_update_Tg1} we have
\begin{align*}
    &\mathbb{E}[\|x^{i}_{k,t+1}-x^{*}_{\mathcal{H}}\|^{2}] \\
    &= \mathbb{E}[\|x^{i}_{k,t}-x^{*}_{\mathcal{H}}-\beta_{k}y^{i}_{k,t}\|^{2}]\\
    &= \mathbb{E}[\|x^{i}_{k,t}-x^{*}_{\mathcal{H}}\|^{2}] -2\beta_{k}\mathbb{E}[(x^{i}_{k,t}-x^{*}_{\mathcal{H}})^{T}y^{i}_{k,t}]+\beta_{k}^{2}\mathbb{E}[\|y^{i}_{k,t}\|^{2}]\\
    &\leq (1+L\beta_{k})\mathbb{E}[\|x^{i}_{k,t} - x^{*}_{\mathcal{H}}\|^{2}]+ \frac{\beta_{k}}{L}(1+L\beta_{k})\mathbb{E}[\|y^{i}_{k,t}\|^{2}]
\end{align*}
Next from the definition of the gradient estimation error, $e^{i}_{k,t}$ we have,
\begin{align*}
    \mathbb{E}[\|y^{i}_{k,t}\|^{2}] &= \mathbb{E}[\|e^{i}_{k,t} + \nabla q^{i}(\Bar{x}_{k})\|^{2}]\\
    &\leq 2\mathbb{E}[\|e^{i}_{k,t}\|^{2}] + 2L^{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]
\end{align*}
using which we further have
\begin{align*}
    &\mathbb{E}[\|x^{i}_{k,t+1}-x^{*}_{\mathcal{H}}\|^{2}] \\
    &\leq (1+L\beta_{k})\mathbb{E}[\|x^{i}_{k,t} - x^{*}_{\mathcal{H}}\|^{2}]\\
    &+ 2L\beta_{k}(1+L\beta_{k})\mathbb{E}[\|\bar{x}_{k} - x^{*}_{\mathcal{H}}\|^{2}]+\frac{2\beta_{k}}{L}(1+L\beta_{k})\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\\
    & \leq (1+L\beta_{k})^{t+1}\mathbb{E}[\|x^{i}_{k,0} - x^{*}_{\mathcal{H}}\|^{2}]\\
    &+ 2L\beta_{k}\sum_{l=1}^{t+1}(1+L\beta_{k})^{l}\mathbb{E}[\|\bar{x}_{k} - x^{*}_{\mathcal{H}}\|^{2}]\\
    &+\frac{2\beta_{k}}{L}\sum_{l=0}^{t}(1+L\beta_{k})^{t-l}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\\
    &\leq (1+L\beta_{k})^{\mathcal{T}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + 2(1+L\beta_{k})^{\mathcal{T}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\frac{2\beta_{k}}{L}\sum_{l=0}^{\mathcal{T}-1}(1+L\beta_{k})^{\mathcal{T}-l-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &\leq 3(1+L\beta_{k})^{\mathcal{T}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + \frac{2(1+L\beta_{k})^{\mathcal{T}}}{L}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag.
\end{align*}
Next using $1+x \leq \exp{(x)}$ for $x >0$ and $L\mathcal{T}\beta_{k} \leq \ln{(2)}$ we have
\begin{align}\label{eq:x_k_l}
    &\mathbb{E}[\|x^{i}_{k,t+1}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &\leq 3\exp{(L\mathcal{T}\beta_{k})}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]+ \frac{2\exp{(L\mathcal{T}\beta_{k})}}{L^{2}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &\leq 6\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + \frac{4}{L^{2}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}].
\end{align}
Further we have the following
\begin{align}\label{eq:error_avg}
    \|x^{i}_{k,t+1}-\Bar{x}_{k}\|^{2} &= \Big\|\sum_{l=0}^{t}(x^{i}_{k,l+1}-x^{i}_{k,l})\Big\|^{2}\notag\\
    & \leq t\sum_{l=0}^{t}\|x^{i}_{k,l+1}-x^{i}_{k,l}\|^{2} = \beta_{k}^{2}t\sum_{l=0}^{t}\|y^{i}_{k,l}\|^{2}\notag\\
    &\leq 2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}.
\end{align}
Next, using the update equation from \eqref{eq:algo_update_Tg1} we have
\begin{align}\label{eq:x_update_error}
    x^{i}_{k,t+1} &= x^{i}_{k,t} - \beta_{k} y^{i}_{k,t} \notag\\
    & = \Bar{x}_{k} -\beta_{k}\sum_{l=0}^{t}y^{i}_{k,l}\notag\\
    & = \Bar{x}_{k} -\beta_{k}\sum_{l=0}^{t}e^{i}_{k,l} -\beta_{k}\sum_{l=0}^{t}\nabla q^{i}(\Bar{x}_{k}).
\end{align}
From which we have
\begin{align}\label{eq:x_update_T}
    x^{i}_{k,\mathcal{T}} = \Bar{x}_{k} -\beta_{k}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l} -\beta_{k}\sum_{l=0}^{\mathcal{T}-1}\nabla q^{i}(\bar{x}_{k}).
\end{align}
For our analysis we note the following
    \begin{align}
        \Bar{x}_{k+1}&=\frac{1}{|\mathcal{F}_{k}|}\sum_{i \in \mathcal{F}_{k}}x^{i}_{k,\mathcal{T}}\notag \\
        &=\frac{1}{|\mathcal{H}|}\Big[\sum_{i\in \mathcal{H}}x^{i}_{k,\mathcal{T}} + \sum_{i\in \mathcal{B}_{k}}x^{i}_{k,\mathcal{T}} - \sum_{i\in \mathcal{H} \backslash \mathcal{H}_{k}}x^{i}_{k,\mathcal{T}}\Big], \notag \\
        & = \frac{1}{|\mathcal{H}|} \sum_{i\in \mathcal{H}}x^{i}_{k,\mathcal{T}}  + V_{x}.\notag
    \end{align}
    where 
    \begin{align}\label{eq:V_x}
        V_{x} = \frac{1}{|\mathcal{H}|}\Big[\sum_{i\in \mathcal{B}_{k}}(x^{i}_{k,\mathcal{T}} -\Bar{x}_{k}) - \sum_{i\in \mathcal{H} \backslash \mathcal{H}_{k}}(x^{i}_{k,\mathcal{T}}-\Bar{x}_{k})\Big]
    \end{align}
    Thus we have the following,
    \begin{align}\label{eq:x_bar_update}
        \Bar{x}_{k+1} &\overset{\eqref{eq:x_update_T}}{=} \Bar{x}_{k}-\mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\Bar{x}_{k})-\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i\in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}+ V_{k},
    \end{align}
    using which we have
    \begin{align}
        &\|\Bar{x}_{k+1} -x^{*}_{\mathcal{H}}\|^{2}\notag \\
        &= \|\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\|^{2} + \Big\|V_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big\|^{2} \notag\\
        &-2\Big(\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\Big)^{T}\Big(V_{x} -\frac{\beta_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big)\notag\\
    \end{align}
    Next using the strongly convex and lipschitz continuity assumption from \eqref{eq:sc_condition},\eqref{eq:Lip_condition} respectively we have the following
    \begin{align}\label{eq:x_bar_opt}
        &\|\Bar{x}_{k+1} -x^{*}_{\mathcal{H}}\|^{2}\notag \\
        &\leq (1-2\mu\mathcal{T}\beta_{k} + \mathcal{T}^{2}L^{2}\beta_{k}^{2})\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} +2\|V_{x}\|^{2}\notag\\
        &+\frac{2\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} + \frac{|\mathcal{H}|}{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}\|V_{x}\|^{2}\notag\\
        &+\frac{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|} \|\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\|^{2} \notag\\
        &+\frac{L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|} \|\bar{x}_{k}-x^{*}_{\mathcal{H}} - \mathcal{T}\beta_{k}\nabla q^{\mathcal{H}}(\bar{x}_{k})\|^{2}\notag\\
        &+\frac{6\beta_{k}}{L}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}\notag\\
    \end{align}
Using the inequality $2a^{T}b \leq \eta\|a\|^{2} + \frac{\|b\|^{2}}{\eta}$ for any non-zero vectors $a,b$ and for all $\eta >0$ we have 
\begin{align}
        &\|\Bar{x}_{k+1} -x^{*}_{\mathcal{H}}\|^{2}\notag \\
        & \leq (1-2\mu\mathcal{T}\beta_{k} + \mathcal{T}^{2}L^{2}\beta_{k}^{2})\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} +2\|V_{x}\|^{2}\notag\\
        &+\frac{2\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} + \frac{|\mathcal{H}|}{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}\|V_{x}\|^{2}\notag\\
        &+\frac{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{|\mathcal{H}|} (\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}+L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}) \notag\\
        &+\frac{L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|} (\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}+L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2})\notag\\
        &+\frac{6\beta_{k}}{L}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}\notag\\
        & \leq (1-2\mu\mathcal{T}\beta_{k} + \mathcal{T}^{2}L^{2}\beta_{k}^{2})\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} \notag\\
        &+\frac{19L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}+ \frac{19L^{3}\mathcal{T}^{3}\beta_{k}^{3}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} \notag\\
        &+2\|V_{x}\|^{2}+ \frac{|\mathcal{H}|}{3L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}\|V_{x}\|^{2}\notag\\
        &+\frac{2\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2} +\frac{6\beta_{k}}{L}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}.
\end{align}
Next, we analyze $\|V_{x}\|^{2}$. Using \eqref{eq:V_x} and the fact that there exists an agent $j \in \mathcal{H}\backslash \mathcal{H}_{k}$ such that $\|x^{i}_{k,t}-\Bar{x}_{k}\| \leq \|x^{j}_{k,t}-\Bar{x}_{k}\|$ for all agent $i \in \mathcal{B}_{k}$, we obtain
\begin{align}
    \|V_{x}\|^{2} &\leq \frac{2|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\|x^{j}_{k,\mathcal{T}} - \Bar{x}_{k}\|^{2} + \frac{2|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\|x^{i}_{k,\mathcal{T}} - \Bar{x}_{k}\|^{2} \notag\\
    & \leq \frac{2|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}(2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2})\notag\\
    &+ \frac{2|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}(2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2})\notag\\
    & \leq \frac{8L^{2}\mathcal{T}^{2}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + \frac{4\mathcal{T}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}\notag\\
    &+ \frac{4\mathcal{T}\beta_{k}^{2}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2},
\end{align}
From which we have 
\begin{align}\label{eq:Vk}
    \mathbb{E}[\|V_{k}\|^{2}] \leq \frac{8L^{2}\mathcal{T}^{2}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] +\frac{8\mathcal{T}\beta_{k}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\epsilon_{k},
\end{align}
where
\begin{align}
    \epsilon_{k} = \sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]
\end{align}
Now putting back putting which back \eqref{eq:Vk} in \eqref{eq:x_bar_opt} we have
\begin{align}
    &\mathbb{E}[\|\Bar{x}_{k+1}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &\leq (1-2\mu\mathcal{T}\beta_{k}+L^{2}\mathcal{T}^{2}\beta_{K}^{2})\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ \frac{35L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\frac{16L^{2}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ \frac{19L^{3}\mathcal{T}^{3}\beta^{3}_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\frac{6\beta_{k}}{L}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]+\frac{2\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+\frac{8\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]+\frac{8\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|^{2}}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+\frac{4\beta_{k}\mathcal{T}|\mathcal{B}_{k}|}{3L|\mathcal{H}|}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]+\frac{4\beta_{k}\mathcal{T}}{3L|\mathcal{H}|}\sum_{i \in \mathcal{H}\backslash\mathcal{H}_{k}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}],\notag
\end{align}
which can be further simplified as the following,
\begin{align}\label{eq:x_bar_opt}
    &\mathbb{E}[\|\Bar{x}_{k+1}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &\leq (1-2\mu\mathcal{T}\beta_{k}+L^{2}\mathcal{T}^{2}\beta_{k}^{2})\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ \frac{35L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\frac{16L^{2}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ \frac{19L^{3}\mathcal{T}^{3}\beta^{3}_{k}|\mathcal{B}_{k}|}{6|\mathcal{H}|}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\Big(2\beta^{2}_{k}\mathcal{T}\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|}+\frac{6\beta_{k}}{L} + \frac{8\beta_{k}|\mathcal{B}_{k}|}{3L|\mathcal{H}|} +  \frac{16\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\epsilon_{k},
\end{align}
where 
\begin{align}\label{eq:epsilon_k}
    \epsilon_{k}= \sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]
\end{align}
Now using the assumption $\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|}\leq \frac{\mu}{3L}$ and the result $L\mathcal{T}\beta_{k} \leq 1$ we further simplify \eqref{eq:x_bar_opt} and \eqref{eq:e_k_v1} we have
\begin{align}
     &\mathbb{E}[\|\Bar{x}_{k+1}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    & \leq (1-2\mu\mathcal{T}\beta_{k} +L^{2}\mathcal{T}^{2}\beta^{2}_{k})\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+ \Big(\frac{35L\mathcal{T}\beta_{k}}{18}+ \frac{51L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18}\Big)\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + \frac{10\beta_{k}}{L}\epsilon_{k}.
\end{align}
Here we represent the co-efficients of $\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]$ and $\epsilon_{k}$ as $C_{1}$ and $D_{1}$  as the following
\begin{align}\label{eq:C1D1}
    C_{1} =\frac{35L\mathcal{T}\beta_{k}}{18}+ \frac{51L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18}, \quad D_1 = \frac{10\beta_{k}}{L}.
\end{align}
Next from the definition of $e^{i}_{k}$ from \eqref{eq:e_k_t} we have
\begin{align}
    &e^{i}_{k,l+1}\notag\\
    &= y^{i}_{k,l+1} - \nabla q^{i}(\Bar{x}_{k}), \notag\\
    &= (1-\alpha_{k})^{l+1}y^{i}_{k,0}\notag\\
    &+ \alpha_{k}\sum_{l' = 0}^{l}(1-\alpha_{k})^{l-l'}\nabla Q^{i}(x^{i}_{k,l};\Delta^{i}_{k,l}) -\nabla q^{i}(\bar{x}_{k})\notag
\end{align}
for $l \in [0,\mathcal{T}]-1$. Next using $e^{i}_{k} = y^{i}_{0}-\Bar{x}_{k}$, we have
\begin{align}
    &\|e^{i}_{k,t}\|\notag\\
    &\leq (1-\alpha_{k})^{\mathcal{T}}\|e^{i}_{k}\| + \alpha_{k}\sum_{l^{'} = 0}^{\mathcal{T}-1}(1-\alpha_{k})^{\mathcal{T}-l'-1}\|\nabla Q^{i}(x^{i}_{k,l};\Delta^{i}_{k,l})\|\notag\\
    &+L|(1-\alpha_{k})^{\mathcal{T}}-1|\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|.\notag
\end{align}
which gives us for any $t \in [0,\mathcal{T}-1]$
\begin{align}
     &\|e^{i}_{k,t+1}\|^{2}\notag\\
     &\leq 4\|e^{i}_{k,t}\|^{2} +4L^{2}\alpha^{2}_{k}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}\notag\\
     &+ 2\alpha^{2}_{k}\mathcal{T}\sum_{l'=0}^{\mathcal{T}-1}(1-\alpha_{k})^{2\mathcal{T}-2l'-2}\|\nabla Q^{i}(x^{i}_{k,l},\Delta^{i}_{k,l})\|^{2}
\end{align}
The last term in the above equation can be analyzed as following
\begin{align}
    &2\alpha^{2}_{k}\mathcal{T}\sum_{l'=0}^{\mathcal{T}-1}(1-\alpha_{k})^{2\mathcal{T}-2l'-2}\|\nabla Q^{i}(x^{i}_{k,l},\Delta^{i}_{k,l})\|^{2}\notag\\
    &\leq 2\alpha^{2}_{k}\mathcal{T}\Big(\sum_{l'=0}^{\mathcal{T}-1}(1-\alpha_{k})^{2\mathcal{T}-2l'-2}\Big)\sum_{l'=0}^{\mathcal{T}-1}\|\nabla Q^{i}(x^{i}_{k,l},\Delta^{i}_{k,l})\|^{2}\notag\\
    & \leq 2\alpha^{2}_{k}\mathcal{T}\sum_{l'=0}^{\mathcal{T}-1}\|\nabla Q^{i}(x^{i}_{k,l},\Delta^{i}_{k,l})\|^{2}\notag
\end{align}
where we used the following
\begin{align}
    \sum_{l'=0}^{\mathcal{T}-1}(1-\alpha_{k})^{2\mathcal{T}-2l'-2} = \frac{(1-\alpha_{k})^{-2\mathcal{T}}-1}{(1-\alpha_{k})^{-2}} \leq (1-\alpha_{k})^{-2\mathcal{T}+2}
\end{align}
Thus we have
\begin{align}
     \mathbb{E}[\|e^{i}_{k,t+1}\|^{2}]&\leq 4\mathbb{E}[\|e^{i}_{k,t}\|^{2}] +4L^{2}\alpha^{2}_{k}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
     &+ 2\alpha^{2}_{k}\mathcal{T}\sum_{l'=0}^{\mathcal{T}-1}\mathbb{E}[\|\nabla Q^{i}(x^{i}_{k,l},\Delta^{i}_{k,l})\|^{2}]\notag
\end{align}
The last term in the above equation can be further be analyzed as
\begin{align}
    &2\alpha^{2}_{k}\mathcal{T}\sum_{l'=0}^{\mathcal{T}-1}\mathbb{E}[\|\nabla Q^{i}(x^{i}_{k,l},\Delta^{i}_{k,l})\|^{2}] \notag\\
    & = 2\alpha^{2}_{k}\mathcal{T}\sum_{l'=0}^{\mathcal{T}-1}\mathbb{E}[\|\nabla Q^{i}(x^{i}_{k,l},\Delta^{i}_{k,l}) - \nabla q^{i}(x^{i}_{k,l})\|^{2}] \notag\\
    &+ 2\alpha^{2}_{k}\mathcal{T}\sum_{l'=0}^{\mathcal{T}-1}\mathbb{E}[\|\nabla q^{i}(x^{i}_{k,l})\|^{2}] \notag\\
    &\overset{\eqref{eq:sigma}}{\leq}  2L^{2}\alpha^{2}_{k}\mathcal{T}\sum_{l'=0}^{\mathcal{T}-1}\mathbb{E}[\|x^{i}_{k,l}-x^{*}_{\mathcal{H}}\|^{2} + 2\alpha^{2}_{k}\mathcal{T}^{2}\sigma^{2} \notag\\
    &\overset{\eqref{eq:x_k_l}}{\leq} 12\alpha^{2}_{k}L^{2}\mathcal{T}^{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + 8\alpha^{2}_{k}\mathcal{T}^{2}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] \notag\\
    &+ 2\alpha^{2}_{k}\mathcal{T}^{2}\sigma^{2}.
\end{align}
Thus we have 
\begin{align}
     \mathbb{E}[\|e^{i}_{k,t+1}\|^{2}]& \leq 16\alpha^{2}_{k}L^{2}\mathcal{T}^{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + 8\alpha^{2}_{k}\mathcal{T}^{2}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] \notag\\
    &+ 4\mathbb{E}[\|e^{i}_{k}\|^{2}] + 2\alpha^{2}_{k}\mathcal{T}^{2}\sigma^{2}
\end{align}
Using which from the definition of $\epsilon_{k}$ we have
\begin{align}
    \epsilon_{k} \leq 4 e_{k} + 8\alpha^{2}_{k}\mathcal{T}\epsilon_{k} + 16\alpha^{2}_{k}L^{2}\mathcal{T}^{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + 2\alpha^{2}_{k}\mathcal{T}^{2}\sigma^{2}\notag
\end{align}
which gives us
\begin{align}
    \epsilon_{k} \leq \frac{4 e_{k}}{1-8\alpha^{2}_{k}\mathcal{T}^{2}} + \frac{16\alpha^{2}_{k}L^{2}\mathcal{T}^{2}}{1-8\alpha^{2}_{k}\mathcal{T}^{2}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + \frac{2\alpha^{2}_{k}\mathcal{T}^{2}\sigma^{2}}{1-8\alpha^{2}_{k}\mathcal{T}^{2}}\notag
\end{align}
Next using the assumption $\alpha_{k} \leq \frac{1}{4\mathcal{T}}$ we have 
\begin{align}\label{eq:epsilon_k}
    \epsilon_{k} \leq 8e_{k} + 32L^{2}\mathcal{T}^{2}\alpha^{2}_{k}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + 2\alpha^{2}_{k}\mathcal{T}^{2}\sigma^{2}.9
\end{align}
Next, we analyze the term $e_{k}$. For this from the definition we have the following
\begin{align}
    &e ^{i}_{k+1}\notag\\
    &= y^{i}_{k+1,0}-\nabla q^{i}(\Bar{x}_{k+1})\notag\\
    &= y^{i}_{k,\mathcal{T}}-\nabla q^{i}(\Bar{x}_{k+1})\notag\\
    &= (1-\alpha_{k})^{\mathcal{T}}y^{i}_{k,0} \notag\\
    &+ \alpha_{k}\sum_{l=0}^{\mathcal{T}-1}(1-\alpha_{k})^{\mathcal{T}-l-1}\nabla Q^{i}(x^{i}_{k,l};\Delta^{i}_{k,l}) - \nabla q^{i}(\Bar{x}_{k+1})\notag\\
    &= (1-\alpha_{k})^{\mathcal{T}}e^{i}_{k} + (1-\alpha_{k})^{\mathcal{T}}\nabla q^{i}(\Bar{x}_{k}) -\nabla q^{i}(\Bar{x}_{k+1})\notag\\
    &+ \alpha_{k}\sum_{l=0}^{\mathcal{T}-1}(1-\alpha_{k})^{\mathcal{T}-l-1}\nabla Q^{i}(x^{i}_{k,l};\Delta^{i}_{k,l})
\end{align}
using which we have
\begin{align}
    &\|e^{i}_{k+1}\|\notag\\
    &\leq (1-\alpha_{k})\|e^{i}_{k}\| + L(2-\alpha_{k})\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|+L\|\Bar{x}_{k}-\Bar{x}_{k+1}\|\notag\\
    & + \alpha_{k}\sum_{l=0}^{\mathcal{T}-1}\|\nabla Q^{i}(x^{i}_{k,l};\Delta^{i}_{k,l})\|.
\end{align}
where in the last term in the right hand side of the above inequality we let $$c_{k} = \sum_{l=0}^{\mathcal{T}-1}\|\nabla Q^{i}(x^{i}_{k,l};\Delta^{i}_{k,l})\|.$$
Next using the assumption $\alpha_{k} \geq \frac{1}{2(1+\eta)}$ we have $2-\alpha_{k} \leq \eta \alpha_{k}$ which also implies $1-\alpha_{k} \geq \eta \alpha_{k}$. Thus we have the following,
\begin{align}
    &\|e^{i}_{k+1}\|\notag\\&\leq (1-\alpha_{k})\|e^{i}_{k}\| + \eta\alpha_{k}L\|\Bar{x}_{k} - x^{*}_{\mathcal{H}}\| + L\|\Bar{x}_{k+1}-\Bar{x}_{k}\| + \alpha_{k}c_{k},\notag
\end{align}
from which we have
\begin{align}
    &\|e^{i}_{k+1}\|^{2}\notag\\
    & \leq (1-\alpha_{k})^{2}\|e^{i}_{k}\|^{2} + 2\alpha_{k}(1-\alpha_{k})\eta L\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|\|e^{i}_{k}\|\notag\\
    &+2L(1-\alpha_{k})\|\Bar{x}_{k+1}-\Bar{x}_{k}\|\|e^{i}_{k}\| + 2\alpha_{k}(1-\alpha_{k})\|\|e^{i}_{k}\|c_{k}\|\notag\\
    &+\Big\|\eta\alpha_{k}L\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|+L\|\Bar{x}_{k+1}-\Bar{x}_{k}\| +\alpha_{k}c_{k}\Big\|^{2}.
\end{align}
Next we use $(a+b)^{2} \leq 2a^{2} + 2b^{2}$ for any $a,b \in \mathbb{R}$ using which we have
\begin{align}
    &\|e^{i}_{k+1}\|^{2}\notag\\
    & \leq (1-\alpha_{k})^{2}\|e^{i}_{k}\|^{2} + 2L^{2}\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}\notag\\
    &+2\alpha_{k}(1-\alpha_{k})\eta L\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|\|e^{i}_{k}\|\notag\\
    &+2L(1-\alpha_{k})\|\Bar{x}_{k+1}-\Bar{x}_{k}\|\|e^{i}_{k}\| + 2\alpha_{k}(1-\alpha_{k})\|\|e^{i}_{k}\|c_{k}\|\notag\\.
\end{align}
Next using the inequality $2ab\leq \frac{\eta}{2} a^{2} + \frac{1}{2\eta}b^{2}$ for all $a,b \in \mathbb{R}$ and $\eta >0$, we have the following
\begin{align}\label{eq:e_i_k_1}
    &\mathbb{E}[\|e^{i}_{k+1}\|^{2}]\notag\\
    &\leq (1-\alpha_{k})^{2}\mathbb{E}[\|e^{i}_{k}\|^{2}]+ 18L^{2}\mathcal{T}^{2}\alpha^{2}_{k}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + 8\mathcal{T}^{2}\alpha^{2}_{k}\sigma^{2}\notag\\
    & + 4L^{2}\mathbb{E}[\|\Bar{x}_{k}-\Bar{x}_{k+1}\|^{2}] + 8L^{2}\mathcal{T}^{2}\alpha^{2}_{k}\beta^{2}_{k}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
     & + \frac{\alpha_{k}(1-\alpha_{k})}{4}\mathbb{E}[\|e^{i}_{k}\|^{2}]  + 36L^{2}\mathcal{T}^{2}\alpha_{k}(1-\alpha_{k})\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    & + \frac{\alpha_{k}(1-\alpha_{k})}{4}\mathbb{E}[\|e^{i}_{k}\|^{2}]  + \frac{4L^{2}}{\alpha_{k}}(1-\alpha_{k})\mathbb{E}[\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}]\notag\\
    &+\frac{\alpha_{k}(1-\alpha_{k})}{4}\mathbb{E}[\|e^{i}_{k}\|^{2}] +4L^{2}\mathcal{T}\alpha_{k}\beta^{2}_{k}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
    &+\frac{\alpha_{k}(1-\alpha_{k})}{4}\mathbb{E}[\|e^{i}_{k}\|^{2}] + 4\mathcal{T}^{2}\alpha_{k}(1-\alpha_{k})\sigma^{2}
\end{align}
Next we analyze the following term
\begin{align}\label{eq: bar_def}
    &L^{2}\mathbb{E}[\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}]\notag\\
    & \leq \frac{2L^{2}\beta^{2}_{k}\mathcal{T}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|y^{i}_{k,l}\|^{2}] + 2L^{2}\mathbb{E}[\|V_{x}\|^{2}]\notag\\
    &\leq 4L^{4}\beta^{2}_{k}\mathcal{T}^{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + \frac{4L^{4}\beta^{2}_{k}}{|\mathcal{H}|}\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}] \notag\\
    & + 2L^{2}\mathbb{E}[\|V_{x}\|^{2}]\notag\\
    &\leq \Big(4L^{4}\beta^{2}_{k}\mathcal{T}^{2} + \frac{16L^{4}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    & + \Big(\frac{4L^{2}\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}+\frac{16L^{2}\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\epsilon_{k}
\end{align}
Next using assumption on $\alpha_{k}$ from \eqref{eq:step_size_a_b_g} we have
\begin{align}
    1-\alpha_{k} \leq \eta \alpha_{k}
\end{align}
where $\eta>0$. Using this and putting back \eqref{eq: bar_def} in \eqref{eq:e_i_k_1}, using  and using the definition of $e_{k+1}$ we have,
\begin{align}\label{eq:e_k_v1}
     &e_{k+1}\notag\\
    &\leq (1-\alpha_{k})e_{k}+ \Big(18(1+2\eta)L^{2}\mathcal{T}^{2}\alpha^{2}_{k}|\mathcal{H}| + 16(1+\eta)L^{4}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{H}|\notag\\
    &+ 64(1+\eta)L^{4}\beta^{2}_{k}|\mathcal{H}|\mathcal{T}^{2}\frac{|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\mathbb{E}[\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ \Big(4(1+2\eta)L^{2}\alpha^{2}_{k}\beta^{2}_{k}\mathcal{T}|\mathcal{H}| + 16(1+\eta)L^{2}\beta^{2}_{k}|\mathcal{H}|\mathcal{T}\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|}\notag\\
    &+ 64(1+\eta)L^{2}\beta^{2}_{k}|\mathcal{H}|\mathcal{T}\frac{|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\epsilon_{k} + 4(2+\eta)\alpha^{2}_{k}\mathcal{T}|\mathcal{H}|\sigma^{2}.
\end{align}

Similarly we simplify $e_{k+1}$ from \eqref{eq:e_k_v1} as
\begin{align}\label{eq:e_k_final}
    &e_{k+1} \leq (1-\alpha_{k})e_{k}\notag\\
    &+ \Big(18(1+2\eta)L^{2}\mathcal{T}^{2}\alpha^{2}_{k} + 24(1+\eta)L^{4}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{H}|\Big)\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ \Big(13(1+\eta)L^{2}\beta^{2}_{k}\mathcal{T}|\mathcal{H}|+4(1+2\eta)L^{2}\alpha^{2}_{k}\beta^{2}_{k}\mathcal{T}|\mathcal{H}|\Big)\epsilon_{k}\notag\\
    &+4(2+\eta)\alpha^{2}_{k}\mathcal{T}|\mathcal{H}|\sigma^{2}.
\end{align}
Here we represent the co-efficients of $\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]$ and $\epsilon_{k}$ as $C_{2}$ and $D_{2}$  as the following
\begin{align}\label{eq:C2D2}
    &C_{2} = 18(1+2\eta)L^{2}\mathcal{T}^{2}\alpha^{2}_{k} + 24(1+\eta)L^{4}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{H}|,\notag\\
    &D_{2} = 13(1+\eta)L^{2}\beta^{2}_{k}\mathcal{T}|\mathcal{H}|+4(1+2\eta)L^{2}\alpha^{2}_{k}\beta^{2}_{k}\mathcal{T}|\mathcal{H}|
\end{align}
 Next, considering the two-time lyapunov function we have the following,
\begin{align}
    &V_{k+1} \notag\\
    &\leq (1-2\mu\mathcal{T}\beta_{k} + L^{2}\beta^{2}_{k}\mathcal{T}^{2})\mathbb{E}[\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + C_{1}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]  \notag\\
    &+ \frac{\gamma\beta_{k}}{\alpha_{k}}\Big((1-\alpha_{k})e_{k} + C_{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + D_{2}\epsilon_{k}\Big)+ D_{1}\epsilon_{k}\notag\\
    &+ 4\gamma(2+\eta)\alpha_{k}\beta_{k}\mathcal{T}|\mathcal{H}|\sigma^{2}.\notag
\end{align}
Now using the relation from \eqref{eq:epsilon_k} the above relation can be expressed as the following
\begin{align}
     &V_{k+1} \notag\\
    &\leq (1-2\mu\mathcal{T}\beta_{k} + L^{2}\beta^{2}_{k}\mathcal{T}^{2})\mathbb{E}[\|\bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + C_{1}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] \notag\\
    &+ \Big(104D_{1}\alpha^{2}_{k}L^{2}\mathcal{T}^{3}|\mathcal{H}| + 104\gamma\alpha_{k}\beta_{k}D_{2}L^{2}\mathcal{T}^{3}|\mathcal{H}|\Big)\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} \notag\\
    &+ \Big(\frac{\gamma \alpha_{k}}{\beta_{k}}(1-\alpha_{k}) + \frac{4\gamma\beta_{k}D_{2}\mathcal{T}}{\alpha_{k}} + 4\mathcal{T}D_{1}\Big)e_{k} + 16\alpha^{2}_{k}\mathcal{T}^{3}D_{1}|\mathcal{H}|\sigma^{2}\notag\\
    &+16\gamma\alpha_{k}\beta_{k}D_{2}\mathcal{T}^{3}|\mathcal{H}|\sigma^{2} + 4(2+\eta)\gamma\alpha_{k}\beta_{k}\mathcal{T}|\mathcal{H}|\sigma^{2},
\end{align}
which upon simplification gives us the following
\begin{align}
    &V_{k+1}\notag\\
    &\leq\Big(1-\frac{\mu\mathcal{T}\beta_{k}}{18}+\frac{69L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18}\Big)\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\Big\{936\alpha^{2}_{k}\beta_{k}L\mathcal{T}^{3}|\mathcal{H}| + 434(1+2\eta)\gamma\alpha_{k}\beta_{k}L^{2}\mathcal{T}^{4} \notag\\
    &+ \frac{24\gamma (1+\eta)\beta^{3}_{k}L^{4}\mathcal{T}^{2}|\mathcal{H}|}{\alpha_{k}} \Big\}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+ 1352(1+\eta)\gamma \alpha_{k}\beta_{k}^{3}L^{4}\mathcal{T}^{4}|\mathcal{H}|^{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\Big\{\frac{\gamma\beta_{k}(1-\alpha_{k})}{\alpha_{k}} + \frac{52\gamma(1+\eta)\beta^{3}_{k}L^{2}\mathcal{T}|\mathcal{H}|}{\alpha_{k}} \Big\}e_{k}\notag\\
    &+ \frac{36\beta_{k}\mathcal{T}}{L}e_{k} + 16\gamma(1+2\eta)\alpha_{k}\beta_{k}L^{2}\mathcal{T}^{2}|\mathcal{H}|\notag\\
    &+ 16\alpha^{2}_{k}\mathcal{T}^{3}D_{1}|\mathcal{H}|\sigma^{2} + 16\gamma\alpha_{k}\beta_{k}D_{2}\mathcal{T}^{3}|\mathcal{H}|\sigma^{2}\notag\\
    &+4(2+\eta)\gamma\alpha_{k}\beta_{k}\mathcal{T}|\mathcal{H}|\sigma^{2}.\notag
\end{align}
Upon further simplifying the above relation, we have the following
\begin{align}\label{eq:V_k_rel_v0}
    &V_{k+1}\notag\\
    &\leq\Big(1-\frac{\mu\mathcal{T}\beta_{k}}{108}\Big)V_{k}+\Big(\frac{-5\mu\mathcal{T}\beta_{k}}{108}+\frac{69L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18}\Big)\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\Big\{936\alpha^{2}_{k}\beta_{k}L\mathcal{T}^{3}|\mathcal{H}| + 434(1+2\eta)\gamma\alpha_{k}\beta_{k}L^{2}\mathcal{T}^{4} \notag\\
    &+ \frac{24\gamma (1+\eta)\beta^{3}_{k}L^{4}\mathcal{T}^{2}|\mathcal{H}|}{\alpha_{k}} + 1352(1+\eta)\gamma \alpha_{k}\beta_{k}^{3}L^{4}\mathcal{T}^{4}|\mathcal{H}|^{2}\Big\}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
    &+\Big\{-\gamma\beta_{k} + \frac{52\gamma(1+\eta)\beta^{3}_{k}L^{2}\mathcal{T}|\mathcal{H}|}{\alpha_{k}} + 16\gamma(1+2\eta)\alpha_{k}\beta_{k}L^{2}\mathcal{T}^{2}|\mathcal{H}|\Big\}e_{k}\notag\\
    &+ \Big\{\frac{36\beta_{k}\mathcal{T}}{L} + \frac{\gamma\mu\mathcal{T}\beta_{k}^{2}}{108\alpha_{k}}\Big\}e_{k} + 16\alpha^{2}_{k}\mathcal{T}^{3}D_{1}|\mathcal{H}|\sigma^{2} + 16\gamma\alpha_{k}\beta_{k}D_{2}\mathcal{T}^{3}|\mathcal{H}|\sigma^{2}\notag\\
    &+4(2+\eta)\gamma\alpha_{k}\beta_{k}\mathcal{T}|\mathcal{H}|\sigma^{2}.
\end{align}
Next using the assumptions from \eqref{eq:step_size_a_b_g} we have the following relations
% , $\beta \leq \frac{\mu}{5450L^{2}\mathcal{T}}$ and $\alpha_{k} \leq \frac{\mu}{550L\mathcal{T}}$
\begin{enumerate}
    \item Using the relation $\beta_{k} \leq \frac{\mu}{5450L^{2}\mathcal{T}}$ we have 
    \begin{align*}
        \frac{69L^{2}\mathcal{T}^{2}\beta^{2}_{k}}{18} -\frac{\mu\mathcal{T}\beta_{k}}{108} = -\mathcal{T}\beta_{k}\Big(\frac{\mu}{108} - \frac{69L^{2}\mathcal{T}\beta_{k}}{18}\Big) \leq 0
    \end{align*}
    \item Next, using $\alpha_{k} \leq \frac{\mu}{550L\mathcal{T}}$ we have
    \begin{align*}
       936\alpha^{2}_{k}\beta_{k}L\mathcal{T}^{3}|\mathcal{H}| -\frac{\mu\mathcal{T}\beta_{k}}{108} = -\mathcal{T}\beta_{k}\Big(\frac{\mu}{108} - 936\alpha^{2}_{k}L\mathcal{T}^{2}|\mathcal{H}|\Big) \leq 0
    \end{align*}
    Further using $1+2\eta \leq \zeta$, 
    \begin{align*}
        &16\gamma(1+2\eta)\alpha_{k}\beta_{k}L^{2}\mathcal{T}^{2}|\mathcal{H}| - \frac{\gamma\beta_{k}}{4} \notag\\
        &= \gamma\beta_{k}\Big(\frac{1}{4} - 16(1+2\eta)\alpha_{k}L^{2}\mathcal{T}^{2}|\mathcal{H}|\Big) \leq 0
    \end{align*}
    \item Using $\gamma \leq \frac{\mu}{(49)^{3}(1+2\zeta)L^{2}\mathcal{T}}$ we have
    \begin{align*}
        &1352(1+\eta)\gamma \alpha_{k}\beta_{k}^{3}L^{4}\mathcal{T}^{4}|\mathcal{H}|^{2} -\frac{\mu\mathcal{T}\beta_{k}}{108}\notag\\
        &\leq 676\gamma(1+2\zeta)\beta_{k}L^{2}\mathcal{T}^{2}|\mathcal{H}|-\frac{\mu\mathcal{T}\beta_{k}}{108}\notag\\
        &= -\beta_{k}\mathcal{T}\Big(\frac{\mu}{108} - 676\gamma(1+2\zeta)L^{2}\mathcal{T}|\mathcal{H}|\Big) \leq 0
    \end{align*}
Similarly we have 
\begin{align*}
    434(1+2\eta)\gamma\alpha_{k}\beta_{k}L^{2}\mathcal{T}^{4} -\frac{\mu\mathcal{T}\beta_{k}}{108} \leq 0
\end{align*}
Further using $\gamma \geq \frac{144\mathcal{T}}{L}$ we have 
\begin{align*}
    \frac{36\beta_{k}\mathcal{T}}{L} - \frac{\gamma\beta_{k}}{4} \leq 0
\end{align*}
\item Next, using the assumption on $\frac{\alpha_{k}}{\beta_{k}}$ for \eqref{eq:step_size_a_b_g} we have the following
\begin{align}
    &\frac{24\gamma (1+\eta)\beta^{3}_{k}L^{4}\mathcal{T}^{2}|\mathcal{H}|}{\alpha_{k}} - \frac{\mu\mathcal{T}\beta_{k}}{108} \leq 0, \notag\\
    &\frac{52\gamma(1+\eta)\beta^{3}_{k}L^{2}\mathcal{T}|\mathcal{H}|}{\alpha_{k}} - \frac{\gamma\beta_{k}}{4} \leq 0,\notag\\
    &\frac{\gamma\mu\mathcal{T}\beta_{k}^{2}}{108\alpha_{k}} - \frac{\gamma\beta_{k}}{4} \leq 0.\notag
\end{align}
\end{enumerate}
Putting the above relations from $1-4$ back into \eqref{eq:V_k_rel_v0} we have the following 
\begin{align*}
    V_{k+1} &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{108}\Big)V_{k}+16\alpha^{2}_{k}\mathcal{T}^{3}D_{1}|\mathcal{H}|\sigma^{2} + 16\gamma\alpha_{k}\beta_{k}D_{2}\mathcal{T}^{3}|\mathcal{H}|\sigma^{2}\notag\\
    &+4(2+\eta)\gamma\alpha_{k}\beta_{k}\mathcal{T}|\mathcal{H}|\sigma^{2}
\end{align*}
Next using the $D_1$ and $D_2$ from \eqref{eq:C1D1} and \eqref{eq:C2D2} we further simplify the above relation as the following
\begin{align*}
    &V_{k+1} \notag\\
    &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{108}\Big)V_{k}+\frac{144\alpha^{2}_{k}\beta_{k}\mathcal{T}^{3}|\mathcal{H}|\sigma^{2}}{L} +4(2+\eta)\gamma\alpha_{k}\beta_{k}\mathcal{T}|\mathcal{H}|\sigma^{2}\notag\\
    &+16\gamma\alpha_{k}\beta_{k}\Big(13(1+\eta)L^{2}\beta_{k}^{2}\mathcal{T}|\mathcal{H}| + 4(1+2\eta)L^{2}\alpha^{2}_{k}\beta^{2}_{k}\mathcal{T}|\mathcal{H}|\Big)\mathcal{T}^{3}|\mathcal{H}|\sigma^{2}\notag\\
\end{align*}
Next using \eqref{eq:eta} we have further simplify the above and arrive at \eqref{eq:convergence_1} given by 
\begin{align*}
    V_{k+1} \leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{108}\Big)V_{k} +\Gamma \alpha_{k}\beta_{k}\sigma^{2}
\end{align*}
Next we choosing the step-sizes as $\alpha_{k} = \frac{\alpha_{0}}{(1+k)^{2/3}}$ and $\beta_{k} = \frac{\beta_{0}}{(1+k)}$ with $\beta_{0} = \frac{108}{\mu\mathcal{T}}$ we get the following
\begin{align*}
    V_{k+1} &\leq \Big(\frac{k}{1+k}\Big)V_{k} + \frac{\Gamma\alpha_{0}\beta_{0}\sigma^{2}}{(1+k)^{5/3}},\notag\\
    & \leq \frac{V_{1}}{1+k} + \frac{\Gamma\alpha_{0}\beta_{0}\sigma^{2}}{1+k}\sum_{l=1}^{k}\frac{1}{(1+l)^{5/3}}, \notag\\
    &\leq \frac{V_{1}}{1+k}+ \frac{\Gamma\alpha_{0}\beta_{0}\sigma^{2}}{1+k}\int_{l=1}^{k}\frac{dl}{(1+l)^{5/3}},\notag\\
    &\leq \frac{V_{1}}{1+k}+ \frac{3\Gamma\alpha_{0}\beta_{0}\sigma^{2}}{(1+k)^{2/3}}.
\end{align*}
Hence proved.
\end{proof}
























==> Theorem_2.tex <==
\subsection{Theorem \ref{Theorem:PL_Tg1} proof}\label{Appendix:Theorem_pl_Tg1}
\begin{proof}
    Using the relations from along with \eqref{eq:PL condition} we have the following
    \begin{align}\label{eq:prerec_eq}
        &\mathbb{E}[\|x^{i}_{k,t+1}-x^{*}_{\mathcal{H}}\|^{2}] \leq \frac{6}{\mu^{2}}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + \frac{4}{L^{2}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}],\notag\\
        &\mathbb{E}[\|x^{i}_{k,t+1}-\Bar{x}_{k}\|^{2}] \notag\\
        &\leq \frac{2L^{2}\mathcal{T}^{2}\beta_{k}}{\mu^{2}}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + 2\mathcal{T}\beta^{2}_{k}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}],\notag\\
        &\mathbb{E}[\|V_{x}\|^{2}] \leq \frac{8L^{2}\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{\mu^{2}|\mathcal{H}|^{2}}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + \frac{8\mathcal{T}^{2}\beta^{2}_{k}|\mathcal{B}_{k}|^{2}}{\mu^{2}|\mathcal{H}|^{2}}e_{k}
    \end{align}
    For our analysis we consider the following
    \begin{align}\label{eq:Lipshitz_PL}
       &\mathbb{E}[q^{\mathcal{H}}(\Bar{x}_{k+1}) - q^{\mathcal{H}}(\Bar{x}_{k})]\notag\\
       &\leq \mathbb{E} [\nabla q^{\mathcal{H}}(\Bar{x}_{k})^{T}(\Bar{x}_{k+1} -\Bar{x}_{k})] + \frac{L}{2}\mathbb{E}[\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}]
    \end{align}
Using \eqref{eq:x_bar_update} we analyze the first term on the right-hand side of the above equation as
\begin{align}
    \mathbb{E} [\nabla q^{\mathcal{H}}(\Bar{x}_{k})^{T}(\Bar{x}_{k+1} -\Bar{x}_{k})] &= -\mathcal{T}\beta_{k}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + V_{x}^{T}\nabla q^{\mathcal{H}}(\Bar{x}_{k})\notag\\
    &-\frac{\beta_{k}}{|\mathcal{H}|}\Big(\sum_{i \in \mathcal{H}}\sum_{l=0}^{\mathcal{T}-1}e^{i}_{k,l}\Big)^{T}\nabla q^{\mathcal{H}}(\Bar{x}_{k}).\notag
\end{align}
Next using the inequality $2a^{T}b \leq \eta\|a\|^{2} + \frac{\|b\|^{2}}{\eta}$ for any non-zero vectors $a,b$ and for all $\eta >0$ we have 
\begin{align}\label{eq:Term1_PL}
    &\mathbb{E} [\nabla q^{\mathcal{H}}(\Bar{x}_{k})^{T}(\Bar{x}_{k+1} -\Bar{x}_{k})] \notag\\
    &\leq -\mathcal{T}\beta_{k}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + \frac{\beta_{k}\mathcal{T}L}{\mu|\mathcal{H}|}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + \frac{\beta_{k}\mu}{4L}\epsilon_{k}\notag\\
    &+ \frac{L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}{10\mu|\mathcal{H}|}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + \frac{\mu|\mathcal{H}|}{2L\mathcal{T}\beta_{k}|\mathcal{B}_{k}|}\mathbb{E}[\|V_{x}\|^{2}]\notag\\
    & \leq -\mathcal{T}\beta_{k}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + \frac{\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
    & + \Big(\frac{\mu\beta_{k}}{4L} + \frac{20\mu\beta_{k}|\mathcal{B}_{k}|}{L|\mathcal{H}|}\Big)\epsilon_{k}.
\end{align}
Here we denote the co-efficients of $\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\|^{2}$ and $\epsilon_{k}$ and $C_{1}$ and $D_{1}$ given respectively by
\begin{align}\label{eq:C1D1_PL}
    & C_{1} = -\frac{2\mathcal{T}\beta_{k}}{3} + \frac{52L^{4}\beta^{2}_{k}\mathcal{T}^{2}}{9\mu^{2}}, \notag\\
    &D_{1} = \frac{23\mu\beta_{k}}{12L} + \frac{29L^{2}\mathcal{T}\beta_{k}^{2}}{9}.
\end{align}
Next for analysis of the second term on the right-hand side of \eqref{eq:Lipshitz_PL} we use the result from \eqref{eq: bar_def} from which we have
\begin{align}\label{eq:Term2_PL}
    &\frac{L}{2}\mathbb{E}[\|\Bar{x}_{k+1}-\Bar{x}_{k}\|^{2}]\notag\\
    &\leq \Big(\frac{4L^{4}\beta^{2}_{k}\mathcal{T}^{2}}{\mu^{2}} + \frac{16L^{4}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{\mu^{2}|\mathcal{H}|^{2}}\Big)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
    & + \Big(\frac{4L^{2}\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}+\frac{16L^{2}\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\epsilon_{k}
\end{align}
Thus putting back \eqref{eq:Term1_PL} and \eqref{eq:Term2_PL} on \eqref{eq:Lipshitz_PL} we have the following
\begin{align}
    &\nabla q^{\mathcal{H}}(\Bar{x}_{k+1})-\nabla q^{\mathcal{H}}(\Bar{x}_{k})\notag\\
    &\leq \Big(-\mathcal{T}\beta_{k} + \frac{\beta_{k}L\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}+\frac{4L^{4}\beta^{2}_{k}\mathcal{T}^{2}}{\mu^{2}}\Big)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]  \notag\\
    &+ \frac{16L^{4}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{B}_{k}|^{2}}{\mu^{2}|\mathcal{H}|^{2}}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + \Big(\frac{\mu\beta_{k}}{4L} + \frac{20\mu\beta_{k}|\mathcal{B}_{k}|}{4L|\mathcal{H}|}\Big)\epsilon_{k}\notag\\
    & + \Big(\frac{4L^{2}\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|}{|\mathcal{H}|}+\frac{16L^{2}\beta^{2}_{k}\mathcal{T}|\mathcal{B}_{k}|^{2}}{|\mathcal{H}|^{2}}\Big)\epsilon_{k}.\notag
\end{align}
Now using the assumption $\frac{|\mathcal{B}_{k}|}{|\mathcal{H}|}\leq \frac{\mu}{3L}$from \eqref{} we have 
\begin{align}\label{eq:q_bar_diff}
    &\nabla q^{\mathcal{H}}(\Bar{x}_{k+1})-\nabla q^{\mathcal{H}}(\Bar{x}_{k})\notag\\
    &\leq\Big(-\frac{2\mathcal{T}\beta_{k}}{3} + \frac{52L^{4}\beta^{2}_{k}\mathcal{T}^{2}}{9\mu^{2}}\Big)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
    &+\Big(\frac{23\mu\beta_{k}}{12L} + \frac{28L^{2}\beta^{2}_{k}\mathcal{T}}{9}\Big)\epsilon_{k}
\end{align}
Next using the results from \eqref{eq:epsilon_k} and \eqref{eq:e_k_final} we have the following 
\begin{align}
    &\epsilon_{k} \leq 8\mathcal{T}e_{k} + \frac{32\alpha^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{H}|}{\mu^{2}}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + 4\alpha^{2}_{k}\mathcal{T}^{2}|\mathcal{H}|\sigma^{2},\notag\\
    &e_{k+1} \leq (1-\alpha_{k})e_{k} + C_{2}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] + D_{2} \epsilon_{k} + 4(2+\eta)\alpha^{2}_{k}\mathcal{T}|\mathcal{H}|\sigma^{2},\notag
\end{align}
using which we have the following
\begin{align}\label{eq:e_k_final}
    &e_{k+1}\notag\\
    &\leq (1-\alpha_{k})e_{k} + \Bigg(C_{2} + \frac{32\alpha^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{H}|D_{2}}{\mu^{2}}\Bigg)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}]\notag\\
    &8\mathcal{T}D_{2}e_{k} + 4\alpha^{2}_{k}\mathcal{T}^{3}|\mathcal{H}|D_{2}\sigma^{2} + 4(2+\eta)\alpha^{2}_{k}\mathcal{T}|\mathcal{H}|\sigma^{2},
\end{align}\
where $C_{2}$ and $D_{2}$ are defined as 
\begin{align}\label{eq:C2D2_PL}
    &C_{2} = \frac{18(1+2\eta)L^{2}\mathcal{T}^{2}2\alpha_{k}^{2}}{\mu^{2}} + \frac{12(1+\eta)L^{4}\beta^{2}_{k}\mathcal{T}^{2}|\mathcal{H}|}{\mu^{2}},\notag\\
    &D_{2} = 18(1+\eta)L^{2}\beta^{2}_{k}\mathcal{T}|\mathcal{H}| + 4(1+\eta)L^{2}\alpha^{2}_{k}\beta^{2}_{k}\mathcal{T}|\mathcal{H}|. 
\end{align}
Next to establish the convergence rate we consider the following Lyapunov function
\begin{align}
    V_{k} = \mathbb{E}[q^{\mathcal{H}}(\Bar{x}_{k})-q^{*}_{\mathcal{H}}] + \frac{\gamma \beta_{k}}{\alpha_{k}}e_{k},
\end{align}
Using which along with the results from \eqref{eq:q_bar_diff} and \eqref{eq:e_k_final} we have the following
\begin{align}
    &V_{k+1} - V_{k}\notag\\
    &\nabla q^{\mathcal{H}}(\Bar{x}_{k+1})-\nabla q^{\mathcal{H}}(\Bar{x}_{k}) + \frac{\gamma \beta_{k}}{\alpha_{k}}(e_{k+1}-e_{k})\notag\\
    &\leq \Bigg(C_{1} + \frac{32\alpha^{2}_{k}L^{2}\mathcal{T}^{2}|\mathcal{H}|D_{1}}{\mu^{2}}\Bigg)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2} \notag\\
    &+ \bigg( \frac{\gamma \beta_{k}C_{2}}{\alpha_{k}} + \frac{32\gamma\beta_{k}\alpha_{k}L^{2}\mathcal{H}^{2}|\mathcal{H}|D_{2}}{\mu^{2}}\Bigg)\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}\notag\\
    &+\Bigg(-\gamma \beta_{k} + \frac{8\gamma\mathcal{T}\beta_{k}D_{2}}{\alpha_{k}} + \frac{8\gamma\mathcal{T}\beta_{k}D_{1}}{\alpha_{k}}\Bigg)e_{k} + 4\alpha^{2}_{k}\mathcal{T}^{3}|\mathcal{H}|D_{1}\sigma^{2}\notag\\
    &+4\gamma\alpha_{k}\beta_{k}\mathcal{T}^{3}|\mathcal{H}|D_{2}\sigma^{2} + 4\gamma(2+\eta)\alpha_{k}\beta_{k}\mathcal{T}|\mathcal{H}|\sigma^{2}.
\end{align}
Next using the assumptions from \eqref{} we obtain the following relations:
\begin{enumerate}
    \item Using $\beta_{k} \leq \frac{3\mu^{2}}{208L^{4}\mathcal{T}}$ we have 
    \begin{align}
        \frac{52L^{4}\mathcal{T}\beta_{k}}{3\mu^{2}}-\frac{\mathcal{T}\beta_{k}}{12} \leq 0
    \end{align}
    \item Using $\alpha_{k} \leq \frac{\mu}{(27)^{2}L\mathcal{T}}$ gives
    \begin{align}
    &\frac{100L^{4}\mathcal{T}^{3}|\mathcal{H}|\alpha^{2}_{k}\beta^{2}_{k}}{\mu^{2}} - \frac{\mathcal{T}\beta_{k}}{12} \leq 0, \notag\\
    &\frac{62L\mathcal{T}^{2}|\mathcal{H}|\alpha^{2}_{k}\beta_{k}}{\mu^{2}} -- \frac{\mathcal{T}\beta_{k}}{12} \leq 0.
    \end{align}
    \item Using the assumption on $\gamma$ from \eqref{} we have the following
    \begin{align}
        &\frac{18\gamma (1+2\eta)L^{2}\mathcal{T}^{2}\alpha_{k}\beta_{k}}{\mu^{2}}-\frac{\mathcal{T}\beta_{k}}{12} \leq 0, \notag\\
        &\frac{576\gamma(1+\eta)L^{4}\mathcal{T}^{3}|\mathcal{H}|^{2}\beta^{3}_{k}\alpha_{k}}{\mu^{2}}-\frac{\mathcal{T}\beta_{k}}{12} \leq 0, \notag\\
        &\frac{128\gamma(1+2\eta)L^{4}\mathcal{T}^{3}|\mathcal{H}|^{2}\alpha^{3}_{k}\beta^{3}_{k}}{\mu^{2}} \leq 0.
    \end{align}
    \item Next, using the assumption of $\frac{\beta_{k}}{\alpha_{k}}$ from \eqref{} we have
    \begin{align}
        &\frac{24\gamma (1+\eta) L^{4}\mathcal{T}^{2}|\mathcal{H}|\beta^{3}_{k}}{\mu^{2}\alpha_{k}} -\frac{\mathcal{T}\beta_{k}}{12} \leq 0, \notag\\
        & \frac{144\gamma(1+\eta)L^{2}\mathcal{T}|\mathcal{H}|\beta^{3}_{k}}{\alpha_{k}} - \frac{\gamma \beta_{k}}{5} \leq 0, \notag\\
        & \frac{46\gamma \mu \beta^{2}_{k}}{3L\alpha_{k}} - \frac{\gamma \beta_{k}}{5} \leq 0, \notag\\
        &\frac{224\gamma L^{2}\mathcal{T}\beta^{2}_{k}}{9\alpha_{k}} -  \frac{\gamma \beta_{k}}{5} \leq 0
    \end{align}
    \item Further using $\eta \leq \zeta -\frac{1}{2}$ from \eqref{} we have 
    \begin{align}
        32\gamma(1+2\eta)L^{2}\mathcal{T}|\mathcal{H}|\alpha_{k}\beta_{k} -\frac{\gamma \beta_{k}}{5} \leq 0
    \end{align}
\end{enumerate}
Using the above relations from $1-5$ and using \eqref{eq:PL condition} we have the following
\begin{align}
    &V_{k+1} - V_{k} \notag\\
    &\leq \frac{-\mathcal{T}\beta_{k}}{12}\mathbb{E}[\|\nabla q^{\mathcal{H}}(\Bar{x}_{k})\|^{2}] -\frac{\gamma \beta_{k}}{5}e_{k} + \frac{8\mu\mathcal{T}^{3}|\mathcal{H}|\alpha_{k}\beta_{k}\sigma^{2}}{L} \notag\\
    &+ 18L\mathcal{T}^{3}|\mathcal{H}|\alpha_{k}\beta_{k}\sigma^{2} + 56\gamma\alpha_{k}\beta_{k}\mathcal{T}^{2}|\mathcal{H}|\sigma^{2} + \frac{370\gamma\alpha_{k}\beta_{k}\mathcal{T}\sigma^{2}}{\mu L}, \notag\\
    & \leq -\frac{\mu\mathcal{T}\beta_{k}}{6}V_{k} -\gamma\beta_{k}\Big(\frac{1}{10}-\frac{\mu\mathcal{T}\beta_{k}}{6\alpha_{k}}\Big)+ \frac{8\mu\mathcal{T}^{3}|\mathcal{H}|\alpha_{k}\beta_{k}\sigma^{2}}{L} \notag\\
    &+ 18L\mathcal{T}^{3}|\mathcal{H}|\alpha_{k}\beta_{k}\sigma^{2} + 56\gamma\alpha_{k}\beta_{k}\mathcal{T}^{2}|\mathcal{H}|\sigma^{2} + \frac{370\gamma\alpha_{k}\beta_{k}\mathcal{T}\sigma^{2}}{\mu L}, \notag\\
\end{align}
from which by virtue of \eqref{} reduces to
\begin{align}
    V_{k+1} &\leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{6}\Big)V_{k} + \frac{8\mu\mathcal{T}^{3}|\mathcal{H}|\alpha_{k}\beta_{k}\sigma^{2}}{L} \notag\\
    &+ 18L\mathcal{T}^{3}|\mathcal{H}|\alpha_{k}\beta_{k}\sigma^{2} + 56\gamma\alpha_{k}\beta_{k}\mathcal{T}^{2}|\mathcal{H}|\sigma^{2} + \frac{370\gamma\alpha_{k}\beta_{k}\mathcal{T}\sigma^{2}}{\mu L}. \notag\\
\end{align}
Next using \eqref{eq:eta} we have further simplify the above and arrive at \eqref{eq:convergence_1} given by 
\begin{align*}
    V_{k+1} \leq \Big(1-\frac{\mu\mathcal{T}\beta_{k}}{6}\Big)V_{k} +\Gamma \alpha_{k}\beta_{k}\sigma^{2}
\end{align*}
Next we choosing the step-sizes as $\alpha_{k} = \frac{\alpha_{0}}{(1+k)^{2/3}}$ and $\beta_{k} = \frac{\beta_{0}}{(1+k)}$ with $\beta_{0} = \frac{6}{\mu\mathcal{T}}$ we get the following
\begin{align*}
    V_{k+1} &\leq \Big(\frac{k}{1+k}\Big)V_{k} + \frac{\Gamma\alpha_{0}\beta_{0}\sigma^{2}}{(1+k)^{5/3}},\notag\\
    & \leq \frac{V_{1}}{1+k} + \frac{\Gamma\alpha_{0}\beta_{0}\sigma^{2}}{1+k}\sum_{l=1}^{k}\frac{1}{(1+l)^{5/3}}, \notag\\
    &\leq \frac{V_{1}}{1+k}+ \frac{\Gamma\alpha_{0}\beta_{0}\sigma^{2}}{1+k}\int_{l=1}^{k}\frac{dl}{(1+l)^{5/3}},\notag\\
    &\leq \frac{V_{1}}{1+k}+ \frac{3\Gamma\alpha_{0}\beta_{0}\sigma^{2}}{(1+k)^{2/3}}.
\end{align*}
Hence proved.
\end{proof}

==> results.tex <==
% % \section{Main Results}
% We begin by establishing a few preliminary results that are crucial for analysis. Firstly, using the update from \eqref{eq:algo_update_Tg1} and \eqref{eq:grad_error} we have
% \begin{align}
%     &\|x^{i}_{k,t+1} - x^{*}_{\mathcal{H}}\|\notag\\
%     &\leq \|x^{i}_{k,t+!} - x^{i}_{k,t}\| + \|x^{i}_{k,t}-x^{*}_{\mathcal{H}}\|\notag\\
%     & = \|x^{i}_{k,t}-x^{*}_{\mathcal{H}}\| + \beta_{k}\|y^{i}_{k,t}\|\notag\\
%     &\leq \|x^{i}_{k,t}-x^{*}_{\mathcal{H}}\| + \beta_{k}L\|\Bar{x}_{k} - x^{*}_{\mathcal{H}}\| + \beta_{k}\|e^{i}_{k,t}\|\notag\\
%     & \leq \|x^{i}_{k,0}-x^{*}_{\mathcal{H}}\| + (t+1)\beta_{k}L\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\| + \beta_{k}\sum_{l=0}^{t}\|e^{i}_{k,l}\|.\notag
% \end{align}
% Next using the fact that $x^{i}_{k,0}=\Bar{x}_{k}$ and $1+x \leq \exp{x}$ for any $x \in \mathbb{R}^{+}$ we have the following
% \begin{align}
%     \|x^{i}_{k,t+1} -x^{*}_{\mathcal{H}}\|&\leq (1+\beta_{k}L\mathcal{T})\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\| + \beta_{k}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|\notag\\
%     & \leq\exp{(\beta_{k}L\mathcal{T})}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\| + \beta_{k}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|.\notag
% \end{align}
% Following from the assumption in \eqref{eq:step_size_a_b_g} we have 
% \begin{align*}
%     \beta_{k}L\mathcal{T} \leq \frac{\mu}{540L} \leq \frac{1}{540} \leq \ln{2}
% \end{align*}
% using which we have
% \begin{align}
%     \|x^{i}_{k,t+1}-x^{*}_{\mathcal{H}}\|\leq 2\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\| + \beta_{k}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|
% \end{align}
% From \eqref{eq:algo_update_Tg1} we have
% \begin{align*}
%     &\mathbb{E}[\|x^{i}_{k,t+1}-x^{*}_{\mathcal{H}}\|^{2}] \\
%     &= \mathbb{E}[\|x^{i}_{k,t}-x^{*}_{\mathcal{H}}-\beta_{k}y^{i}_{k,t}\|^{2}]\\
%     &= \mathbb{E}[\|x^{i}_{k,t}-x^{*}_{\mathcal{H}}\|^{2}] -2\beta_{k}\mathbb{E}[(x^{i}_{k,t}-x^{*}_{\mathcal{H}})^{T}y^{i}_{k,t}]+\beta_{k}^{2}\mathbb{E}[\|y^{i}_{k,t}\|^{2}]\\
%     &\leq (1+L\beta_{k})\mathbb{E}[\|x^{i}_{k,t} - x^{*}_{\mathcal{H}}\|^{2}]+ \frac{\beta_{k}}{L}(1+L\beta_{k})\mathbb{E}[\|y^{i}_{k,t}\|^{2}]
% \end{align*}
% Next from the definition of the gradient estimation error, $e^{i}_{k,t}$ we have,
% \begin{align*}
%     \mathbb{E}[\|y^{i}_{k,t}\|^{2}] &= \mathbb{E}[\|e^{i}_{k,t} + \nabla q^{i}(\Bar{x}_{k})\|^{2}]\\
%     &\leq 2\mathbb{E}[\|e^{i}_{k,t}\|^{2}] + 2L^{2}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]
% \end{align*}
% using which we further have
% \begin{align*}
%     &\mathbb{E}[\|x^{i}_{k,t+1}-x^{*}_{\mathcal{H}}\|^{2}] \\
%     &\leq (1+L\beta_{k})\mathbb{E}[\|x^{i}_{k,t} - x^{*}_{\mathcal{H}}\|^{2}]\\
%     &+ 2L\beta_{k}(1+L\beta_{k})\mathbb{E}[\|\bar{x}_{k} - x^{*}_{\mathcal{H}}\|^{2}]+\frac{2\beta_{k}}{L}(1+L\beta_{k})\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\\
%     & \leq (1+L\beta_{k})^{t+1}\mathbb{E}[\|x^{i}_{k,0} - x^{*}_{\mathcal{H}}\|^{2}]\\
%     &+ 2L\beta_{k}\sum_{l=1}^{t+1}(1+L\beta_{k})^{l}\mathbb{E}[\|\bar{x}_{k} - x^{*}_{\mathcal{H}}\|^{2}]\\
%     &+\frac{2\beta_{k}}{L}\sum_{l=0}^{t}(1+L\beta_{k})^{t-l}\mathbb{E}[\|e^{i}_{k,t}\|^{2}]\\
%     &\leq (1+L\beta_{k})^{\mathcal{T}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + 2(1+L\beta_{k})^{\mathcal{T}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
%     &+\frac{2\beta_{k}}{L}\sum_{l=0}^{\mathcal{T}-1}(1+L\beta_{k})^{\mathcal{T}-l-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
%     &\leq 3(1+L\beta_{k})^{\mathcal{T}}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + \frac{2(1+L\beta_{k})^{\mathcal{T}}}{L}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag.
% \end{align*}
% Next using $1+x \leq \exp{(x)}$ for $x >0$ and $L\mathcal{T}\beta_{k} \leq \ln{(2)}$ we have
% \begin{align}\label{eq:x_k_l}
%     &\mathbb{E}[\|x^{i}_{k,t+1}-x^{*}_{\mathcal{H}}\|^{2}]\notag\\
%     &\leq 3\exp{(L\mathcal{T}\beta_{k})}\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}]+ \frac{2\exp{(L\mathcal{T}\beta_{k})}}{L^{2}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}]\notag\\
%     &\leq 6\mathbb{E}[\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2}] + \frac{4}{L^{2}}\sum_{l=0}^{\mathcal{T}-1}\mathbb{E}[\|e^{i}_{k,l}\|^{2}].
% \end{align}
% Further we have the following
% \begin{align}\label{eq:error_avg}
%     \|x^{i}_{k,t+1}-\Bar{x}_{k}\|^{2} &= \Big\|\sum_{l=0}^{t}(x^{i}_{k,l+1}-x^{i}_{k,l})\Big\|^{2}\notag\\
%     & \leq t\sum_{l=0}^{t}\|x^{i}_{k,l+1}-x^{i}_{k,l}\|^{2} = \beta_{k}^{2}t\sum_{l=0}^{t}\|y^{i}_{k,l}\|^{2}\notag\\
%     &\leq 2L^{2}\mathcal{T}^{2}\beta_{k}^{2}\|\Bar{x}_{k}-x^{*}_{\mathcal{H}}\|^{2} + 2\mathcal{T}\beta_{k}^{2}\sum_{l=0}^{\mathcal{T}-1}\|e^{i}_{k,l}\|^{2}.
% \end{align}
